The Complexity of Verifying Population Protocols

Population protocols [Angluin et al., PODC, 2004] are a model of distributed computation in which indistinguishable, finite-state agents interact in pairs to decide if their initial configuration, i.e., the initial number of agents in each state, satisfies a given property. In a seminal paper Angluin et al. classified population protocols according to their communication mechanism, and conducted an exhaustive study of the expressive power of each class, that is, of the properties they can decide [Angluin et al., Distributed Computing, 2007]. In this paper we study the correctness problem for population protocols, i.e., whether a given protocol decides a given property. A previous paper [Esparza et al., Acta Informatica, 2017] has shown that the problem is decidable for the main population protocol model, but at least as hard as the reachability problem for Petri nets, which has recently been proved to have non-elementary complexity. Motivated by this result, we study the computational complexity of the correctness problem for all other classes introduced by Angluin et al., some of which are less powerful than the main model. Our main results show that for the class of observation models the complexity of the problem is much lower, ranging from ${\Pi}_2^p$ to PSPACE.

==> correctness-intro.tex <==
First we give some notations for initial configurations and output configurations which will help us in expressing and solving the correctness problems.

\begin{definition}
\label{def:initial-configurations}
Let $\PP$ be a protocol over an alphabet $\Sigma$ and with initial state mapping $\iota$, and let $\varphi$ be a quantifier-free Presburger predicate over $\pop{\Sigma}$. 
For every $D$ in $\pop{\Sigma}$, the inital state mapping $\iota$ maps $D$ to a configuration we (abusively) note $\iota(D)$ such that $\iota(D)=\sum_{\sigma \in \Sigma} D (\sigma)\iota(\sigma)$.
For $b \in \{ 0,1 \}$, we define 
$${I}_b = \{ \iota(D) | \varphi(D)=b \}$$
the set of \emph{initial configurations that converge to $b$} if the protocol is well-specified.  

If $\PP$ is a MFDO protocol and we want to interpret ${I}_b$ as an extended configuration set, then we associate to it the minimal seen set.
\end{definition}
 
%The single-instance correctness problem can now be expressed as: given a protocol $\PP$ over an alphabet $\Sigma$ and with initial state mapping $\iota$, a quantifier-free Presburger predicate $\varphi$ over $\Sigma$ and an initial configuration $C_0 \in {I}_b$,
%do all fair runs starting in $C_0$ converge to $b$ ?

\begin{definition}
\label{def:consensusandco}
Given a population protocol $\PP$, a configuration $C$ is a \emph{stable $b$-consensus} if $C$ is a $b$-consensus and so is $C'$ for every $C'$ reachable from $C$.
Let $\Cons{b}$ denote the set of $b$-consensus configurations.
If $\PP$ is a MFDO protocol and we want to interpret $\Cons{b}$ as an extended configuration set, then we associate to it all the seen sets bigger and including the minimal seen set.

Let $\Stab{b}$ denote the set of stable $b$-consensus configurations of $\PP$. 
Observe that $\Stab{b} = \compl{\prestar(\compl{\Cons{b}})}$. 
Remark that in the MFDO setting with extended configurations, unlike for ${I}_b$ and $\Cons{b}$, describing the seen sets of $\Stab{b}$ is not trivial.
\end{definition}

For the following results, we need the predicates $\varphi$ we consider to be describable by counting constraints.
A predicate $\varphi \colon \mathbb{N}^k \rightarrow \{0,1\}$ is \emph{describable by counting constraint} if there is a counting constraint $\Gamma$ such that  $\varphi(\vec{v})=1$ if{}f $\vec{v}$ satisfies $\Gamma$.
If $\varphi$ is a predicate over $\pop{\Sigma}$ that is describable by counting constraint, $k$ is the dimension of the symbol alphabet $\Sigma$, and populations $D \in \pop{\Sigma}$ are seen as vectors $\vec{v} \in \mathbb{N}^k$.
Fortunately, as mentioned in Section \ref{sec:expressivity}, Angluin \etal show in \cite{AAER07} that IO protocols compute exactly the predicates representable by counting constraints, and DO (and so also MFDO) protocols compute a subset of these. 


We use the following repredicatetion of correctness from \cite{}.

\begin{restatable}{proposition}{PropCharacterization}
\label{prop:wellspecification}
A protocol $\PP$ is correct for a predicate $\varphi$ if{}f the following hold for $b\in \set{0,1}$:
$$\poststar({I}_{b}) \subseteq \prestar(\Stab{b} )$$
\end{restatable}

This holds when $\PP$ is an IO protocol or an MFDO protocol. 
For DO protocols, we will consider a version of this Proposition but with slightly modified reachability operators.


==> do-single-instance-well-specification.tex <==
In this section, we show that the single-instance correctness problem is in co\NP \ for MFDO protocols, and in $\Pi_2$ for DO protocols.
Combined with the hardness results of Section \ref{sec:mfdo-do-hardness}, these problems are thus complete for these complexity classes. 

Using the Shortening Theorem \ref{thm:mfdoshortening}, we prove that it is only necessary to look at "short" runs to prove single-instance correctness for MFDO protocols. 
 %Then we give a witness of non-well-specification that is describable in \PSPACE, and show that we can verify it in PTIME, thus proving the following:
First we give some notations for initial configurations and output configurations which will help us in defining and solving the correctness problems.

\begin{definition}
\label{def:initial-configurations}
Let $\PP$ be a protocol over an alphabet $\Sigma$ and with initial state mapping $\iota$, and let $\varphi$ be a quantifier-free Presburger predicate over $\Sigma$. 
For every $D$ in $\pop{\Sigma}$, the inital state mapping $\iota$ maps $D$ to a configuration we (abusively) note $\iota(D)$ such that $\iota(D)=\sum_{\sigma \in \Sigma} D (\sigma)\iota(\sigma)$.
For $b \in \{ 0,1 \}$, we define 
$${I}_b = \{ \iota(D) | \varphi(D)=b \}$$
the set of \emph{initial configurations that converge to $b$} if the protocol is well-specified.  

If $\PP$ is a MFDO protocol and we want to interpret ${I}_b$ as an extended configuration set, then we associate to it the minimal seen set.
\end{definition}
 
The single-instance correctness problem can now be expressed as: given a protocol $\PP$ over an alphabet $\Sigma$ and with initial state mapping $\iota$, a quantifier-free Presburger predicate $\varphi$ over $\Sigma$ and an initial configuration $C_0 \in {I}_b$,
do all fair runs starting in $C_0$ converge to $b$ ?

\begin{definition}
\label{def:consensusandco}
Given a population protocol $\PP$, a configuration $C$ is a \emph{stable $b$-consensus} if $C$ is a $b$-consensus and so is $C'$ for every $C'$ reachable from $C$.
Let $\Cons{b}$ denote the set of $b$-consensus configurations.
If $\PP$ is a MFDO protocol and we want to interpret $\Cons{b}$ as an extended configuration set, then we associate to it all the seen sets bigger and including the minimal seen set.

Let $\Stab{b}$ denote the set of stable $b$-consensus configurations of $\PP$. 
Observe that $\Stab{b} = \compl{\prestar(\compl{\Cons{b}})}$. 
Remark that in the MFDO setting with extended configurations, unlike for ${I}_b$ and $\Cons{b}$, describing the seen sets of $\Stab{b}$ is not trivial.
\end{definition}
 
 \begin{theorem}
 \label{thm:single-correctness-do-mfdo}
 Single-instance correctness of MFDO protocols is solvable in co-NP.
 \end{theorem}
 %
 \begin{proof}
 Let $\PP=(Q,\delta,\Sigma, \iota, o)$ be an MFDO protocol, $\varphi$ a predicate over $\pop{\Sigma}$ and $C_0$ a configuration of ${I}_b$. 
 We want to show that the problem of checking whether instance $(\PP , \varphi , C_0)$ is \emph{not} correct is in \NP.
 To do this we show that a witness $\pi$ of non-correctness is checkable in PTIME.
We let $\pi$ be a (possibly infinite) fair run $\pi=C_0C_1C_2\ldots$ such that there exists no indice $j\geq 0$ such that $C_j \in \Stab{b}$, where $\Stab{b}$ is the set of stable $b$-consensus configurations.

We use Theorem \ref{thm:mfdoshortening} to prove that we can consider only fair runs that can be described in \PSPACE.
Indeed consider a (possibly infinite) fair run $\pi=C_0C_1C_2\ldots$. 
We can equivalently consider the extended run $(C_0,\seen_0)(C_1,\seen_1)(C_2,\seen_2)\ldots$ of minimal seen sets $\mathcal{S}_i =\{ q| \exists j\leq i \ . \ C_j(q)\geq 1\}$, which we abusively also note $\pi$.
Let $\seen$ be the set of states that are visited by agents of this run, \ie the maximal seen set of $\pi$.
This set is finite as it is included in $Q$, and the seen sets can only grow over the length of the run.
Therefore there is only a finite number of transitions before all the states of $\seen$ have been visited by agents of $\pi$, and we call $k$ the first index such that this is true.

The agents of the run then move independently through the graph of allowed transitions given the seen set $\seen$.
That is, the graph whose nodes are the states of the protocol, and whose directed arcs are the transitions enabled in the protocol when the seen set is $\seen$.
%[Something about the size of this reachability graph, to prove PTIME checking]
We call bottom strongly connected component (BSCC) of the graph a maximal set of mutually reachable configurations closed under reachability.
The BSCCs of this graph can be computed in polynomial time in the size of the graph, so also in the size of the protocol. 
We mark the BSCCs of the graph such that all the states of the BSCC have output $b$, and call the resulting structure the \emph{marked graph}.

Because the run we consider is fair and the number of agents does not change, there is a only a finite number of transitions between $C_k$ and the moment in which all the agents of $\pi$ reach  BSCCs of the marked graph. 
Let us call $C$ the configuration in $\pi$ at this moment. 
If we apply Theorem \ref{thm:mfdoshortening} to the prefix of $\pi$ ending in $C$, we can replace it with a "shorter" prefix from $(C_0,\seen_0)$ to $(C,\seen)$. 
This new prefix is of the form $t_1^{k_1} t_2^{k_2} \ldots t_n^{k_n}$, with $n\leq |C_0||Q|^3$.
Let us note $\pi'$ the run that starts in $C_0$, uses this new prefix till $C$, then reuses the transitions of $\pi$.
If $\pi$ is such that there exists no indice $j\geq 0$ such that $C_j \in \Stab{b}$, then this is still the case for $\pi'$.
And $\pi'$ is still fair because we just changed a finite prefix of the fair run $\pi$.

Run $\pi'$ is \PSPACE-describable by $(\pi'|_C, \seen,M)$ where $\pi'|_C$ is the prefix of $\pi'$ until $(C,\seen)$ (which takes polynomial space in in the input), and $M$ is a multiset over the BSCCs of the marked graph of $\PP$ for seen set $\seen$ describing the number of agents in each BSCC in configuration $C$.
Any witness run $\pi$ can be turned into a "shorter" run $\pi'$ which can be described by such a "small" triple.
Checking that a run thus described is a witness for non-correctness is doable in polynomial time: we verify that the prefix is indeed a run, calculate the marked graph of $\PP$ for seen set $\seen$, and using $M$ check if all the agents are only in marked BSCCs of the marked graph, \ie the agents remain in $b$-consensuses. 
This proves single-instance correctness is a co\NP{} problem for MFDO protocols.

%Let $\pi$ be a witness fair run of the non-correctness of instance $(\PP , \varphi , C_0)$ for $\PP=(Q,M,\delta_s, \delta_r,\Sigma, \iota, o)$ a DO protocol.
%By Lemma \ref{lm:do-to-mfdo}, we can transform any finite run of a DO protocol $\PP$ to a run in the corresponding MFDO protocol of Definition \ref{def:corresponding-mfdo}.
%As above this run $\pi$ can be described by a \PSPACE-describable triple $(\pi', \seen,M)$.
%The prefix $\pi'$ can be reconverted to a DO run.
%Set $\seen$ describes the seen set but also equivalently the messages sent in this case, as we assume in our run conversion that "enough" messages are sent once the state sending them is visited.
%         \mr{What is enough? It might be that the configuration switches the output until it runs out of some kind of messages, then stabilises.}
%         So similarly we have single-instance correctness is a co\NP{} problem for DO protocols.
  \end{proof}
 
Now, before showing that the same problem is in $\Pi_2$ for DO protocols, we introduce a procedure on zero-message DO configurations called \emph{message saturation}:

Consider a configuration $C \in \N^{Q \cup M}$ such that $C(m)=0$ for all $m \in M$, and let $n$ be $C(Q)$ the number of agents in $C$.
For every populated state $q \in Q$ in $C$, let one of the agents in $q$ send $n|Q|+|Q|^2$ messages $\delta_s(q)$.
As long as there are reachable states $q$s that have not yet sent $n|Q|+|Q|^2$ messages, let an agent go there by a shortest path (which is of length at most $|Q|-1$, see proof of Theorem \ref{thm:mfdoshortening}) and let the agent send $n|Q|+|Q|^2$ messages $\delta_s(q)$.
Since at most $|Q| \times |Q|$ messages are consumed to reach new message-sending states, the resulting configuration $MS(C)$ has at least $n |Q|$ messages of each represented type, and no state emitting other message types is reachable.
Note that we always have $C \trans{*} MS(C)$.
 
 \begin{theorem}
  \label{thm:single-correctness-do}
 Single-instance correctness of DO protocols is solvable in $\Pi_2$.
 \end{theorem}
 %
 \begin{proof}
Let $\PP=(Q,M,\delta_r, \delta_s,\Sigma, \iota, o)$ be a DO protocol, $\varphi$ a predicate over $\pop{\Sigma}$ and $C_0$ a configuration of ${I}_b$. 
 We want to show that the problem of checking whether instance $(\PP , \varphi , C_0)$ is \emph{not} correct is in $\Sigma_2$. To do this we give a condition in $\Sigma_2$ and prove that $(\PP,\varphi,C_0)$ is incorrect if and only if the condition holds.
 
 Consider the following condition
 \begin{align*}
 &\exists C_D,C_{NC}. \ C_0 \trans{*} C_D \trans{*}C_{NC} \text{ and } \\
 &\forall C_{ZM}. \ C_D \trans{*} C_{ZM} \Rightarrow [ \ \exists C_D'. \ MS(C_{ZM}) \trans{*} C_D' \ ]
 \end{align*}
 where $C_D$ is a zero-message configuration, $C_{NC}$ contains at least one agent with opinion $1-b$, the $C_{ZM}$ are zero-message and $C_D'$ is equal to $D$ over $\N^Q$ but may contain messages.
 
Suppose the condition holds. 
If a stable consensus configuration $C_{SC}$ is reachable from the ``deadend" configuration $C_D$, then we can reach a zero-message configuration $C_{ZM}$ from $C_{SC}$.
Indeed, any configuration can always reach some zero-message configuration: since the message receiving transition function is total, all messages can be received by agents of the configuration, thus resulting in some new configuration with zero messages.
%perhaps export this consideration out of the proof as it is reduced for small instance lemma
We then apply the message-saturation procedure to get $MS(C_{ZM})$ and from there reach some $C_D'$ equal to $C_D$ on $\N^Q$.
From there we can reach $C_{NC}'$ equal to $C_{NC}$ on $\N^Q$ following the same transition sequence as from to $C_D$ to $C_{NC}$ (a few extra messages change nothing).
Like configuration $C_{NC}$, there is an agent in $C_{NC}'$ with opinion $1-b$, thus bringing a contradiction to $C_{SC}$ being a stable consensus.

Suppose the condition does not hold.
As discussed above, we can always reach a zero-message configuration $C$ from $C_0$.
There is a finite reachability graph on zero-message configurations.
%, and every fair run reaches a BSCC in it 
From $C$, we can always reach a zero-message configuration $C_D$ that is in a bottom strongly connected component (BSCC) of this graph.
It is reachable from all configurations reachable from it.
Since the condition does not hold, no configuration with an agent of opinion $1-b$ is reachable from it, and so it is a stable $b$-consensus.

Now let us justify that the condition is indeed in $\Sigma_2$.
The existential quantification over $C_D,C_{NC}$ include the transition sequences between them and $C_0$.
The universal quantification on $C_{ZM}$ is a universal quantification on all zero-message configurations of same size as $C_D$ and all reachability certificates. 
The latter are reachability certificates between zero-message configurations, which can be seen as reachability between configurations of the corresponding MFDO protocol to our DO protocol by Lemma \ref{lm:do-to-mfdo}.
As in the proof of Theorem \ref{thm:single-correctness-do-mfdo} these certificates are in \NP.

Finally,  we show that the reachability condition on $MS(C_{ZM})$ does not actually require a new existential quantifier (putting our condition in $\Sigma_3$).
Configuration $MS(C_{ZM})$ has enough messages that it does not need to send new ones to get to any new configuration.
Indeed if an agent can go from $q$ to $q'$ it can go there in $|Q|-1$ receive transitions, and each reachable message exists in the configuration.
So the question of whether $MS(C_{ZM})$ can reach $C_D'$ such that $C_D|_Q = C_D'|_Q$ is only a question of how to transfer all the agents.
To solve this question, we can apply the Edmonds-Karp algorithm to the following graph with capacities:

\begin{itemize} 
\item Let the nodes be $|Q|$ copies of the states of the protocol written $q^{(1)},q^{(2)}, \ldots q^{(|Q|)}$ for each $q \in Q$, a source node $s$, and a target node $t$.

\item Let there be directed arcs from $s$ to each $q^{(1)}$ with capacity $MS(C_{ZM})(q)$ and from each $q^{(|Q|)}$ to $t$ with capacity $C_D(q)$.

\item For each $i=1,\ldots,|Q|-1$, let there be a directed arc from $q^{(i)}$ to $q'^{(i+1)}$ whenever there is a receive transition from $q$ to $q'$ using a message of $MS(C_{ZM})$ in the protocol, or when $q=q'$. 
These arcs have capacity $\infty$.
\end{itemize} 

If there exists a maximum flow solution to this graph, then it uses a flow of value $\sum_q MS(C_{ZM})(q)= \sum_q C_D(q)$, by construction because there are no inner edges with smaller capacity.
This gives a solution to the reachability problem of whether $MS(C_{ZM})$ can reach a configuration with the same agent distribution as $C_D$.
If there is a transition sequence from $MS(C_{ZM})$ to a configuration with the same agent distribution as $C_D$, then there is a solution in this capacity graph by taking the arcs corresponding to the transitions of the sequence.

\cwk{the graph could also be defined using only two copies of each q. would this be better ?}
%For example, we can enumerate the point-to-point reachability
%in the graph by brute force, then apply Edmonds-Karp algorithm to the graph
%[source — $MS(q)$ capacity — $\uparrow q$ — infinite capacity — $q \downarrow$ — $D(q)$ — target] to
%check if we can match all the agents. \cwk{to be rewritten more clearly}
  \end{proof}


==> do-well-specification.tex <==
Using the results of the pruning section, we show that the MFDO general correctness problem is also solvable in co\NP. 
To describe (possibly infinite) sets of configurations, we reuse the notions of counting sets introduced in \cite{EsparzaGMW18} - which is in the context of IO protocols - in the new context of MFDO. 
The results still hold, with even better bounds because of the better bound on the MFDO Pruning Theorem.

%almost directly from old article
\paragraph{Counting constraints and counting sets. }  A \emph{cube} of a protocol $\PP$ is defined as a set of configurations given by a lower bound $L \colon P \rightarrow \N$ and an upper bound $U \colon Q \rightarrow \N \cup \{\infty\}$, written $(L,U)$, and such that configuration $C \in (L,U)$ if{}f $L \leq C \leq U$. 
In the rest of the paper, the term cube will refer both to the set of configurations and to the description by upper and lower bound $(L,U)$.
A \emph{counting constraint} is a formal finite union of cubes, i.e. a formal finite union of upper and lower bound pairs of the form $(L,U)$.
The semantics of a counting constraint is called a \emph{counting set} and it is the union of the cubes defining the counting constraint.
The counting set for a counting constraint $\Gamma$ is denoted $\sem{\Gamma}$.
Notice that one counting set can be the semantics of different counting constraints.
For example, consider a protocol with just one state $q_1$. Let $(L,U)=(1,3)$, $(L',U')=(2,4)$, $(L'',U'')=(1,4)$. 
The counting constraints $(L,U)\cup(L',U')$ and $(L'',U'')$ define the same counting set.
It is easy to show (see also \cite{EsparzaGMW18}) that counting sets are closed under Boolean operations.

%\cwk{new}
An \emph{extended cube} is defined as a cube $\mathcal{C}$ and a seen set $\mathcal{S}$.
An \emph{extended counting constraint} is a formal finite union of extended cubes, and its semantics is called an \emph{extended counting set}.

\paragraph{Measures of counting constraints.} Let $\mathcal{C}=(L,U)$ be a cube, and let $\Gamma = \bigcup_{i=1}^m \mathcal{C}_i$
be a counting constraint. We use the following notations:
$$\begin{array}{lcl}
\lnorm{\mathcal{C}} \defeq \displaystyle \sum_{p \in Q} L(p) & \quad & \unorm{\mathcal{C}} \defeq \displaystyle \sum_{\substack{p\in Q\\ U(p)<\infty}} \!\!\!\!U(p) \mbox{ (and \( 0\) if \(U(p)=\infty\) for all \(p\))}. \\[0.2cm]
\lnorm{\Gamma} \defeq \displaystyle \max_{i\in [1,m]} \{ \lnorm{\mathcal{C}_i} \} &  & \unorm{\Gamma} \defeq \displaystyle \max_{i\in[1,m]} \{ \unorm{\mathcal{C}_i} \}
\end{array}$$
\noindent We call $\lnorm{\mathcal{C}}$ the $l$-norm  and $\unorm{\mathcal{C}}$ the $u$-norm of $\mathcal{C}$. Similarly for $\Gamma$.
We recall Proposition 5 of~\cite{EsparzaGMW18} for the norms of the union, intersection and complement.

\begin{proposition}
\label{prop:oponconf}
Let $\Gamma_1, \Gamma_2$ be counting constraints.
\begin{itemize}
\item There exists a counting constraint $\Gamma$ with $\sem{\Gamma} = \sem{\Gamma_1} \cup \sem{\Gamma_2}$ such that
$\unorm{\Gamma} \leq \max \{\unorm{\Gamma_1}, \unorm{\Gamma_2} \}$ and $\lnorm{\Gamma} \leq \max \{\lnorm{\Gamma_1}, \lnorm{\Gamma_2} \}$.
%
\item  There exists a counting constraint $\Gamma$ with $\sem{\Gamma} = \sem{\Gamma_1} \cap \sem{\Gamma_2}$ such that
$\unorm{\Gamma} \leq \unorm{\Gamma_1} + \unorm{\Gamma_2}$ and $\lnorm{\Gamma} \leq \lnorm{\Gamma_1} + \lnorm{\Gamma_2}$.
%
\item There exists a counting constraint $\Gamma$ with $\sem{\Gamma} = \N^n \setminus \sem{\Gamma_1}$ such that
$\unorm{\Gamma} \leq n\lnorm{\Gamma_1}$ and $\lnorm{\Gamma} \leq n\unorm{\Gamma_1} + n$.
%
\end{itemize}
 \end{proposition}

%\cwk{new}
We do not take the seen sets into account when defining the norm 
of an extended counting constraint. 
Indeed, a seen set is always of size smaller or equal to the number of states, and so is negligible in the context of our complexity problems.

\paragraph{Predecessors and successors of counting sets.}
Fix an MFDO protocol $\PP$. The sets of predecessors and successors of a set $\mathcal{M}$ of configurations of $\PP$ are defined as follows:
$\prestar(\mathcal{M}) \defeq \{ C' | \exists C \in \mathcal{M} \, . \, C' \xrightarrow{*} C \}$, and 
$\poststar(\mathcal{M}) \defeq \{ C | \exists C' \in \mathcal{M} \, . \, C' \xrightarrow{*} C \}$.\\
%\cwk{new} 
The predecessor set and successor set for an extended counting set $(\mathcal{M},\mathcal{S})$ are:
$\prestar(\mathcal{M},\mathcal{S}) \defeq \{ (C',\mathcal{S}') | \exists C \in \mathcal{C} \, . \, (C',\mathcal{S}') \xrightarrow{*} (C,\mathcal{S}) \}$, and
$\poststar(\mathcal{M},\mathcal{S}) \defeq \{ (C,\mathcal{S}') | \exists C' \in \mathcal{M} \, . \, (C',\mathcal{S}) \xrightarrow{*} (C,\mathcal{S}') \}$

%\cwk{end of part from old article}

\begin{lemma}
\label{lm:smallminterm}
%\cwk{we could change the notation of cube to $\mathcal{K}$ to not have notation problems}
Let $(\mathcal{C},\mathcal{S})$ be an extended cube of an MFDO protocol $\PP$ of state set $Q$.
For all $(C',\mathcal{S}') \in \prestar(\mathcal{C},\mathcal{S})$, there exists an extended cube $(\mathcal{C}',\mathcal{S}')$ such that 
\begin{enumerate}
\item $(C',\mathcal{S}') \in (\mathcal{C}',\mathcal{S}') \subseteq  \prestar(\mathcal{C},\mathcal{S})$, and
\item $\lnorm{\mathcal{C}'} \leq \lnorm{\mathcal{C}}  + |Q|$ and $\unorm{\mathcal{C}'} \leq \unorm{\mathcal{C}}$.
\end{enumerate}
\end{lemma}
%
\begin{proof}
Let $L\in \N^Q$, $U\in (\N \cup \{ \infty \})^Q$ be lower and upper bounds such that $\mathcal{C}=(L,U)$.
Let $(C',\mathcal{S}')$ be an extended configuration of $\prestar(\mathcal{C},\mathcal{S})$.
There exists a configuration $C \in (L,U)$ such that $(C',\mathcal{S}') \trans{*} (C,\mathcal{S})$, and $C \geq L$.
The construction from the Pruning Theorem applied to this run yields configurations $D',D$ such that 
\begin{center}
\(
\begin{array}[b]{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
(C',\mathcal{S}') &  \trans{\hspace{1em}*\hspace{1em}} & (C,\mathcal{S}) & \  \geq \ &L  \\[0.1cm]
\geq &  & \geq \\[0.1cm]
(D',\mathcal{S}') & \trans{\hspace{1em}*\hspace{1em}} &(D,\mathcal{S})  & \geq & L
\end{array}
\)
\end{center}
and $|D'| \leq |L| + |Q|$.
Since $C$ is in $(L,U)$, we have $U\geq C \geq D \geq L$ and so configuration $D$ is in $\mathcal{C}=(L,U)$ and $D'$ is in $\prestar(\mathcal{C},\mathcal{S})$.

We want to find $\mathcal{C}'$ satisfying the conditions of the Lemma, i.e. such that $C' \in \mathcal{C}'$ and $(\mathcal{C}',\mathcal{S}') \subseteq  \prestar(\mathcal{C},\mathcal{S})$.
We define $L'$ as equal to configuration $D'$ over each state of $Q$.
The following part of the proof plays out in the setting of the pruning theorems section, in which the agents are de-anonymized. 
Let $(H_C, \mathcal{S}')$ be a well-structured realizable extended history from $(C',\mathcal{S}')$ to $(C,\mathcal{S})$. 
For each $q\in Q$, we define $U'(q)$ depending on the final states of trajectories in $H_C$ that have $q$ as initial state.

\noindent
\emph{Case 1.} 
If there exists a trajectory in $H_C$ that has $q$ as initial state and whose final state $p$ is such that $U(p) = \infty$, then we define $U'(q)$ to be $\infty$.

\noindent
\emph{Case 2.}
Otherwise, we define $U'(q)$ to be equal to $C'(q)$.

%We define $L'$ as equal to configuration $D'$ and $U'$ equal to $C'$ over each state of $Q$.
%\mr{If $U$ has infinities and $C'$ is large enough,
%        $U'$ will have an unacceptably high norm}
Let $\mathcal{C}'$ be the cube defined by $(L',U')$.
Let us show that cube $\mathcal{C}'$ has the properties we want.
The construction from the Pruning Theorem ``prunes" extended history $(H_C,\mathcal{S}')$ into a well-structured realizable extended history $(H_D,\mathcal{S}')$ from $(D',\mathcal{S}')$ to $(D,\mathcal{S})$, where $H_D$ is a set $\{ \tau_q | q \in Q \}$ of trajectories first reaching states $q$ at the same moment as in $H_C$ plus a set $H_L \subseteq H_C$ of trajectories reaching configuration $L$.
We are going to show that $\mathcal{C}' \subseteq \prestar(\mathcal{C},\mathcal{S})$ by ``re-adding" trajectories of history $H_C$ to history $H_D$ to create extended histories $(H_R,\mathcal{S}')$ which will start in any configuration $(R',\mathcal{S}')$ of $(\mathcal{C}',\mathcal{S}')$ and end at some configuration $(R,\mathcal{S})$ in $(\mathcal{C},\mathcal{S})$.
Figure \ref{figure-boost} illustrates the case where $R' \in \mathcal{C}'$ and $R'\leq C'$.

\input{figure-boost.tex}

Let $R'$ be any configuration in $\mathcal{C}'=(L',U')$.
For each state $q$, we have $D'(q)=L'(q) \leq R'(q) \leq U'(q)$.
We initialize a new history $H_R$ as the trajectories of history $H_D$.
For each state $q \in Q$ such that $U'(q)=C'(q)$, we add $R'(q)-D'(q)$ trajectories beginning in $q$ from $H_C-H_D$. 
These trajectories exist because $ R'(q) \leq C'(q)$.
For each state $q \in Q$ such that $U'(q)=\infty$, we pick a trajectory from $q$ to $p$ such that $U(p)=\infty$ in $H_C$ and add it to $H_R$ with multiplicity $R'(q)-D'(q)$.
Informally we do not need to worry about exceeding the upper bounds of $\mathcal{C}$ because the upper bound of the final place of this trajectory is infinite.

The resulting augmented extended history $(H_R,\mathcal{S}')$ is still well-structured and realizable as the set $\{ \tau_q | q \in Q \}$ of "enabling" trajectories (that first see states at the right moment) is still present. 
%argument similar to the one of the pruning theorem, to be done?

History $H_R$ begins in configuration $R'$ and ends in a configuration $R$.
Configuration $R$ covers $D\geq L$ because history $H_R$ was initialized on history $H_D$ and we have only added agents to the final configuration of the history.
Configuration $R$ is covered by $U$ because we added either trajectories that arrive in a state $p$ in which $U$ is unbounded, or trajectories that were already present in $H_C$.
%a little akward, could be rewritten
So $R \in \mathcal{C}=(L,U)$ and $R' \in \prestar(\mathcal{C})$.

Finally, we show that the norms of $(L',U')$ are bounded.
For the $l$-norm, we simply add up the tokens in $D=L'$. 
Thus by the Pruning theorem
\begin{align*}
\lnorm{\mathcal{C}'} \leq |L| + |Q| \leq \lnorm{\mathcal{C}} + |Q|
\end{align*}
%
By definition of the $u$-norm and $U'$, 
$$
\unorm{\mathcal{C'}} = \sum_{\substack{q\in Q | U'(q)<\infty}} U'(q) = \sum_{\substack{q\in Q | U'(q)<\infty}} C'(q).
$$
If $U'(q)<\infty$ then all the trajectories from $q$ in $H_C$ go to some $p$ such that $U(p)<\infty$. So:
\begin{align*}
\unorm{\mathcal{C'}} = \sum_{\substack{q\in Q | U'(q)<\infty}} C'(q) &\leq \sum_{\substack{q\in Q | U(q)<\infty}} C(q) \\
 &\leq \sum_{\substack{q\in Q | U(q)<\infty}} U(q) = \unorm{\mathcal{C}}.
\end{align*}
%there are also traj leaving from q such that U'(q)=infty going to p such that U(p)<infty
 \end{proof}

This results in the following theorem:

\begin{restatable}{theorem}{ThmCCReachability}
\label{thm:reachofcc}
Let $\PP$ be an MFDO protocol with a set $Q$ of states, and let $\mathcal{D}$ be an extended counting set. \cwk{what is a good notation for extended counting cstrs/sets?}
Then $pre^*(\mathcal{D})$ is an extended counting set and there exist extended counting constraints $\Gamma$ and $\Gamma'$ satisfying $\sem{\Gamma} = \mathcal{D}$, $\sem{\Gamma'} = \prestar(\mathcal{D})$ and we can bound the norm of $\Gamma'$ by
 \begin{align*}
\unorm{\Gamma'} \leq \unorm{\Gamma} \text{ and }
\lnorm{\Gamma'} \leq  \lnorm{\Gamma} + |Q|
 \end{align*}
The same holds for $\poststar$ by using the protocol with reversed transitions.
%TRUE FOR ANY GAMMA REPRESENTING D - CHANGE ?
\end{restatable}
%
\begin{proof}[Sketch]
%careful, this is the same proof sketch as for IO
Lemma \ref{lm:smallminterm} gives ``small" extended cubes such that $\prestar(\mathcal{D})$ is the union of these extended cubes.
Since there are only a finite number of such ``small" extended cubes, this union is finite and $\prestar(\mathcal{D})$ is an extended counting set. 
The bounds on the norms of $\prestar(\mathcal{D})$ are derived from the bounds on the norms of these extended cubes.
 \end{proof}

We are going to show that correctness can be reduced to reachability questions over certain counting sets which are "small" (in terms of number of agents of their minimal configurations), and thus we need only study "small" instances to prove correctness.
%Theorem \ref{thm:reachofcc} tell us that we can concentrate on configurations with "small" agent count to prove whether a protocol is correct.
We use the following repredicatetion of correctness from \cite{CONCUR}.

\begin{proposition}
\label{prop:wellspecification}
A protocol is correct if{}f the following hold for $b=0,1$:
$$\poststar({I}_{b}) \subseteq \prestar(\Stab{b} )$$
\end{proposition}
%insert proof that will go to appendix

For the following results, we need the predicates $\varphi$ we consider to be describable by counting constraints.
That is, predicates $\varphi \colon \mathbb{N}^k \rightarrow \{0,1\}$ for which there is a counting constraint $\Gamma$  such that  $\varphi(\vec{v})=1$ if{}f $\vec{v}$ satisfies $\Gamma$.
Fortunately, in \cite{AAER07} Angluin \etal show that IO protocols compute exactly the predicates representable by counting constraints, and DO protocols compute a subset of these. 
Since DO and MFDO have the same expressivity, this is also true for MFDO.
\cwk{This needs to be changed to fit our setting of predicate representation, but it is a placeholder for now}

\begin{lemma}
        \label{lemma:mfdo-do-non-ws-pruning}
        If a
        MFDO protocol
        or a
        DO protocol
        with state set $Q$
        is not correct for a predicate $\varphi$,
        then it is not correct on some specific instance
        with agent count polynomial in the size of the input, \ie in $|Q|$ and $size(\varphi)$.
\end{lemma}
%
\begin{proof}
If a protocol is not correct, then there exists, for some $b\in \{0,1\}$ a configuration in ${I}_b$ that does not converge to $b$.
Let us fix this $b$ for the rest of the proof.
The result relies on the fact that both $\Stab{b}$ and ${I}_b$ are counting sets with "small" norms relative to the size of the input, \ie $\PP$ and $\varphi$.
Indeed, recall that $\Stab{b}$ is given by $\compl{ \prestar( \compl{ \Cons{b} } ) }$ where $\Cons{b}$, for $b \in \{ 0,1 \}$, can be represented by the cube defined by the upper bound equal to $0$ on all places $q$ with output $o(q)=1-b$ and $\infty$ otherwise, and the lower bound equal to $0$ everywhere. 
By Proposition \ref{prop:oponconf} and Theorem \ref{thm:reachofcc}, $\Stab{b}$ is a counting set of polynomial norm.
Since $\varphi$ is a predicate representable by a counting constraint, ${I}_b$ is either this counting constraint or the counting constraint corresponding to $1-\varphi$.

\noindent \textbf{MFDO Case: }First we consider the message-free delayed observation case.
        By Proposition \ref{prop:wellspecification}, the condition for correctness can be rewritten as 
\begin{equation*}
\poststar({I}_{b}) \cap \compl{\prestar(\Stab{b} )} = \emptyset.
\end{equation*}
        By Proposition \ref{prop:oponconf} and Theorem \ref{thm:reachofcc}, this
        is an equality between a counting set with
        polynomial norm and the empty set.
        If equality is false, by definition of the norm of a counting set, there is a configuration
        of size smaller or equal to the norm in the intersection.
        This provides us our incorrect instance.

\noindent \textbf{DO Case: }Now we consider delayed observation protocols. 
We are again going to consider an expression of correctness as a predicate over sets of configurations, but we need a new operator $\widetilde{\prestar}$ to do so.

Before defining this new operator, we remark that any configuration can always reach some zero-message configuration.
Indeed, since the message receiving transition function is total, all messages in a DO configuration can be received by agents of the configuration, thus resulting in some new configuration with zero messages.

For $C \in \N^Q$ defining a zero-message configuration of our DO protocol, we define $\widetilde{\prestar}(C)$ as the zero-message configurations $C'$ such that 
$$
(C',\seen_{C'}) \in \bigcup_{\seen | \seen \supseteq \text{ minimal seen set for } C} \prestar(C,\seen)
$$
where $\seen_{C'}$ is the minimal seen set for $C'$, and the operator $\prestar$ is applied in the MFDO protocol corresponding to our DO protocol (see Definition \ref{def:corresponding-mfdo}).

By Lemma \ref{lm:do-to-mfdo} and the above discussion on zero-message configurations, this operator describes zero-message reachability in our DO protocol (\ie reachability from a configuration with zero messages to another configuration with zero messages).
By Proposition \ref{prop:oponconf} and Theorem \ref{thm:reachofcc} and the fact that the norm of an extended counting set does not take into account the seen set, the bounds on the number of agents of the minimal configurations in $\widetilde{\prestar}(C)$ are still polynomial in $|Q|$ and $|C|$.

We express correctness as
\begin{equation*}
%\label{do-correctness}
{I}_{b} \cap \widetilde{\prestar}(\compl{\widetilde{\prestar}(\widetilde{\Stab{b}} )}) = \emptyset.
\end{equation*}
where $\widetilde{\Stab{b}}$ is equal to $\compl{\widetilde{\prestar}( \compl{ \Cons{b} } ) }$.
Indeed, DO initial configurations are zero-message.
Now we need to argue that reaching zero-message non-$b$-consensus is always possible if we can reach non-$b$-consensus with messages. 
This is true as soon as we have $\geq 2$ agents, because we can keep one agent that has output $1-b$ and let the other agents consume all the messages. 

By the definition of $\widetilde{\prestar}$, the norms on the counting sets describing the agent count of $\widetilde{\prestar}(\compl{\widetilde{\prestar}(\widetilde{\Stab{b}} )})$ are polynomial in the input.
So if the intersection is non-empty, there exists a (zero-message) configuration in the intersection with polynomial agent count.
 \end{proof}

\begin{theorem}
        The correctness problem for
               message-free delayed observation protocols
%        and
%        delayed observation
        protocols 
        is in co\NP.
\end{theorem}
%
\begin{proof}
By Lemma~\ref{lemma:mfdo-do-non-ws-pruning}, 
        it is enough to verify single-instance correctness for
        all instances with agent count up to $O(|Q|^k)$.
        Non-correctness means that there exists
        an initial configuration that doesn't satisfy 
        single-instance correctness.
%        Since initial configurations are always zero-message, only their agent count determines their size.
        By Theorem~\ref{thm:single-correctness-do-mfdo}, single-instance non-correctness
        has polynomial-time verifiable certificates.
        A pair of an initial configuration and its non-correctness
        certificate is a certificate of global non-correctness, and therefore correctness of MFDO is in co\NP.
 \end{proof}

\begin{theorem}
        The correctness problem for delayed observation
        protocols 
        is in $\Pi_2$.
\end{theorem}
%
\begin{proof}
By Lemma~\ref{lemma:mfdo-do-non-ws-pruning}, 
it is enough to verify single-instance correctness for
all instances with agent count up to $O(|Q|^k)$.
Non-correctness means that there exists
an initial configuration that doesn't satisfy 
single-instance correctness, and initial configurations are zero-message in DO protocols, \ie completely defined by their agent count.
By Theorem~\ref{thm:single-correctness-do}, single-instance non-correctness over a configuration $C_0$ can be characterized by a $\Sigma_2$ condition of the form $\exists C_D,C_{NC}. \ \ C_0 \trans{*} C_D \trans{*}C_{NC} \land
 \forall C_{ZM}. \ \ C_D \trans{*} C_{ZM} \Rightarrow MS(C_{ZM}) \trans{*} C_D'$.
The condition remains in $\Sigma_2$ if we add existential quantifiers $\exists b, C_0$ at the beginning, with the constraints that $b \in \{ 0,1 \}$ and $C_0$ in the intersection of ${I}_b$ and the instances with agent count up to $O(|Q|^k)$.
Thus the all-instance correctness problem for DO protocols is in $\Pi_2$.
 \end{proof}


==> intro-observation-models.tex <==
In the next three sections  we prove that the correctness problem is \PSPACE-complete for IO protocols and $\Pi_2^p$-complete for DO protocols.
%In Proposition \ref{prop:corr} we rephrased the correctness problem (whether a given protocol computes a given predicate) as two twin reachability questions, one for each of the two possible consensus values, $0$ and $1$. Each question is of the form: Given two infinite sets of configurations $\mathcal{C}_1, \mathcal{C}_2$, is some configuration of $\mathcal{C}_2$ reachable from some configuration of $\mathcal{C}_1$? %
These are the most involved results of this paper. They can only be obtained after a detailed study of the reachability problem of IO and DO protocols, which we believe to be of independent interest. The roadmap for the three sections is as follows. 

\medskip\noindent\textbf{Section \ref{sec:reach-obs}.} Section \ref{sec:mfdo} introduces \emph{message-free delayed-ob\-ser\-vation protocols} (MFDO), an auxiliary model very close to DO protocols, but technically more convenient. As its name indicates, agents of MFDO protocols do not communicate by messages. Instead, they directly observe the current \emph{or past} states of other agents. As a consequence, a configuration of an MFDO protocol is completely determined by the states of its agents, which has technical advantages. At the same time, MFDO and DO protocols are very close, in the following sense. We call a configuration of a DO protocol a \emph{zero-message} configuration if all messages sent by the agents have already been received.  Given a DO protocol $\PP$ we can construct an MFDO protocol $\widehat{\PP}$, with the same set of states, such that for any two zero-message configurations $Z, Z'$ of $\PP$, we have $Z \trans{*} Z'$ in $\PP$ if{}f $Z \trans{*} Z'$ in $\widehat{\PP}$. (Observe that, since $\PP$ and $\widehat{\PP}$ have the same set of states, a zero-message configuration of  $\PP$ is also a configuration of $\widehat{\PP}$.) So, any question about the reachability relation between zero-message configurations of $\PP$ can be ``transferred'' to $\widehat{\PP}$, and answered there.

Section \ref{sec:pruning} states and proves the Pruning Theorems for IO and MFDO protocols.
Intuitively, these theorems state that executions starting from configurations with many agents can be ``pruned'', yielding ``equivalent'' executions starting from smaller configurations. The section also proves the Shortening Theorems for MFDO and DO protocols. Loosely speaking,
they state that for every execution $C \trans{*} C'$, there is another execution $C \trans{\xi} C'$ where 
$\xi=t_1^{k_1} t_2^{k_2} \ldots t_m^{k_m}$ for a small number $m$ \emph{independent} from $C$ and $C'$.

\medskip\noindent\textbf{Section \ref{sec:sym-reach-obs}.} This section applies the Pruning and Shortening Theorems to the reachability problem between \emph{counting sets} of configurations. Intuitively, a counting set of configurations is a union of \emph{cubes}, and a cube is the set of all configurations $C$ lying between a lower bound configuration $L$ and an upper bound configuration $U$ with possibly infinite components. Observe  that counting sets may be infinite, but always have a finite representation. The reachability problem for counting sets asks, given two counting sets 
$\mathcal{C}$ and $\mathcal{C}'$, whether some configuration of  $\mathcal{C}'$ is reachable from some configuration of $\mathcal{C}'$.  
The section proves two very powerful Closure Theorems for IO and DO. The Closure Theorems state that for every counting set $\mathcal{C}$,
 the set $\poststar(\mathcal{C})$ of all configurations reachable from $\mathcal{C}$ is also a counting set; further, the same holds for the set $\prestar(\mathcal{C})$ of all configurations from which $\mathcal{C}$ can be reached. So, loosely speaking, counting sets are closed under reachability. 
Furthermore, the section shows that if $\mathcal{C}$ has a representation with ``small'' cubes, in a sense to be determined, then so do $\prestar(\mathcal{C})$ and $\poststar(\mathcal{C})$.

\medskip\noindent\textbf{Section \ref{sec:coNP}.} This section applies the Pruning, Shortening, and Closure Theorems to prove the \PSPACE \  and $\Pi_2^p$ upper bounds for the correctness problems of IO and DO protocols, respectively. The section shows that this is also the complexity of the single-instance correctness problems. 

%Recall that a delayed observation protocol (respectively an immediate observation protocol) is a tuple $(Q,M,\delta_s,\delta_r,\Sigma, \iota, o)$ (resp. $(Q,\delta,\Sigma, \iota, o)$).

\medskip
\medskip\noindent\textbf{Notation.}Throughout these sections, the last three components of the tuples describing protocols (input symbol set $\Sigma$, initial set mapping $\iota$, and output mapping $o$) play no role.
Therefore we represent a DO protocol by the simplified tuple $(Q,M,\delta_s,\delta_r)$, and an IO protocol as just a pair $(Q,\delta)$.


==> io-correctness-sans-reachability.tex <==
Proposition \ref{prop:wellspecification} predicatetes the problem of correctness of an IO protocol as a predicate with boolean and reachability operators over counting sets.
We use the results of Section \ref{sec:small-instance} to show that we only need to examine ``small" configurations to verify this predicate, thus yielding a \PSPACE \ algorithm for checking correctness.

\begin{theorem}
\label{thm:pspace-io-correctness}
The correctness problem for IO protocols is solvable in \PSPACE.
\end{theorem}
%
\begin{proof}
Let $\PP=(Q,\delta,\Sigma, \iota, o)$ be an IO protocol, and $\varphi$ a predicate over $\pop{\sigma}$.
The fairness condition ensures that if a configuration can always reach a set of configurations along an execution, it will reach it infinitely often.
Once the set of stable consensuses $\Stab{b}$ is reached by an execution, this execution can only reach $b$-consensuses afterwards, by definition of stable consensuses.
Because of this, and by Proposition \ref{prop:wellspecification}, the problem of correctness for $(\PP, \varphi)$ can be expressed as checking if  
\begin{equation}
\label{correct}
\poststar({I}_{b}) \cap \compl{\prestar(\Stab{b} )} = \emptyset.
\end{equation}
for $b \in \{ 0,1 \}$.

Recall Definition \ref{def:consensusandco}: for $b \in \{0,1\}$, we call \(\Stab{b}\) the stable consensus configurations given by \(\compl{ \prestar( \compl{ \Cons{b} } ) }\), where $\Cons{b}$ is the configurations in consensus $b$. 
The set $\Cons{b}$ is given by the cube defined by the upper bound equal to $0$ on all states $q_i\in O^{-1}(1-b)$ and $\infty$ otherwise, and the lower bound equal to $0$ everywhere.
By Proposition \ref{prop:oponconf} and Theorem \ref{thm:ccreach-io}, $\Stab{b}$ is a counting set of polynomial norm.
Since $\varphi$ is a predicate representable by a counting constraint, ${I}_b$ is either this counting constraint or the counting constraint corresponding to $1-\varphi$.
Hence ${I}_{b}$ is a counting set of polynomial norm, and so is $\poststar({I}_{b}) \cap \compl{\prestar(\Stab{b} )}$.

Therefore, $\poststar({I}_{b}) \cap \compl{\prestar(\Stab{b} )} \ne \emptyset$ holds
if and only if there is a “small” configuration $C$ in the intersection, of size $|C|$ bounded by the polynomial norm of $\poststar({I}_{b}) \cap \compl{\prestar(\Stab{b} )}$. 
We guess a configuration $C$ of this size.
By unfolding (\ref{correct}), we obtain that $C$ is in the intersection if and only if it verifies the following specification:
\begin{equation*}
\exists I \in I_b \ . \ I \trans{*} C \land \forall X\ . \ C \trans{*} X \Rightarrow (\forall Y\ . \ X \trans{*} Y \Rightarrow Y \in \Cons{b})
\end{equation*}
where $\trans{*}$ is the reachability relation in our IO protocol.
Notice that all the configurations in this predicate have the same agent count as $C$.
We check the reachability predicates of the form $x\trans{*} y$ by guessing an execution step by step leading from $x$ to $y$. 
This can be performed in polynomial space because each configuration along the path is of size \(|C|\), and we only need to store the current configuration to check if it is equal to the final configuration $y$.
This gives us our \PSPACE{} decision procedure, using that $\PSPACE=\NPSPACE$ by Savitch's Theorem.
%The \PSPACE{} decision procedure takes the following steps:
%\textsf{\textbf{1)}}    Guess a “small” configuration $C \in S$.
%\textsf{\textbf{2)}}  Check that \(C\) belongs to \(\poststar(S_0)\).
%
%The algorithm for \textsf{\textbf{2)}} is to guess a configuration \(C_0 \in S_0\) such that \(|C_0|=|C|\), and then guess a run  (step by step), leading from \(C_0\) to $C$. 
%This can be performed in polynomial space because each configuration along the path is of size \(|C|\), and we only need to store the current configuration to check if it is equal to \(C\).
 \end{proof}

\begin{remark}
The same proof idea also shows that the problem of reachability between two counting sets in IO protocols is in \PSPACE.
\end{remark}


==> io-correctness.tex <==
We use the results of Section \ref{sec:small-instance} to show that we only need to examine ``small" configurations to verify reachability between counting sets.
Thus we prove that the cube-reachability problem for IO protocols is in \PSPACE, and then that the correctness problem is too.

\begin{theorem}
\label{thm:set-seteasy}
Cube-reachability for IO protocols is solvable in \PSPACE.
\end{theorem}
%
\begin{proof}
Let $\PP$ be an IO protocol with set of states $Q$, and let $S_0$ and $S$ be cubes.
Some configuration of $S$ is reachable from some configuration of $S_0$ if{}f $\poststar(S_0) \cap S \neq \emptyset$. 
Let $\Gamma_0$ and $\Gamma$ be two counting constraints for $S_0$ and $S$ respectively.
By Theorem~\ref{thm:ccreach-io}  and Proposition~\ref{prop:oponconf}, there exists a counting constraint $\Gamma'$ such that $\sem{\Gamma'}=\poststar(S_0) \cap S$, and such that $\unorm{\Gamma'} \leq \unorm{\Gamma_0} + \unorm{\Gamma}$ and $\lnorm{\Gamma'} \leq \lnorm{\Gamma_0} + |Q|^3 + \lnorm{\Gamma}$.
Therefore, $\poststar(S_0) \cap S \ne \emptyset$ holds
if{}f \(\poststar(S_0) \cap S\) contains a  “small” configuration $C$ satisfying \(|C| \leq  \lnorm{\Gamma_0} +  |Q|^3 + \lnorm{\Gamma} \). 
The \PSPACE{} decision procedure takes the following steps:
\textsf{\textbf{1)}}    Guess a “small” configuration $C \in S$.
\textsf{\textbf{2)}}  Check that \(C\) belongs to \(\poststar(S_0)\).

The algorithm for \textsf{\textbf{2)}} is to guess a configuration \(C_0 \in S_0\) such that \(|C_0|=|C|\), and then guess a run  (step by step), leading from \(C_0\) to $C$. 
This can be performed in polynomial space because each configuration along the path is of size \(|C|\), and we only need to store the current configuration to check if it is equal to \(C\).
 \end{proof}

Notice that cube-reachability can be extended to counting set reachability simply by virtue of a counting set being a finite union of cubes.
Using Proposition \ref{prop:wellspecification}, which predicatetes the problem of correctness as a counting set reachability problem, and  the above result on counting set reachability being solvable in \PSPACE, we show that the correctness problem for IO protocols is solvable in \PSPACE.

\begin{theorem}
\label{thm:pspace-io-correctness}
The correctness problem for IO protocols is solvable in \PSPACE.
\end{theorem}
%
%
\begin{proof}
Let $\PP=(Q,\delta,\Sigma, \iota, o)$ be an IO protocol, and $\varphi$ a predicate over $\pop{\sigma}$.
The fairness condition ensures that if a configuration can always reach a set of configurations along a run, it will reach it infinitely often.
Once the set of stable consensuses $\Stab{b}$ is reached by a run, this run can only reach $b$-consensuses afterwards, by definition of stable consensuses.
Because of this, and by Proposition \ref{prop:wellspecification}, the problem of correctness for $(\PP, \varphi)$ can be expressed as checking if  
\begin{equation}
\label{correct}
\poststar({I}_{b}) \cap \compl{\prestar(\Stab{b} )} = \emptyset.
\end{equation}
for $b \in \{ 0,1 \}$.

Deciding (\ref{correct}) is equivalent to deciding whether $\compl{\prestar(\Stab{b} )}$ is reachable from ${I}_{b}$.
Recall Definition \ref{def:consensusandco}: for $b \in \{0,1\}$, we call \(\Stab{b}\) the stable consensus configurations given by \(\compl{ \prestar( \compl{ \Cons{b} } ) }\), where $\Cons{b}$ is the configurations in consensus $b$. 
The set $\Cons{b}$ is given by the cube defined by the upper bound equal to $0$ on all states $q_i\in O^{-1}(1-b)$ and $\infty$ otherwise, and the lower bound equal to $0$ everywhere.
By Proposition \ref{prop:oponconf} and Theorem \ref{thm:reachofcc}, $\Stab{b}$ is a counting set of polynomial norm.
Since $\varphi$ is a predicate representable by a counting constraint, ${I}_b$ is either this counting constraint or the counting constraint corresponding to $1-\varphi$.
So by Theorem \ref{thm:set-seteasy} this reachability problem can be solved in \PSPACE.
 \end{proof}


==> io-pruning.tex <==
As before, we show that the class of well-structured and realizable histories is sufficient for describing all the runs for IO protocols.
Then we show that any run can be replaced by a smaller (in the number of agents) run, by generalizing the pruning technique to IO protocols.
IO protocols are more expressive then MFDO ones, and well-structured histories are less easily compatible with an IO run (we need more than just having states be \emph{first} visited at an early enough moment).
Because of this, the Pruning Theorem for IO protocols is less powerful than the MFDO pruning result, and we do not present a shortening result.

\begin{restatable}{lemma}{LemmaRealizableIO}
\label{lem:realizable-io}
Let $\PP$ be an IO protocol.
Then $C \trans{*} C'$ if{}f there exists a well-structured history realizable in $\PP$ with $C$ and $C'$ as initial and final configurations.
\end{restatable}

We now proceed to give a syntactic characterization of the well-structured realizable histories. 

\begin{definition}
$H$ is \emph{compatible with IO protocol $\PP$}
if for every trajectory $\tau$ of $H$ and for every non-horizontal step $\tau(i)\tau(i+1)$ of $\tau$, 
the protocol $\PP$ contains a transition $\tau(i) \trans{o} \tau(i+1)$ for some state $o$
and $H$ contains a trajectory $\tau'$ with $\tau'(i)=\tau'(i+1)=o$.
\end{definition}

\begin{restatable}{lemma}{LemmaHistoryIO}
\label{lem:compatible-io}
Let $\PP$ be an IO protocol. A well-structured history is realizable in $\PP$ if{}f it is compatible with $\PP$.
\end{restatable}

The pruning technique is a little more involved for IO protocols than for MFDO protocols. 
We introduce the notion of bunches of trajectories, then present an intermediary lemma about pruning bunches. 
Finally, we prove the IO Pruning Theorem.

\begin{definition}
 A \emph{bunch} is a multiset of trajectories with the same length and the same initial and final state. 
\end{definition}

We show that every well-structured realizable history containing a bunch of size larger than $|Q|$ can be ``pruned'', meaning that the bunch can be replaced by a smaller one, while keeping the history well-structured and realizable.

\begin{lemma}
\label{lm:pruning}
Let $\PP$ be an IO protocol. Let $H$ be a well-structured history realizable in $\PP$ containing a bunch $B\subseteq H$ of size larger than $|Q|$. There exists a nonempty bunch $B'$ of size at most $|Q|$ with the same initial and final
states as $B$, such that the history $H' \defeq H - B + B'$ (where $+, -$ denote multiset addition and subtraction) is also well-structured and realizable in $\PP$.
\end{lemma}
%
\begin{proof}
Let $Q_B$ be a set of all states visited by at least one trajectory in the bunch $B$.
        For every $q\in Q_B$ let $f(q)$ and $l(q)$ be the earliest and the latest
        moment in time when this state has been used by any of the trajectories
        (the first and the last occurrence can be in different trajectories).

        Let $\tau_q, q\in Q_B$ be a trajectory that first goes to $q$ by the moment $f(q)$, then
        waits there until $l(q)$, then goes from $q$ to the final state.
        To go to and from $q$ it uses fragments of trajectories of $B$.

        We will take $B'=\{\tau_q\mid q\in Q_B\}$ and prove that replacing $B$ with $B'$ in $H$
        does not violate the requirements for being a well-structured history realizable in $\PP$.
        Note that we can copy the same fragment of
        a trajectory multiple times.

        First let us check the well-structuring condition. Note that we build $\tau_q$ by taking fragments
        of existing trajectories and using them at the exact same moments in time, and by adding some
        horizontal fragments. Therefore, the set of non-horizontal steps in $B'$ is a subset (if
        we ignore multiplicity) of the set of non-horizontal steps in $B$, and the replacement
        operation cannot increase the set of non-horizontal steps occurring in $H$.

        Now let us check compatibility with $\PP$. 
       % Let us prove that all the non-horizontal steps in $H'$ are still enabled after pruning. 
        Consider any non-horizontal step in $H'$ in any trajectory at position $(i,i+1)$. By construction, the same step at the same position is also present in $H$. History $H$ is realizable in $\PP$ and thus by Lemma \ref{lem:compatible-io} it is compatible with $\PP$, so $H$ contains an enabling horizontal step $o o$ in some trajectory at that position $(i,i+1)$. There are two cases: either that step $o o$ was provided by a bunch being pruned, or by a bunch not affected by pruning. In the first case, note that the state $o$ of this horizontal step must be first observed no later than $j$, and last observed not earlier than $j+1$. This implies $f(o)\leq i<i+1\leq l(o)$. As $H'$ contains a horizontal step $o o$ for all positions between $f(o)$ and $l(o)$, in particular it contains it at position $(i,i+1)$. In the second case the same horizontal step is present in $H'$ as a part of the same trajectory. 
       
       So $H'$ is well-structured and compatible with $\PP$, and thus by Lemma \ref{lem:compatible-io} realizable in $\PP$.
 \end{proof}

Using Lemma \ref{lm:pruning} we can now prove the Pruning Theorem for IO protocols:

\begin{theorem} [IO Pruning]
\label{thm:pruning}
Let $\PP$ be an IO protocol, let $C$ be a configuration of $\PP$, and let
$C'' \trans{*} C'$ be a run of $\PP$ such that $C' \geq C$.
There exist configurations $D''$ and $D'$ such that 
\begin{center}
\(
\begin{array}[b]{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
C'' &  \trans{\hspace{1em}*\hspace{1em}} & C' & \  \geq \ &C  \\[0.1cm]
\geq &  & \geq \\[0.1cm]
D'' & \trans{\hspace{1em}*\hspace{1em}} &D'  & \geq  & C
\end{array}
\)
\end{center}
and $|D''| \leq |C| + |Q|^3$.
\end{theorem}
%
\begin{proof}
Let $C'' \trans{*}  C'  \  \geq  \ C$. 
By Lemma \ref{lem:realizable-io}, there is a well-structured realizable history $H$ with $C''$ and $C'$ as initial and final configurations, respectively. Let $H_C \subset H$ be an arbitrary sub(multi)set of $H$ with final
configuration $C$, and define $H'=H-H_C$. Further, for every $p, p' \in Q$, let $H'_{p,p'}$ be the bunch of all trajectories of $H'$ with $p$ and $p'$ as initial and final states, respectively. We have
$$H' = \sum_{p,p' \in Q} H'_{p,p'}$$

So $H'$ is the union of $|Q|^2$ (possibly empty) bunches. Apply Lemma \ref{lm:pruning} to each bunch of $H'$ with more than $|Q|$ trajectories yields a new history

$$H'' = \sum_{p,p' \in p} H''_{p,p'}$$

\noindent such that $|H''_{p,p'}| \leq |Q|$ for every $p, p' \in Q$, and such that the history $H'' + H_C$ is well-structured and realizable. 

Let $D''$ and $D'$ be the initial and final configurations of $H'' + H_C$. We show that $D''$ and $D'$ satisfy the required properties:
\begin{itemize}
\item $D'' \trans{*} D'$, because  $H'' + H_C$ is well-structured and realizable.
\item $D' \geq C$, because $H_C \subseteq H'' + H_C$. 
\item $|D''| \leq |C| + |Q|^3$ because $|H'' + H_C| = \sum_{p', p} |H''_{p,p'}| + |H_C| \leq |Q|^2 \cdot |Q| + |C| = |C| + |Q|^3$.
\end{itemize}
This concludes the proof.
 \end{proof}


==> io-single-instance-well-specification.tex <==
Using the counting constraints defined above, and a intermediary result generalizing Lemma \ref{lm:smallminterm} to IO protocols, we arrive at a theorem similar to Theorem \ref{thm:reachofcc} that says that the reachability set of a counting set in an IO protocol is still a counting set. 
Using this, we show that reachability in IO protocols is \PSPACE-complete, whether it be between single configurations or cubes (and so also unions of cubes, \ie counting sets).
We then reduce the correctness problem for IO protocols to a reachability question.

\begin{restatable}{lemma}{LemmaSmallCubeIO}
Let $(L,U)$ be a cube of an IO protocol $\PP$ of state set $Q$.
For all $C' \in \prestar(L,U)$, there exists a cube $(L',U')$ such that 
\begin{enumerate}
\item $C' \in (L',U') \subseteq  \prestar(L,U)$, and
\item $\lnorm{(L',U')} \leq \lnorm{(L,U)}  + |Q|^3$ and $\unorm{(L',U')} \leq \unorm{(L,U)}$.
\end{enumerate}
\end{restatable}

\begin{restatable}{theorem}{ThmCCReachabilityIO}
\label{thm:ccreach-io} 
Let $\PP$ be an IO protocol with a set $Q$ of states, and let $S$ be a counting set.
Then $pre^*(S)$ is a counting set and there exist counting constraints $\Gamma$ and $\Gamma'$ satisfying $\sem{\Gamma} = S$, $\sem{\Gamma'} = \prestar(S)$ and we can bound the norm of $\Gamma'$ by
 \begin{align*}
\unorm{\Gamma'} \leq \unorm{\Gamma} \text{ and }
\lnorm{\Gamma'} \leq  \lnorm{\Gamma} + |Q|^3
 \end{align*}
The same holds for $\poststar$ by using the protocol with reversed transitions.
\end{restatable}

We prove that the cube-reachability problem for IO protocols is in \PSPACE.

\begin{theorem}
\label{thm:set-seteasy}
Cube-reachability for IO protocols is solvable in \PSPACE.
\end{theorem}
%
\begin{proof}
Let $\PP$ be an IO protocol with set of states $Q$, and let $S_0$ and $S$ be cubes.
Some configuration of $S$ is reachable from some configuration of $S_0$ if{}f $\poststar(S_0) \cap S \neq \emptyset$. 
Let $\Gamma_0$ and $\Gamma$ be two counting constraints for $S_0$ and $S$ respectively.
By Theorem~\ref{thm:ccreach-io}  and Proposition~\ref{prop:oponconf}, there exists a counting constraint $\Gamma'$ such that $\sem{\Gamma'}=\poststar(S_0) \cap S$, and such that $\unorm{\Gamma'} \leq \unorm{\Gamma_0} + \unorm{\Gamma}$ and $\lnorm{\Gamma'} \leq \lnorm{\Gamma_0} + |Q|^3 + \lnorm{\Gamma}$.
Therefore, $\poststar(S_0) \cap S \ne \emptyset$ holds
if{}f \(\poststar(S_0) \cap S\) contains a  “small” configuration $C$ satisfying \(|C| \leq  \lnorm{\Gamma_0} +  |Q|^3 + \lnorm{\Gamma} \). 
The \PSPACE{} decision procedure takes the following steps:
\textsf{\textbf{1)}}    Guess a “small” configuration $C \in S$.
\textsf{\textbf{2)}}  Check that \(C\) belongs to \(\poststar(S_0)\).

The algorithm for \textsf{\textbf{2)}} is to guess a configuration \(C_0 \in S_0\) such that \(|C_0|=|C|\), and then guess a run  (step by step), leading from \(C_0\) to $C$. 
This can be performed in polynomial space because each configuration along the path is of size \(|C|\), and we only need to store the current configuration to check if it is equal to \(C\).
 \end{proof}

Notice that cube-reachability can be extended to counting set-reachability simply by virtue of a counting set being a finite union of cubes.

\begin{theorem}
Single-instance correctness of IO protocols is solvable in \PSPACE.
\end{theorem}
%
\begin{proof}
Let $\PP=(Q,\delta,\Sigma, \iota, o)$ be an IO protocol, $\varphi$ a predicate over $\pop{\sigma}$, and $C_0$ an initial configuration of ${I}_b$ (defined in Definition \ref{def:initial-configurations}). 
Recall Definition \ref{def:consensusandco}: for $b \in \{0,1\}$, we call \(\Stab{b}\) the stable consensus configurations given by \(\compl{ \prestar( \compl{ \Cons{b} } ) }\), where $\Cons{b}$ is the configurations in consensus $b$. 
The set $\Cons{b}$ is given by the cube defined by the upper bound equal to $0$ on all states $q_i\in O^{-1}(1-b)$ and $\infty$ otherwise, and the lower bound equal to $0$ everywhere.
The fairness condition ensures that if a configuration can always reach a set of configurations along a run, it will reach it infinitely often.
Once the set of stable consensuses $\Stab{b}$ is reached by a run, this run can only reach $b$-consensuses afterwards, by definition of stable consensuses.
Because of this, and similarly to Proposition \ref{prop:wellspecification}, the problem of single-instance correctness for $(\PP, \varphi, C_0)$ can be expressed as checking if  
\begin{equation}
\label{correct}
\poststar(C_0)\cap \compl{\prestar(\Stab{b})} = \emptyset.
\end{equation}
%prove this?
for $b$ such that $C_0 \in {I}_b$.

Deciding (\ref{correct}) is equivalent to deciding whether $\compl{\prestar(\Stab{b} )}$ is reachable from $\{ C_0 \}$.
Sets $\{ C_0 \}$ and $\compl{\prestar(\Stab{b} )}$ are counting sets, because reachability sets and boolean combinations of counting sets remain counting sets.
To solve the single-instance well-specification for $(\PP, \varphi, C_0)$, we simply apply the \PSPACE \ procedure for counting set reachability in IO protocols.
 \end{proof}



==> io-well-specification.tex <==
Using Proposition \ref{prop:wellspecification}, which predicatetes the problem of correctness as a counting set reachability problem, and  the above result on counting-set reachability being solvable in \PSPACE, we show that the correctness problem for IO protocols is solvable in \PSPACE.
\begin{theorem}
The correctness problem for IO protocols is solvable in \PSPACE.
\end{theorem}


==> message-based.tex <==
In delayed delivery models agents communicate by sending and receiving messages. The set of messages that can be sent (and received) is finite. Messages are sent to and received from one 
single pool of messages; in particular, the sender does not choose the recipient of the message.
Agents update their state after sending or receiving a message. Angluin \etal define \cite{AAER07} three delayed delivery models. 

\paragraph{Queued Transmission Protocols (QT).}  The set of messages an agent is willing to receive depends on its current state. In particular, in some states the agent may not be willing to receive any message.

\begin{definition}
\label{def:queued-transmission}
A \emph{queued transmission protocol} is a septuple $\PP=(Q,M,\delta_s,\delta_r,\Sigma, \iota, o)$ where 
$Q$ is a finite set of states, 
$M$ is a finite set of messages,
$\delta_s \colon Q\rightarrow M\times Q$ is the transition function for sent messages,
$\delta_r \colon Q\times M \rightharpoonup Q$ is the partial transition function for received messages,
$\Sigma$ is a finite set of input symbols,
$\iota \colon \Sigma\rightarrow Q$ is the initial state mapping, and
$o \colon Q\rightarrow \{0,1\}$ is the state output mapping.
\end{definition}

Every queued transmission protocol determines a protocol in the sense of Definition \ref{def:unified} as follows, where $C, C' \in \pop{Q}$, $M \in \pop{\Sigma}$, and $b \in \{0,1\}$:
\begin{itemize}
\item  the configurations are the non-empty populations over of $Q\cup M$, \ie $\Conf = \pop{Q\cup M}$; 
\item $(C, C') \in \Step$ if there exist states $q_1,q_2$ and a message $m$ such that
	\subitem $\delta_s(q_1)= (m,q_2)$, $C(q_1)>0$, and $C'=C-q_1+q_2+m$; or
	\subitem $\delta_r(q_1,m)= q_2$, $C'(q_1)>0$, $C'(m)>0$, and $C=C'-q_1-m+q_2$.
\item $I(C)=\sum_{\sigma \in \Sigma} C(\sigma)\iota(\sigma)$;
\item $O(C)=b$ if $o(q)=b$ for all $q$ such that $C(q)>0$.
\end{itemize}

%Angluin \etal prove this model also computes exactly the predicates of Presburger arithmetic \cite{AAER07}.

%Among the one-way protocols we investigate in this article, the delayed transmission and delayed  observation protocols are message based protocols with supplementary conditions on the transitions functions in comparison to the queued transmission protocol.

%\begin{remark}
%In the Angluin \etal paper, the set of transitions is defined by a transition function and so the steps are deterministic. 
%We keep this determinism. 
%\end{remark}

\paragraph{Delayed Transmission Protocols (DT).}
DT-protocols are the subclass of QT-protocols in which, loosely speaking, agents can never refuse to receive a message. This is modeled by requiring the receive transition function to be total. 

\begin{definition}
\label{def:queued-transmission}
A queued transmission protocol $\PP=(Q,M,\delta_s,\delta_r,\Sigma, \iota, o)$ is a \emph{delayed transmission protocol} if $\delta_r \colon Q\times M \rightharpoonup Q$ is a total function. 
\end{definition}

\paragraph{Delayed Observation Protocols (DO).}

Intuitively, DO-protocols are the subclass of DT-protocols in which ``sender'' and ``receiver'' actually means ``observee'' and ``observer''. This is modeled by forbidding the sender to change its state when it sends a message (since the observee many not even know it is being observed).

\begin{definition}
\label{def:queued-transmission}
A queued transmission protocol $\PP=(Q,M,\delta_s,\delta_r,\Sigma, \iota, o)$ is a \emph{delayed observation protocol} if $\delta_r \colon Q\times M \rightharpoonup Q$ is a total function and 
for every $q \in Q$ the funtion $\delta_s$ satisfies $\delta_s(q)=(q,m)$ for some $m\in M$.
\end{definition}



==> mfdo-correctness.tex <==
We show that the correctness problem for DO protocols is in $\Pi_2$ by using the results of Section \ref{sec:small-instance}.
These imply that we only need to check that there does not exists a ``small" initial configuration that is \emph{not} correct. 
We prove that checking non-correctness of a single instance is in $\Sigma_2$ for DO protocols.
% and for this proof we need to also examine the single-instance non-correctness problem for MFDO protocols, which we prove to be a \NP \ problem.

Recall the single-instance non-correctness problem: given a protocol $\PP$ over an alphabet $\Sigma$ with initial state mapping $\iota$, a quantifier-free Presburger predicate $\varphi$ over $\Sigma$ and an initial configuration $C_0 \in {I}_b$,
does there exist a fair execution starting in $C_0$ that does not converge to $b$ ?
%
%\begin{theorem}
% \label{thm:single-correctness-do-mfdo}
% Single-instance non-correctness of MFDO protocols is solvable in \NP.
% \end{theorem}
% %
% \begin{proof}
% Let $\PP=(Q,\delta,\Sigma, \iota, o)$ be an MFDO protocol, $\varphi$ a predicate over $\pop{\Sigma}$ and $C_0$ a configuration of ${I}_b$. 
% We want to show that the problem of checking whether instance $(\PP , \varphi , C_0)$ is \emph{not} correct is in \NP.
% To do this we show that a witness $\pi$ of non-correctness is checkable in PTIME.
%We let $\pi$ be a (possibly infinite) fair run $\pi=C_0C_1C_2\ldots$ such that there exists no indice $j\geq 0$ such that $C_j \in \Stab{b}$, where $\Stab{b}$ is the set of stable $b$-consensus configurations.
%
%We use Theorem \ref{thm:mfdoshortening} to prove that we can consider only fair runs that can be described in \PSPACE.
%Indeed consider a (possibly infinite) fair run $\pi=C_0C_1C_2\ldots$. 
%We can equivalently consider the extended run $(C_0,\seen_0)(C_1,\seen_1)(C_2,\seen_2)\ldots$ of minimal seen sets $\mathcal{S}_i =\{ q| \exists j\leq i \ . \ C_j(q)\geq 1\}$, which we abusively also note $\pi$.
%Let $\seen$ be the set of states that are visited by agents of this run, \ie the maximal seen set of $\pi$.
%This set is finite as it is included in $Q$, and the seen sets can only grow over the length of the run.
%Therefore there is only a finite number of transitions before all the states of $\seen$ have been visited by agents of $\pi$, and we call $k$ the first index such that this is true.
%
%The agents of the run then move independently through the graph of allowed transitions given the seen set $\seen$.
%That is, the graph whose nodes are the states of the protocol, and whose directed arcs are the transitions enabled in the protocol when the seen set is $\seen$.
%%[Something about the size of this reachability graph, to prove PTIME checking]
%We call bottom strongly connected component (BSCC) of the graph a maximal set of mutually reachable configurations closed under reachability.
%The BSCCs of this graph can be computed in polynomial time in the size of the graph, so also in the size of the protocol. 
%We mark the BSCCs of the graph such that all the states of the BSCC have output $b$, and call the resulting structure the \emph{marked graph}.
%
%Because the run we consider is fair and the number of agents does not change, there is a only a finite number of transitions between $C_k$ and the moment in which all the agents of $\pi$ reach  BSCCs of the marked graph. 
%Let us call $C$ the configuration in $\pi$ at this moment. 
%If we apply Theorem \ref{thm:mfdoshortening} to the prefix of $\pi$ ending in $C$, we can replace it with a "shorter" prefix from $(C_0,\seen_0)$ to $(C,\seen)$. 
%This new prefix is of the form $t_1^{k_1} t_2^{k_2} \ldots t_n^{k_n}$, with $n\leq |C_0||Q|^3$.
%Let us note $\pi'$ the run that starts in $C_0$, uses this new prefix till $C$, then reuses the transitions of $\pi$.
%If $\pi$ is such that there exists no indice $j\geq 0$ such that $C_j \in \Stab{b}$, then this is still the case for $\pi'$.
%And $\pi'$ is still fair because we just changed a finite prefix of the fair run $\pi$.
%
%Run $\pi'$ is \PSPACE-describable by $(\pi'|_C, \seen,M)$ where $\pi'|_C$ is the prefix of $\pi'$ until $(C,\seen)$ (which takes polynomial space in in the input), and $M$ is a multiset over the BSCCs of the marked graph of $\PP$ for seen set $\seen$ describing the number of agents in each BSCC in configuration $C$.
%Any witness run $\pi$ can be turned into a "shorter" run $\pi'$ which can be described by such a "small" triple.
%Checking that a run thus described is a witness for non-correctness is doable in polynomial time: we verify that the prefix is indeed a run, calculate the marked graph of $\PP$ for seen set $\seen$, and using $M$ check if all the agents are only in marked BSCCs of the marked graph, \ie the agents remain in $b$-consensuses. 
%%This proves single-instance correctness is a co\NP{} problem for MFDO protocols.
%
%%Let $\pi$ be a witness fair run of the non-correctness of instance $(\PP , \varphi , C_0)$ for $\PP=(Q,M,\delta_s, \delta_r,\Sigma, \iota, o)$ a DO protocol.
%%By Lemma \ref{lm:do-to-mfdo}, we can transform any finite run of a DO protocol $\PP$ to a run in the corresponding MFDO protocol of Definition \ref{def:corresponding-mfdo}.
%%As above this run $\pi$ can be described by a \PSPACE-describable triple $(\pi', \seen,M)$.
%%The prefix $\pi'$ can be reconverted to a DO run.
%%Set $\seen$ describes the seen set but also equivalently the messages sent in this case, as we assume in our run conversion that "enough" messages are sent once the state sending them is visited.
%%         \mr{What is enough? It might be that the configuration switches the output until it runs out of some kind of messages, then stabilises.}
%%         So similarly we have single-instance correctness is a co\NP{} problem for DO protocols.
%  \end{proof}
 
\begin{remark}
\label{rmk:zeromessage}
Any configuration of a DO protocol can always reach some zero-message configuration: since the message receiving transition function is total, all the messages can be received by the agents of the configuration, thus resulting in some new configuration with zero messages.
\end{remark}
 
%Now, before showing that the same problem is in $\Sigma_2$ for DO protocols, 
We introduce a procedure on zero-message DO configurations called \emph{message saturation}:

Consider a configuration $C \in \N^{Q \cup M}$ such that $C(m)=0$ for all $m \in M$, and let $n$ be $|C|$ the number of agents in $C$.
For every populated state $q \in Q$ in $C$, let one of the agents in $q$ send $n|Q|+|Q|^2$ messages $\delta_s(q)$.
As long as there are reachable states $q$ that have not yet sent $n|Q|+|Q|^2$ messages, let an agent go there by a shortest path (which is of length at most $|Q|-1$, see proof of Theorem \ref{thm:mfdoshortening}) and let the agent send $n|Q|+|Q|^2$ messages $\delta_s(q)$.
Since at most $|Q| \times |Q|$ messages are consumed to reach new message-sending states, the resulting configuration $MS(C)$ has at least $n |Q|$ messages of each represented type, and no state emitting other message types is reachable.
Note that we always have $C \trans{*} MS(C)$.
 
 \begin{theorem}
  \label{thm:single-correctness-do}
 Single-instance non-correctness of DO protocols is solvable in $\Sigma_2$.
 \end{theorem}
 %
 \begin{proof}
Let $\PP=(Q,M,\delta_r, \delta_s,\Sigma, \iota, o)$ be a DO protocol, $\varphi$ a predicate over $\pop{\Sigma}$ and $C_0$ a configuration of ${I}_b$. 
 We want to show that the problem of checking whether instance $(\PP , \varphi , C_0)$ is \emph{not} correct is in $\Sigma_2$. To do this we give a condition in $\Sigma_2$ and prove that $(\PP,\varphi,C_0)$ is incorrect if and only if the condition holds.
 
 Consider the following condition
 \begin{align*}
 &\exists C_D,C_{NC}. \ C_0 \trans{*} C_D \trans{*}C_{NC} \text{ and } \\
 &\forall C_{ZM}. \ C_D \trans{*} C_{ZM} \Rightarrow [ \ \exists C_D'. \ MS(C_{ZM}) \trans{*} C_D' \ ]
 \end{align*}
 where $C_D$ is a zero-message configuration, $C_{NC}$ contains at least one agent with opinion $1-b$, the $C_{ZM}$ are zero-message and $C_D'$ is equal to $C_D$ over $\N^Q$ but may contain messages.
 
Suppose the condition holds. 
If a stable consensus configuration $C_{SC}$ is reachable from the ``deadend" configuration $C_D$, then we can reach a zero-message configuration $C_{ZM}$ from $C_{SC}$, as described in Remark \ref{rmk:zeromessage}.
We then apply the message-saturation procedure to get $MS(C_{ZM})$ and from there reach some $C_D'$ equal to $C_D$ on $\N^Q$.
From there we can reach $C_{NC}'$ equal to $C_{NC}$ on $\N^Q$ following the same transition sequence as from to $C_D$ to $C_{NC}$ (a few extra messages change nothing).
Like configuration $C_{NC}$, there is an agent in $C_{NC}'$ with opinion $1-b$, thus bringing a contradiction to $C_{SC}$ being a stable consensus.

Suppose the condition does not hold.
By Remark \ref{rmk:zeromessage}, we can always reach a zero-message configuration $C$ from $C_0$.
There is a finite reachability graph on zero-message configurations.
%, and every fair run reaches a BSCC in it 
From $C$, we can always reach a zero-message configuration $C_D$ that is in a bottom strongly connected component (BSCC) of this graph.
It is reachable from all configurations reachable from it.
Since the condition does not hold, no configuration with an agent of opinion $1-b$ is reachable from it, and so it is a stable $b$-consensus.

Now let us justify that the condition is indeed in $\Sigma_2$.
The existential quantification over $C_D,C_{NC}$ include the transition sequences between them and $C_0$.
The universal quantification on $C_{ZM}$ is a universal quantification on all zero-message configurations of same size as $C_D$ and all reachability certificates. 
The latter are reachability certificates between zero-message configurations, which can be seen as reachability between configurations of the corresponding MFDO protocol to our DO protocol by Lemma \ref{lm:do-to-mfdo}.
%As in the proof of Theorem \ref{thm:single-correctness-do-mfdo} these certificates are in \NP.
By Theorem \ref{thm:mfdoshortening}, we can consider only certificates that are polynomial in $|Q|$ and $|C_0|=|C_D|$.
\cwk{more details?}

Finally,  we show that the reachability condition on $MS(C_{ZM})$ does not actually require a new existential quantifier (putting our condition in $\Sigma_3$).
Configuration $MS(C_{ZM})$ has enough messages that it does not need to send new ones to get to any new configuration.
Indeed if an agent can go from $q$ to $q'$ it can go there in $|Q|-1$ receive transitions, and each reachable message exists in the configuration.
So the question of whether $MS(C_{ZM})$ can reach $C_D'$ such that $C_D|_Q = C_D'|_Q$ is only a question of how to transfer all the agents.
To solve this question, we can apply the Edmonds-Karp algorithm to the following graph with capacities:

\begin{itemize} 
\item Let the nodes be $|Q|$ copies of the states of the protocol written $q^{(1)},q^{(2)}, \ldots q^{(|Q|)}$ for each $q \in Q$, a source node $s$, and a target node $t$.

\item Let there be directed arcs from $s$ to each $q^{(1)}$ with capacity $MS(C_{ZM})(q)$ and from each $q^{(|Q|)}$ to $t$ with capacity $C_D(q)$.

\item For each $i=1,\ldots,|Q|-1$, let there be a directed arc from $q^{(i)}$ to $q'^{(i+1)}$ whenever there is a receive transition from $q$ to $q'$ using a message of $MS(C_{ZM})$ in the protocol, or when $q=q'$. 
These arcs have capacity $\infty$.
\end{itemize} 

If there exists a maximum flow solution to this graph, then it uses a flow of value $\sum_q MS(C_{ZM})(q)= \sum_q C_D(q)$ by construction because there are no inner edges with smaller capacity.
This gives a solution to the reachability problem of whether $MS(C_{ZM})$ can reach a configuration with the same agent distribution as $C_D$.
If there is a transition sequence from $MS(C_{ZM})$ to a configuration with the same agent distribution as $C_D$, then there is a solution in this capacity graph by taking the arcs corresponding to the transitions of the sequence.

\cwk{the graph could also be defined using only two copies of each q. would this be better ?}
%For example, we can enumerate the point-to-point reachability
%in the graph by brute force, then apply Edmonds-Karp algorithm to the graph
%[source — $MS(q)$ capacity — $\uparrow q$ — infinite capacity — $q \downarrow$ — $D(q)$ — target] to
%check if we can match all the agents. \cwk{to be rewritten more clearly}
  \end{proof}

We define a reachability operator $\widetilde{\prestar}$ for DO protocols based on the MFDO $\prestar$ operator.
We then use $\widetilde{\prestar}$ to express a version of Proposition \ref{prop:wellspecification} adapted to DO protocols.

\begin{definition}
Let $\PP$ a DO protocol with state set $Q$.
For any $C \in \N^Q$, we note $C_z$ the corresponding zero-message configuration in $\N^{Q\cup M}$.
Define $\widetilde{\prestar}(C_z)$ as the set of zero-message configurations $C'_z$ such that 
$$
(C',\seen_{C'}) \in \bigcup_{\seen | \seen \supseteq \text{ minimal seen set for } C} \prestar(C,\seen)
$$
where $\seen_{C'}$ is the minimal seen set for $C'$, and the operator $\prestar$ is applied in the MFDO protocol corresponding to DO protocol $\PP$ (see Definition \ref{def:corresponding-mfdo}).
\end{definition}

\begin{restatable}{proposition}{PropDOCharacterization}
\label{prop:do-correctness}
A DO protocol $\PP$ is correct for a predicate $\varphi$ if{}f the following hold for $b\in \set{0,1}$:
$$
{I}_{b} \cap \widetilde{\prestar}(\compl{\widetilde{\prestar}(\widetilde{\Stab{b}} )}) = \emptyset.
$$
where $\widetilde{\Stab{b}}$ is equal to $\compl{\widetilde{\prestar}( \compl{ \Cons{b} } ) }$.
\end{restatable}
%
\begin{proof}
Notice that this intersection is well defined as DO initial configurations are zero-message.
Now we need to argue that reaching zero-message non-$b$-consensus is always possible if we can reach non-$b$-consensus with messages. 
This is true as soon as we have strictly more than one agent, because we can keep one agent that has output $1-b$ and let the other agents consume all the messages, as described in Remark \ref{rmk:zeromessage}. \cwk{is this enough of a proof?}
 \end{proof}

%\begin{lemma}
%        \label{lemma:mfdo-do-non-ws-pruning}
%        If a
%        DO protocol
%        with state set $Q$
%        is not correct for a predicate $\varphi$,
%        then it is not correct on some instance
%        with agent count polynomial in the size of the input, \ie in $|Q|$ and $size(\varphi)$.
%\end{lemma}
%%
%\begin{proof}
%If a protocol is not correct, then there exists, for some $b\in \{0,1\}$ a configuration in ${I}_b$ that does not converge to $b$.
%Let us fix this $b$ for the rest of the proof.
%The result relies on the fact that both $\Stab{b}$ and ${I}_b$ are counting sets with "small" norms relative to the size of the input, \ie $\PP$ and $\varphi$.
%Indeed, recall that $\Stab{b}$ is given by $\compl{ \prestar( \compl{ \Cons{b} } ) }$ where $\Cons{b}$, for $b \in \{ 0,1 \}$, can be represented by the cube defined by the upper bound equal to $0$ on all places $q$ with output $o(q)=1-b$ and $\infty$ otherwise, and the lower bound equal to $0$ everywhere. 
%By Proposition \ref{prop:oponconf} and Theorem \ref{thm:reachofcc}, $\Stab{b}$ is a counting set of polynomial norm.
%Since $\varphi$ is a predicate representable by a counting constraint, ${I}_b$ is either this counting constraint or the counting constraint corresponding to $1-\varphi$.
%
%We are going to consider an expression of correctness similar to the one of  Propostion \ref{prop:wellspecification} as a predicate over sets of configurations, but using a new operator $\widetilde{\prestar}$ over DO configurations that relies on the $\prestar$ operator over MFDO configurations.
%Before defining this new operator, recall that any configuration can always reach some zero-message configuration by Remark \ref{rmk:zeromessage}.
%For $C \in \N^Q$ defining a zero-message configuration of our DO protocol, we define $\widetilde{\prestar}(C)$ as the zero-message configurations $C'$ such that 
%$$
%(C',\seen_{C'}) \in \bigcup_{\seen | \seen \supseteq \text{ minimal seen set for } C} \prestar(C,\seen)
%$$
%where $\seen_{C'}$ is the minimal seen set for $C'$, and the operator $\prestar$ is applied in the MFDO protocol corresponding to our DO protocol (see Definition \ref{def:corresponding-mfdo}).
%
%By Lemma \ref{lm:do-to-mfdo} and the above discussion on zero-message configurations, this operator describes zero-message reachability in our DO protocol (\ie reachability from a configuration with zero messages to another configuration with zero messages).
%By Proposition \ref{prop:oponconf} and Theorem \ref{thm:reachofcc} and the fact that the norm of an extended counting set does not take into account the seen set, the bounds on the number of agents of the minimal configurations in $\widetilde{\prestar}(C)$ are still polynomial in $|Q|$ and $|C|$.
%
%We express correctness as
%\begin{equation*}
%%\label{do-correctness}
%{I}_{b} \cap \widetilde{\prestar}(\compl{\widetilde{\prestar}(\widetilde{\Stab{b}} )}) = \emptyset.
%\end{equation*}
%where $\widetilde{\Stab{b}}$ is equal to $\compl{\widetilde{\prestar}( \compl{ \Cons{b} } ) }$.
%Indeed, DO initial configurations are zero-message.
%Now we need to argue that reaching zero-message non-$b$-consensus is always possible if we can reach non-$b$-consensus with messages. 
%This is true as soon as we have $\geq 2$ agents, because we can keep one agent that has output $1-b$ and let the other agents consume all the messages. 
%
%By the definition of $\widetilde{\prestar}$, the norms on the counting sets describing the agent count of $\widetilde{\prestar}(\compl{\widetilde{\prestar}(\widetilde{\Stab{b}} )})$ are polynomial in the input.
%So if the intersection is non-empty, there exists a (zero-message) configuration in the intersection with polynomial agent count.
% \end{proof}

\begin{theorem}
        The correctness problem for DO
        protocols 
        is in $\Pi_2$.
\end{theorem}
%
\begin{proof}
%By Lemma~\ref{lemma:mfdo-do-non-ws-pruning}, 
%it is enough to verify single-instance correctness for
%all instances with agent count up to $O(|Q|^k)$.
We prove that the non-correctness problem for DO protocols is in $\Sigma_2$.
Let $\PP$ be a DO protocol.
Non-correctness means that there exists
an initial configuration that does not satisfy 
single-instance correctness, and initial configurations are zero-message in DO protocols, \ie completely defined by their agent count.

Let us first show that it is enough to consider only instances with agent count polynomial in the size of the input, \ie $\PP$ and $\varphi$.
Proposition \ref{prop:do-correctness} says that $\PP$ is correct if and only if 
\begin{equation}
\label{eq:do-correctness}
{I}_{b} \cap \widetilde{\prestar}(\compl{\widetilde{\prestar}(\widetilde{\Stab{b}} )}) = \emptyset.
\end{equation}
By Proposition \ref{prop:oponconf} and Theorem \ref{thm:reachofcc} and the fact that the norm of an extended counting set does not take into account the seen set, the bounds on the number of agents of the minimal configurations in $\widetilde{\prestar}(C)$ are polynomial in $|Q|$ and $|C|$.
As in the proof of Theorem \ref{thm:pspace-io-correctness}, $\Stab{b}$ and ${I}_b$ are counting sets with "small" norms relative to the size of the input.
Thus, by definition of $\widetilde{\prestar}$, the norms on the counting sets describing the agent count of $\widetilde{\prestar}(\compl{\widetilde{\prestar}(\widetilde{\Stab{b}} )})$ are polynomial.
So if the intersection of (\ref{eq:do-correctness}) is non-empty, there exists a zero-message initial configuration in the intersection with polynomial agent count.

By Theorem~\ref{thm:single-correctness-do}, single-instance non-correctness over a configuration $C_0$ can be characterized by a $\Sigma_2$ condition of the form $\exists C_D,C_{NC}. \ \ C_0 \trans{*} C_D \trans{*}C_{NC} \land
 \forall C_{ZM}. \ \ C_D \trans{*} C_{ZM} \Rightarrow MS(C_{ZM}) \trans{*} C_D'$.
The condition remains in $\Sigma_2$ if we add existential quantifiers $\exists b, C_0$ at the beginning, with the constraints that $b \in \{ 0,1 \}$ and $C_0$ in the intersection of ${I}_b$ and the instances with polynomial agent count.
Thus the all-instance correctness problem for DO protocols is in $\Pi_2$.
 \end{proof}


==> mfdo-do-hardness.tex <==
We consider the single-instance and the general correctness problems, and prove that they are $\Pi_2^p$-hard for DO protocols.
These results are proved by a reduction using the circuit-satisfiability problem to the non-correctness problem over a single instance,
\ie checking that a single initial configuration of a protocol does not converge to the desired answer.
The circuit satisfiability problem asks, given a boolean circuit, whether there exists
a combination of input values that make the circuit output $1$.
This problem is \NP-complete.
\cwk{make this section more formal (using notations)?}

\begin{definition}
        \label{def:circuit-eval-observation}
        Consider a boolean circuit $C$.
        The \emph{circuit evaluation protocol} for $C$ 
        with output node $o$
        is defined as an DO protocol as follows.
\begin{itemize}
\item Each state contains a node identity
        of the circuit $C$
        (the node can be an input node 
        or an operation node),
        the current value of this node
        (the value can be $0$, $1$ or $\square$ denoting that the 
        value is still unknown),
        the last seen values of the node's arguments
        (unless the node is an input node),
        and the last seen value of the output node.
        
\item Each agent in a state can send a message containing the state's identity and current value.
%        Input nodes can switch from current value $\square$ 
%        to either of the values $0$ and $1$ on observation. %of themselves?
\item An agent in an input state (\ie a state with input node ID) can switch from value $\square$ to value $0$ on observation of itself (\ie on reception of a message with its state identity and current value), or from $\square$ to value $1$ on observation of an agent in the output state (\ie on reception of a message with state identity the output state).
Each agent updates its memory of its arguments' values and the value of the output when it observes agents corresponding to these nodes with non-$\square$ value.
        Operation node agents replace their current value
        with the result of the operation whenever 
        they observe the non-$\square$ value of an argument and 
        know the non-$\square$ values of the other arguments.
        
\item The output function returns the saved value of the output node
        if it is known and $0$ if it is $\square$.
        
\item The input symbols are the (input, operation, and output) nodes of circuit $C$, and the initial state mapping maps a node of $C$ to the state with the the same node identity and with all stored values $\square$.
\end{itemize}
\end{definition}

The following lemma describes the behaviour of the circuit evaluation protocol for a given circuit and a configuration which assigns exactly one agent to each node of the circuit.
%The following lemma states the single-instance correctness of the the circuit evaluation protocol for a given circuit and a configuration which assigns exactly one agent to each node of the circuit.

\begin{lemma}
        \label{lm:circuit-evaluation-correct}
        Consider a circuit evaluation protocol for a circuit $C$, and a configuration with exactly one agent corresponding to each node of $C$.
        A fair run starting in this configuration eventually reaches a configuration where each input node
        has value $0$ or $1$ and these values do not change 
        afterwards.
        Once these values have been assigned, the run eventually converges to a stable
        consensus with the output equal to the value of circuit $C$
        on these assigned inputs.
%        In a fair run, 
%        a circuit evaluation protocol configuration
%        with exactly one agent corresponding to each node of the circuit
%        eventually reaches a configuration where each input node
%        has value $0$ or $1$ and these values do not change 
%        afterwards.
%
%        Each such run eventually converges to a stable
%        consensus with the output equal to the value of the circuit 
%        on the chosen inputs. This is true for the MFDO definition of the circuit evaluation protocol as well as the DO definition.
\end{lemma}

\begin{proof}
Every input node can change its own current value if it is $\square$
and cannot otherwise; by fairness of the run and definition of how an input node can update its $\square$ value, the input nodes will eventually all change their values
from $\square$ and keep these afterwards. 

By induction over the depth of an operation node,
we can see that the value of each operation node eventually converges
        to the value of this node in circuit $C$, without ever holding the opposite value; 
        moreover,
once a node adopts a value, the value stays stable.

Once the output value converges, each node will eventually 
learn it.

The transitions of the circuit evaluation protocol always depend only on current values of nodes, so the DO protocol cannot have a problem with lack of old messages.
%Note that the current value is always suitable for performing the transitions, 
%so the DO protocol cannot have a problem with lack of old messages.
 \end{proof}

\begin{theorem}
Single-instance correctness of DO and MFDO protocols is co\NP-hard.
\end{theorem}
%
\begin{proof}
We prove that circuit satisfiability is polynomial-time reducible
to verification of single-instance incorrectness of MFDO protocols 
for the predicate that answers $0$ on all inputs.
The same is true for DO.

        For any given circuit $C$ 
        we consider the corresponding circuit evaluation
        protocol and the initial configuration
        with exactly one agent per node with all stored values
        being $\square$.
        This protocol can converge to $1$ if the circuit is satisfiable
        and always converges to $0$ otherwise, as 
        by Lemma~\ref{lm:circuit-evaluation-correct} it converges to 
        a correct evaluation of a circuit on some input and an unsatisfiable 
        circuit always outputs $0$.
        
Since circuit satisfiability is \NP-complete, the single-instance correctness of DO and MFDO protocols is co\NP-hard.
 \end{proof}

To prove that the general all-instance correctness problem is also co\NP-hard we need to add to the circuit evaluation protocol construction.
We add an extra failure state $\bot$ with output $0$. 
Each agent representing an input node switches to $\bot$ on observing an agent for the same node with a different non-$\square$ value, and any state switches to $\bot$ on observing $\bot$.
The rest of the construction remains the same, and we refer to this as the \emph{modified} circuit evaluation protocol.

\begin{theorem}
All-instance correctness
 of DO and MFDO protocols is co\NP-hard.
\end{theorem}
%
\begin{proof}
%We do a few minor modifications to 
%the circuit evaluation protocol construction.
%For all-instance correctness problem we should define the 
%set of input states. 
%        We define the input states to be those where all the stored values
%        (the local one, the argument values and the circuit output)
%        are unknown ($\square$).
Given a circuit $C$ we construct the corresponding modified circuit evaluation
protocol, and consider the constant $0$ predicate.
If some node is not represented, the global circuit output
stays $0$ because the circuit output value remains unknown, \ie
%is universally assumed to be 
$\square$.
If some input is represented by multiple agents and they disagree on the input value,
the protocol will eventually converge to the state $\bot$ with the output $0$.
If for each input there is an agreement on its value, the run will converge 
to the value of the circuit.

The only way to avoid converging to $0$ is to have a satisfying assignment 
and choose the corresponding input values. Therefore always converging to $0$ is also equivalent to the (co\NP-hard) circuit satisfiability problem.
 \end{proof}

It turns out that DO protocol correctness is even harder, specifically $\Pi_2$-hard.
This only holds for DO protocols and not for MFDO; the difference is that for a state
that has been visited a finite number of times, a DO protocol eventually consumes all the
messages, thus ``forgetting" that the state was visited. 
An MFDO protocol never forgets a state once visited.

\begin{theorem}
Single-instance and all-instance correctness
 of DO protocols is $\Pi_2^p$-hard.
\end{theorem}

\begin{proof}
%We use the $\Sigma_2^p$-complete problem of $\exists\forall$-truth value.
We proceed by reduction from the satisfiability problem for quantified boolean predicates from the $\exists\forall$ fragment, which is $\Sigma_2^p$-complete.

We encode this problem as a circuit $C$, and a subset of inputs of $C$ that 
are quantified universally (the rest are quantified existentially).
We change the modified circuit evaluation protocol in the following way.
If an agent representing a universally quantified input with known (non-$\square$) current value receives a message from an agent representing the circuit output node with output value $1$, then the first agent can change the current input value from $0$ to $1$ or $1$ to $0$.
Additionally, it is now only agents of \emph{existential} input states with conflicting values that switch to $\bot$ on receiving the state of the other.
This does not apply to agents in \emph{universal} input states.
All agents that receive a message sent by an agent in the $\bot$ state still switch to $\bot$. 
%but now we only allow switching to $\bot$ for conflicting values of existentially quantified input nodes.

Let us first assume the statement $\exists\vect{x}:\forall\vect{y}:C(\vect{x},\vect{y})$ is false.
Then the protocol either lacks the agents for some nodes,
or converges to $\bot$ or eventually converges to a consistent set of values
for existentially quantified inputs.
This specifies some $\vect{x}$; by assumption there is an $\vect{y}$
such that $C(\vect{x},\vect{y})=0$.

Let us prove that we can reach a stable consensus of $0$. 
Let all messages be consumed.
If from the resulting zero-message configuration it is possible to reach a configuration with an agent in 
circuit output $1$, do so. 
Then send enough messages to switch all the agents 
representing universally quantified input nodes into agreement with $\vect{y}$,
and after switching let the output node consume all the outstanding 
messages and then perform circuit evaluation.
%as described in Lemma~\ref{lm:circuit-evaluation-correct}.
That is, let each of the operation node agents observe the arguments' values and update their current value (or more accurately, let the agents for the argument nodes emit messages and let the operation node agents read them and update their state). 
Do this inductively on the depth of the operation node until the output node agents update their current value (which by choice of $\vect{y}$ will be $0$). 
Finally let all the agents learn the output node's current value.
        From that point on, all the states 
        and all the messages are consistent with the evaluation of $C$ on
        $\vect{x}$ and $\vect{y}$ with result $0$.
        The universal inputs don't change, since they only change on output $1$.
Therefore from every configuration we can reach a stable consensus with output $0$, and every fair run converges to $0$.

Now assume the statement $\exists\vect{x}:\forall\vect{y}:C(\vect{x},\vect{y})$ is true.
If there is at least one agent for each node of the circuit,
the protocol may choose the universally quantified inputs according to a satisfying $\vect{x}$,
and every configuration reachable after this moment can reach a consensus (possibly non-stable) 
%why not stable? if there are the right existential inputs, then any combination of the universal inputs will output 1
of $1$ by consuming all messages then evaluating the circuit.
%why do we need to consume  all the messages first ?

As we want to evaluate the constant $0$ predicate, we see that the protocol is correct if and only if
$\exists\vect{x}:\forall\vect{y}:C(\vect{x},\vect{y})$ fails,
and it is enough to consider a single instance where there is a single agent per node.
Therefore correctness for DO protocols is $\Pi^p_2$-hard.
 \end{proof}


==> mfdo-intro.tex <==
We introduce a new protocol model called \emph{message-free delayed observation} (MFDO) to help us prove verification questions for the delayed observation model.
Immediate observation and delayed observation protocols present similarities. 
Essentially, in an immediate observation protocol an agent updates its state when it observes that another agent is \emph{currently} in a certain state $q$, while in a delayed observation protocol the agent observes that another agent \emph{was} in a certain state $q$, provided that agent \emph{emitted a message when it was in $q$}.

In  a message-free delayed observation protocol, we assume that such a message
is always emitted by default.  Equivalently, we dispense with the message, and directly assume 
that an agent can observe whether another agent went through a given state in the past. This is 
why we call the model ``message-free delayed'' observation. 

\begin{definition}
A message-free delayed observation (MFDO) protocol is a pair $(Q, \delta)$, where $Q$ is a set of states and $\delta: Q^2 \rightarrow Q$ is a set of transitions.
Transitions are of the form $q,o \rightarrow q',o$, written $q \trans{o} q'$,
 where $q,q',o \in Q$. 
A transition $q \trans{o} q'$ is enabled in an execution $C_0\trans{t_1} C_1 \trans{t_2} \ldots$ at step $i\geq 0$ if $C_i(q)\geq 1$ and $\exists j\leq i$ such that $C_j(o)\geq 1$, \ie there is an agent in $q$ and there was an agent in $o$. 
We say the agent in state $q$ \emph{observes} that there \emph{was} an agent in state $o$ and changes its state to $q'$.
\end{definition}

Given a DO protocol, we define a corresponding MFDO protocol. 

\begin{definition}
\label{def:corresponding-mfdo}
Let $\PP_\textit{DO}=(Q, M, \delta_r, \delta_s)$ be a DO protocol.
Let $\PP_\textit{MFDO}=(Q,\delta)$ be a MFDO protocol where $\delta$ is defined as the transitions $q \trans{o} q'$ such that $q' = \delta_r(q,m)$ for some message $m\in M$, and $o$ is a state such that $m = \delta_s(o)$, for $q \in Q$.
Protocol $\PP_\textit{MFDO}$ is called the \emph{corresponding MFDO protocol} of protocol $\PP_\textit{DO}$.
\end{definition}

Notice that there can be two non-equal states $p,q$ such that $\delta_s(p)=\delta_s(q)=m$ for some message $m\in M$ in $\PP_\textit{DO}$.
In this case, if there exists some $q',q''$ such that $\delta_r(q',m)=q''$, then protocol $\PP_\textit{MFDO}$ contains transitions $q'\trans{p} q''$ and $q' \trans{q} q''$.

\begin{example}\label{do-protocol-mfdo}
Consider the DO protocol $\PP_\textit{DO}=(Q, M, \delta_r, \delta_s)$
where  $Q=M=\set{a, b, ab}$, $\Sigma=\set{a,b}$, $\iota(a) = a$, and $\iota(b)=b$.
The send transitions are given by $\delta_s(q)=(q, q)$ for all $q \in Q$, \ie, every state 
can send a message with its own identity to itself, denoted $q \send{q} q$. The receive transitions are $\delta_r(a,b)=ab$ and $\delta_r(b,a)=ab$, denoted $a \trans{b} ab$ and $b \trans{a} ab$. The output function is defined by $o(a)=o(b)=0$ and $o(ab)=1$.

The corresponding MFDO protocol is $\PP_\textit{MFDO}=(Q, \delta)$ with $\delta$ defined as the transitions $a \trans{b} ab$ and $b \trans{a} ab$.
%The protocol calculates the predicate which is true if and only if there is at least one $a$ and one $b$ initially.
\end{example}

Well-specification in MFDO and DO are different: we can find DO protocols whose corresponding MFDO protocols are well-specified whereas they are not, and vice-versa. 
Indeed, an agent in a DO protocol can ``choose" not to send a message when it goes through a state, and thus not enable a future transition using this message. 
The protocol can get ``stuck" in a non-consensus or a falsely stable consensus. 
This does not happen in MFDO as the agent is assumed to always send enough messages when it goes through a state.
In the other direction, an MFDO protocol can allow some transition to an undesirable state indefinitely by virtue of there always being enough messages, whereas in the DO protocol the messages will eventually run out and the undesirable state will no longer be reachable.

\begin{example}
In Example \ref{do-protocol-mfdo}, the DO protocol $\PP_\textit{DO}$ is not well-specified.
Indeed, the execution $(a \send{a})(b \trans{a} ab)$ starting in the configuration with one agent in $a$ and one agent in $b$ is fair (because finite and non-extendable) and ends in a non-consensus configuration.

On the other hand, the corresponding MFDO protocol $\PP_\textit{MFDO}$ cannot get ``stuck" in the same way, as the agent initially in state $b$ enables transition $a \trans{b} ab$ to be fired, resulting in all agents being in state $ab$.
The protocol $\PP_\textit{MFDO}$ is well-specified and correct for the predicate which is true if and only if there is at least one $a$ and one $b$ initially.
%prove this?
\end{example}

\begin{example}
Consider the DO protocol $\PP_\textit{DO}=(Q, M, \delta_r, \delta_s, \Sigma,\iota,o)$.
The state set and message set is $Q=M=\set{init, accept, wait}$, and the only input symbol is $init$, which is mapped to state $init$.
Each state can send a message equal to itself, \ie $\delta_s(q)=q$ for all $q \in Q$.
The receive transitions are $init \trans{init} accept$, $accept \trans{init} wait$ and $wait \trans{wait} accept$.
The output function is defined by $o(q)=1$ if $q=accept$ and $0$ otherwise.
The corresponding MFDO protocol is not well-specified: the agent initially in $init$ all eventually go to state $accept$, but then by "observing in the past" $init$, they can switch indefinitely between $accept$ and $wait$ thus never reaching a stable consensus.

In $\PP_\textit{DO}$, once all the agents have left the $init$ state, the $init$ messages will eventually run out and agents in $accept$ will stay in $accept$. 
By fairness, the agents still left in $wait$ will send $wait$ messages and eventually all of them will switch their state to $accept$, thus reaching a stable consensus of $1$.
\end{example}

The expressive power of MFDO protocols is still the same as for DO protocols,
as the proofs for both lower and upper bounds from \cite{AAER07} are applicable.
We show that there is an equivalence between reachability in MFDO and reachability in DO. 

\begin{restatable}{lemma}{LemmaDOtoMFDO}
\label{lm:do-to-mfdo}
Let $\PP_\textit{DO}=(Q, M, \delta_r, \delta_s)$ be a DO protocol, and let $\PP_\textit{MFDO}=(Q,\delta)$ be its corresponding MFDO protocol.
Let $C,C'$ be two multisets in $\N^{Q}$.
We note $C_z,C'_z$ their extension to multisets of $\N^{Q \cup M}$ with only zeros on the $M$ components.
Then $C'_z\trans{*}C_z$ in $\PP_{DO}$ if and only if $C' \trans{*} C$ in $\PP_\textit{MFDO}$.
\end{restatable}
%
\begin{proof}[Sketch]
\noindent \textbf{DO to MFDO.}
Let $\sigma$ be an execution from $C'_z$ to $C_z$ in $\PP_\textit{DO}$.
We define an MFDO execution $\sigma'$ by deleting the send transitions and replacing receive transitions $q \trans{m} q'$ by MFDO transitions $q \trans{o} q'$, where $o$ is such that there is a send transition $o \overset{m}{\twoheadrightarrow}$ in $\sigma$ prior to this receive transition.

\noindent \textbf{MFDO to DO.}
Let $\sigma'=(C'=C_0) \trans{t_1} C_1 \trans{t_2} C_2 \ldots C$ be an execution from $C'$ to $C$ in $\PP_\textit{MFDO}$.
It can be made into a DO execution $\sigma$ by adding as many send events as needed each time an agent enters a state, and maintaining a set of the messages in transit with $(0,0,\ldots,0)$ being the initial set of such messages.
 \end{proof}

\cwk{here there could be an example of a DO run being transformed to a MFDO run and vice versa}

%optional last paragraph
Adapting the idea of ``pruning" from \cite{} to the MFDO, we will show that the single-instance correctness problem as well as the general correctness problem for DO protocols are in $\Pi_2^p$.


==> mfdo-pruning-JE.tex <==
We present results that says that any run can be replaced by a \emph{smaller and shorter} run  in an MFDO protocol. 
Smaller in the number of agents, shorter in the number of "aggregated" (or "accelerated") transitions. 
We show these results for extended configurations and extended histories, as this will be useful for future proofs.
%They always also hold for non-extended configurations and histories by Lemma \ref{lm:extendedrun}.

First, we show that the class of well-structured and realizable extended histories is sufficient for describing all the runs of MFDO protocols.

\begin{restatable}{lemma}{LemmaRealizableMFDO}
Let $\PP$ be an MFDO protocol.
Then $(C,\mathcal{S}) \trans{*} (C',\mathcal{S}')$ if{}f there exists a well-structured extended history of initial seen set $\mathcal{S}$ realizable in $\PP$ with $(C,\mathcal{S})$ and $(C',\mathcal{S}')$ as initial and final extended configurations.
\end{restatable}

\begin{remark}
By simply ignoring the seen sets, the above lemma is also true if $C$ and $C'$ are not extended configurations and the history is not an extended history. 
By the same reasoning, this will be true of all the results on extended histories in this section.
\end{remark}

We now proceed to give a syntactic characterization of the well-structured realizable extended histories. 

\begin{definition}
Extended history $(H,\mathcal{S}_H)$ is \emph{compatible with MFDO protocol $\PP$}
if for every trajectory $\tau$ of $H$ and for every non-horizontal step $\tau(i)\tau(i+1)$ of $\tau$, 
the protocol $\PP$ contains a transition $\tau(i) \trans{o} \tau(i+1)$ for some state $o$
such that $o \in \mathcal{S}_H^i$, \ie state $o$ is in the seen set at moment $i$.
\end{definition}

\begin{remark}
%necessary ?
In the case of a non extended history, $H$ is \emph{compatible with MFDO protocol $\PP$}
if for every trajectory $\tau$ of $H$ and for every non-horizontal step $\tau(i)\tau(i+1)$ of $\tau$, 
the protocol $\PP$ contains a transition $\tau(i) \trans{o} \tau(i+1)$ for some state $o$
and $H$ contains a trajectory $\tau'$ with $\tau'(j)=\tau'(j+1)=o$ for some $j\leq i$.
\end{remark}

\begin{restatable}{lemma}{LemmaHistoryMFDO}
Let $\PP$ be an MFDO protocol. 
A well-structured extended history is realizable in $\PP$ if{}f it is compatible with $\PP$.
\end{restatable}

The Pruning Theorem states that we can replace "large" runs by runs with less agents.

\begin{theorem}[Pruning]
\label{thm:mfdopruning}
Let $\PP = (Q,\Delta)$ be an MFDO protocol, let $C$ be a configuration of $\PP$,
and let $(C'',\mathcal{S}'') \trans{*} (C',\mathcal{S}')$ be a run of $\PP$ such that $C' \geq C$.
There exist configurations $D''$ and $D'$ such that 
\begin{center}
\(
\begin{array}[b]{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
(C''&,\mathcal{S}'')   \trans{\hspace{1em}*\hspace{1em}} & (C'&,\mathcal{S}')  \  \geq \ &C  \\[0.1cm]
\geq &  & \geq \\[0.1cm]
(D''&,\mathcal{S}'')  \trans{\hspace{1em}*\hspace{1em}} &(D'&,\mathcal{S}')   \geq  & C
\end{array}
\)
\end{center}
and $|D''| \leq |C| + |Q|$.
\end{theorem}
%
\begin{proof}
By Lemma \ref{lm:extendedcharact}, we can restrict ourselves to run $(C'',\mathcal{S}'') \trans{*} (C',\mathcal{S}')$ such that $\mathcal{S}''=\{ q| C''(q)\geq 1\}$ and $\mathcal{S}'$ is the set of states visited by agents during the run.

Let $(H,\mathcal{S}'')$ be a well-structured realizable extended history for run $(C'',\mathcal{S}'') \trans{*} (C',\mathcal{S}') \geq C$.
For every $q$ in $\mathcal{S}'$, let $f(q)$ be the smallest index $i$ such that $q \in \mathcal{S}_H^i$.
For each state $q$ of $\mathcal{S}'$, we pick a trajectory $\tau_q$ of $H$ such that $q$ is reached by $\tau_q$ at moment $f(q)$.
Define $H'$ as the history $\{ \tau_q | q \in \mathcal{S}' \} \cup H_C$, where $H_C \subset H$ is an arbitrary sub(multi)set of $H$ with final configuration $C$.

This new history $H'$ verifies the $C$-covering property we want, and it is "small": it has at most $|Q|+|C|$ trajectories.
Extended history $(H',\mathcal{S}'')$ is still well-structured and realizable, i.e. compatible with a run of $\PP$. 
To prove this, we rely on the fact that each state is \emph{first} visited by a trajectory in $H'$ at the same moment that it was visited in $H$.
So the seen states are the same along extended histories $(H,\mathcal{S}'')$ and $(H',\mathcal{S}'')$, thus enabling the same transitions in the corresponding runs.
%details to be done
 \end{proof}

We introduce a new measure of the length of runs, the \emph{aggregated length} of a run.
We are going to show, using the setting of the Pruning Theorem, that we can also make runs of MFDO protocols "shorter".
The total number of transitions in the runs we shorten stays the same, but the aggregated length becomes smaller.

\begin{definition}
Let $\PP=(Q,\Delta)$ be an MFDO protocol, and let $\sigma$ be a run in $\PP$.
Run $\sigma$ can be written as $t_1^{k_1} t_2^{k_2} \ldots t_n^{k_n}$ with $t_1,\ldots,t_n \in \Delta$ such that $\forall i, t_i$ and $t_{i+1}$ are distinct, and $k_1,\ldots, k_n \in \N^*$.
We call $n$ the \emph{aggregated length} of $\sigma$ and note it $|\sigma|_a$.
\end{definition}

The Shortening Theorem says we can replace "long" runs with shorter runs (in terms of aggregated length).
This theorem will be used for proving the complexity of the single-instance problem for MFDO and DO protocols.

\begin{theorem}[Shortening]
\label{thm:mfdoshortening}
Let $\PP = (Q,\Delta)$ be an MFDO protocol, and let $(C',\mathcal{S}') \trans{*} (C,\mathcal{S})$ be a run of $\PP$.
Then there exists a run $\sigma$ such that $(C',\mathcal{S}') \trans{\sigma} (C,\mathcal{S})$ and $|\sigma|_a \leq |C||Q|+|Q|^2$.
\end{theorem}
%
\begin{proof}
Let $(H,\mathcal{S}')$ be a well-structured and realizable extended history 
for run $(C',\mathcal{S}') \trans{*} (C,\mathcal{S})$. 

We split the history into at most $|Q|$ segments such that each
segment corresponds to a different seen set of the current extended
configuration. Each segment has exactly one extra element in the
seen set compared to the previous one.
We want to replace each segment with another one 
of bounded length without changing the seen sets corresponding
to the segments.
We ``shorten'' each segment using the following observation.

\textbf{Shortest-path use.} If a trajectory goes from state
$q$ to state $q'$ while the seen set is at most $\seen$ 
(except the last moment where it is $\seen \cup\{q'\}$),
it can go from $q$ to $q'$ in at most $|Q|-1$ steps 
with the seen set $\seen$.
Indeed, each transition in the trajectory 
from $q$ to $q'$ is allowed if the seen set is $\seen$,
and the trajectory represents a path in the oriented
graph of allowed transitions betwen the states.
Removing all the cycles from the path yields the necessary
trajectory of length at most $|Q|-1$. 
%ok, but explanation to be clarified, or drawn

For each non-final segment we choose one of the trajectories $\tau$
that contains the previously unseen state $q'$ in the first 
moment of the next segment. 
Let $q$ be the state in which $\tau$ is at the beginning of the segment.
We replace $\tau$ by the shortest-path from $q$ to $q'$, which is always possible by the discussion in the previous paragraph.
All the other trajectories we let be only horizontal steps, that is they stay in the same state they were at the beginning of the segment.

In the case of the last segment,
we replace each trajectory by the shortest path
from its current state to its final state.

We have $|Q|-1$  segments of length at most $|Q|-1$,
        and one last segment where at most $|C|\times(|Q|-1)$ non-horizontal steps occur.
        Thus, the total number of non-horizontal steps over the whole shortened history is at most $|C||Q|+|Q|^2$.
 \end{proof}


==> mfdo-pruning.tex <==
We present results that says that any run can be replaced by a \emph{smaller and shorter} run  in an MFDO protocol. 
Smaller in the number of agents, shorter in the number of "aggregated" (or "accelerated") transitions. 
We show these results for extended configurations and extended histories, as this will be useful for future proofs.
%They always also hold for non-extended configurations and histories by Lemma \ref{lm:extendedrun}.

First, we show that the class of well-structured and realizable extended histories is sufficient for describing all the runs of MFDO protocols.

\begin{restatable}{lemma}{LemmaRealizableMFDO}
Let $\PP$ be an MFDO protocol.
Then $(C,\mathcal{S}) \trans{*} (C',\mathcal{S}')$ if{}f there exists a well-structured extended history of initial seen set $\mathcal{S}$ realizable in $\PP$ with $(C,\mathcal{S})$ and $(C',\mathcal{S}')$ as initial and final extended configurations.
\end{restatable}

\begin{remark}
By simply ignoring the seen sets, the above lemma is also true if $C$ and $C'$ are not extended configurations and the history is not an extended history. 
By the same reasoning, this will be true of all the results on extended histories in this section.
\end{remark}

We now proceed to give a syntactic characterization of the well-structured realizable extended histories. 

\begin{definition}
Extended history $(H,\mathcal{S}_H)$ is \emph{compatible with MFDO protocol $\PP$}
if for every trajectory $\tau$ of $H$ and for every non-horizontal step $\tau(i)\tau(i+1)$ of $\tau$, 
the protocol $\PP$ contains a transition $\tau(i) \trans{o} \tau(i+1)$ for some state $o$
such that $o \in \mathcal{S}_H^i$, \ie state $o$ is in the seen set at moment $i$.
\end{definition}

\begin{remark}
%necessary ?
In the case of a non extended history, $H$ is \emph{compatible with MFDO protocol $\PP$}
if for every trajectory $\tau$ of $H$ and for every non-horizontal step $\tau(i)\tau(i+1)$ of $\tau$, 
the protocol $\PP$ contains a transition $\tau(i) \trans{o} \tau(i+1)$ for some state $o$
and $H$ contains a trajectory $\tau'$ with $\tau'(j)=\tau'(j+1)=o$ for some $j\leq i$.
\end{remark}

\begin{restatable}{lemma}{LemmaHistoryMFDO}
Let $\PP$ be an MFDO protocol. 
A well-structured extended history is realizable in $\PP$ if{}f it is compatible with $\PP$.
\end{restatable}

The Pruning Theorem states that we can replace "large" runs by runs with less agents.

\begin{theorem}[Pruning]
\label{thm:mfdopruning}
Let $\PP = (Q,\Delta)$ be an MFDO protocol, let $C$ be a configuration of $\PP$,
and let $(C'',\mathcal{S}'') \trans{*} (C',\mathcal{S}')$ be a run of $\PP$ such that $C' \geq C$.
There exist configurations $D''$ and $D'$ such that 
\begin{center}
\(
\begin{array}[b]{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
(C''&,\mathcal{S}'')   \trans{\hspace{1em}*\hspace{1em}} & (C'&,\mathcal{S}')  \  \geq \ &C  \\[0.1cm]
\geq &  & \geq \\[0.1cm]
(D''&,\mathcal{S}'')  \trans{\hspace{1em}*\hspace{1em}} &(D'&,\mathcal{S}')   \geq  & C
\end{array}
\)
\end{center}
and $|D''| \leq |C| + |Q|$.
\end{theorem}
%
\begin{proof}
By Lemma \ref{lm:extendedcharact}, we can restrict ourselves to run $(C'',\mathcal{S}'') \trans{*} (C',\mathcal{S}')$ such that $\mathcal{S}''=\{ q| C''(q)\geq 1\}$ and $\mathcal{S}'$ is the set of states visited by agents during the run.

Let $(H,\mathcal{S}'')$ be a well-structured realizable extended history for run $(C'',\mathcal{S}'') \trans{*} (C',\mathcal{S}') \geq C$.
For every $q$ in $\mathcal{S}'$, let $f(q)$ be the smallest index $i$ such that $q \in \mathcal{S}_H^i$.
For each state $q$ of $\mathcal{S}'$, we pick a trajectory $\tau_q$ of $H$ such that $q$ is reached by $\tau_q$ at moment $f(q)$.
Define $H'$ as the history $\{ \tau_q | q \in \mathcal{S}' \} \cup H_C$, where $H_C \subset H$ is an arbitrary sub(multi)set of $H$ with final configuration $C$.

This new history $H'$ verifies the $C$-covering property we want, and it is "small": it has at most $|Q|+|C|$ trajectories.
Extended history $(H',\mathcal{S}'')$ is still well-structured and realizable, i.e. compatible with a run of $\PP$. 
To prove this, we rely on the fact that each state is \emph{first} visited by a trajectory in $H'$ at the same moment that it was visited in $H$.
So the seen states are the same along extended histories $(H,\mathcal{S}'')$ and $(H',\mathcal{S}'')$, thus enabling the same transitions in the corresponding runs.
%details to be done
 \end{proof}

We introduce a new measure of the length of runs, the \emph{aggregated length} of a run.
We are going to show, using the setting of the Pruning Theorem, that we can also make runs of MFDO protocols "shorter".
The total number of transitions in the runs we shorten stays the same, but the aggregated length becomes smaller.

\begin{definition}
Let $\PP=(Q,\Delta)$ be an MFDO protocol, and let $\sigma$ be a run in $\PP$.
Run $\sigma$ can be written as $t_1^{k_1} t_2^{k_2} \ldots t_n^{k_n}$ with $t_1,\ldots,t_n \in \Delta$ such that $\forall i, t_i$ and $t_{i+1}$ are distinct, and $k_1,\ldots, k_n \in \N^*$.
We call $n$ the \emph{aggregated length} of $\sigma$ and note it $|\sigma|_a$.
\end{definition}

The Shortening Theorem says we can replace "long" runs with shorter runs (in terms of aggregated length).
This theorem will be used for proving the complexity of the single-instance problem for MFDO and DO protocols.

\begin{theorem}[Shortening]
\label{thm:mfdoshortening}
Let $\PP = (Q,\Delta)$ be an MFDO protocol, and let $(C',\mathcal{S}') \trans{*} (C,\mathcal{S})$ be a run of $\PP$.
Then there exists a run $\sigma$ such that $(C',\mathcal{S}') \trans{\sigma} (C,\mathcal{S})$ and $|\sigma|_a \leq |C||Q|+|Q|^2$.
\end{theorem}
%
\begin{proof}
Let $(H,\mathcal{S}')$ be a well-structured and realizable extended history 
for run $(C',\mathcal{S}') \trans{*} (C,\mathcal{S})$. 

We split the history into at most $|Q|$ segments such that each
segment corresponds to a different seen set of the current extended
configuration. Each segment has exactly one extra element in the
seen set compared to the previous one.
We want to replace each segment with another one 
of bounded length without changing the seen sets corresponding
to the segments.
We ``shorten'' each segment using the following observation.

\textbf{Shortest-path use.} If a trajectory goes from state
$q$ to state $q'$ while the seen set is at most $\seen$ 
(except the last moment where it is $\seen \cup\{q'\}$),
it can go from $q$ to $q'$ in at most $|Q|-1$ steps 
with the seen set $\seen$.
Indeed, each transition in the trajectory 
from $q$ to $q'$ is allowed if the seen set is $\seen$,
and the trajectory represents a path in the oriented
graph of allowed transitions betwen the states.
Removing all the cycles from the path yields the necessary
trajectory of length at most $|Q|-1$. 
%ok, but explanation to be clarified, or drawn

For each non-final segment we choose one of the trajectories $\tau$
that contains the previously unseen state $q'$ in the first 
moment of the next segment. 
Let $q$ be the state in which $\tau$ is at the beginning of the segment.
We replace $\tau$ by the shortest-path from $q$ to $q'$, which is always possible by the discussion in the previous paragraph.
All the other trajectories we let be only horizontal steps, that is they stay in the same state they were at the beginning of the segment.

In the case of the last segment,
we replace each trajectory by the shortest path
from its current state to its final state.

We have $|Q|-1$  segments of length at most $|Q|-1$,
        and one last segment where at most $|C|\times(|Q|-1)$ non-horizontal steps occur.
        Thus, the total number of non-horizontal steps over the whole shortened history is at most $|C||Q|+|Q|^2$.
 \end{proof}


==> new-pruning-setting.tex <==
This section introduces so-called pruning theorems for MFDO and IO protocols. 
These results are the central tool for proving the easiness results for the well-specification problem for DO and IO protocols.
A pruning theorem for IO protocols was presented in \cite{CONCUR}.
We recall it and adapt it to MFDO protocols.
%Put a note somewhere in the section on why it doesnt work for message-passing protocols and non-observation protocols

%the rest of the setting is currently quite similar to last paper's pruning section - might need to be changed to avoid self-plagiarism
Intuitively, the pruning theorems state that if a configuration $C$ is coverable from a configuration $C"$, then it is also coverable from a "small" configuration $D"\leq C"$, where small means $|D"| \leq |C|+|Q|^3$.
To do this, given a covering execution, we look at the trajectories of the different agents and keep only the ones that are ''necessary". 
Since the transitions of population protocols do not create or destroy agents, we can give agents identities. 
%\je{What for? Before introducing definitions or results, tell the reader why they are needed.}
Given an execution, each agent of the initial configuration follows a \emph{trajectory}, or sequence of \emph{steps}, through the states of the protocol until it reaches the final configuration of the run. 

\begin{definition}
A \emph{trajectory} is a sequence $\tau =p_1 \ldots p_n$ of states. We denote $\tau(i)$ the $i$-th state of $\tau$. The \emph{$i$-th step} of $\tau$ is the pair $\tau(i)\tau(i+1)$ of adjacent states.

A \emph{history} is a multiset of trajectories of the same length. The length of a history is the common length of its trajectories. 
Given a history $H$ of length $n$ and index $1 \leq i \leq n$, the \emph{$i$-th configuration of $H$}, denoted $C_{H}^i$, is defined as follows: for every state $p$, $C_{H}^i(p)$ is the number of trajectories $\tau \in H$ such that $\tau(i)=p$. 
The configurations $C_{H}^1$ and $C_{H}^n$ are called the \emph{initial} and \emph{final} configurations of $H$.
\end{definition}

\begin{example}
\label{history-ex}
Histories can be graphically represented. Figure \ref{figure-history} shows a history $H$ of length $7$. It consists of five trajectories: one trajectory from $q_3$ to $q_3$ passing only through $q_3$, and four trajectories from $q_1$ to $q_3$ which follow different state sequences.
The first configuration of $H$ is $C_{H}^1= (4,0,1)$ and the seventh and last configuration is $C_{H}^7=(0,0,5)$. 
\end{example}

\begin{definition}
A history $H$ of length $n\geq 1$ is \emph{realizable} in a population protocol $\PP$ if there exist transitions of $\PP$ $t_1, \ldots, t_{n-1}$ and numbers $k_1, \ldots, k_{n-1} \geq 0$ such that 
$$C_{H}^1 \trans{t_1^{k_1}}C_{H}^2 \cdots  C_{H}^{n-1} \trans{t_{n-1}^{k_{n-1}}} C_{H}^n \ .$$
\noindent For every transition $t$ of $\PP$, we define $t^0$ as the \emph{empty transition} which moves no agents and is always enabled, and we note it $t_{\varepsilon}$. \je{Where is this needed?}
%new addition

\end{definition}

\begin{remark}
Notice that histories of length $1$ are always realizable. Observe also that there may be more than one realizable history corresponding to a firing sequence, because the firing sequence does not keep track of which agent visits which states, while the history does.
\end{remark}

\input{figure-history.tex}
%
\begin{example}
\label{history-ex2}
Let $\PP=(Q,\delta)$  be the IO protocol with $Q=\{ q_1,q_2,q_3 \}$ and $\delta = \{t_1, t_2, t_3, t_4\}$, where 
$$\begin{array}{lcl}
t_1 = q_1 \trans{q_1} q_2  & \quad  & t_3 = q_1 \trans{q_3} q_3\\
t_2 = q_2 \trans{q_2} q_3  &            & t_4 = q_2 \trans{q_3} q_3
\end{array}$$
The history $H$ of Example \ref{history-ex} is realizable in $\PP$. 
Indeed, we have  $C_{H}^1 \trans{t_3 \, t_1^2 \, t_3 \, t_2 \, t_4 } C_{H}^7$.
\end{example}

\begin{definition}
A step $\tau(i)\tau(i+1)$ of a trajectory $\tau$ is \emph{horizontal} if $\tau(i) = \tau(i+1)$, and \emph{non-horizontal} otherwise.

A history $H$ of length $n$ is \emph{well-structured} if for every $1 \leq i \leq n-1$ one of the two following conditions hold:
\begin{itemize}
\item For every trajectory $\tau \in H$, the $i$-th step of $\tau$ is horizontal.
\item For every two trajectories $\tau_1, \tau_2 \in H$, if the $i$-th steps of $\tau_1$ and $\tau_2$ are non-horizontal, then they are equal.
\end{itemize}
\end{definition}

\noindent \textbf{Extended Configurations} 
%\je{Why is this here? Where is it going to be used?} 
The results we prove over MFDO can be expressed in a clearer way by reasoning over extended configurations that include a set of states.
In an execution, these extended configurations keep track of which states have been visited, or ''seen" by agents of the execution.
These extended configurations allow us to express that a transition is enabled in a local way. 

\begin{definition} 
        An \emph{extended configuration} for an MFDO protocol is
        a configuration $C$ together with a set $\mathcal{S}$ of \emph{seen states}.
        The intended semantics of the seen state set, or \emph{seen set},
        is to represent the states that have occurred 
        in the configurations preceding and including $C$ in a certain execution.
        We require that the set of seen states contain
        all the states of configuration $C$ in which there is at least one agent, \ie $\{ q \ | \ C(q)\geq 1\} \subseteq \seen$.

        %Extended configurations allow us to define MFDO transition enabled-ness 
        %without reference to the run. 
        Given an extended configuration $(C,\mathcal{S})$, transition $q\trans{o}q'$ is enabled
        if{}f $C(q)\geq 1$ and $o\in \mathcal{S}$. 
        The resulting extended configuration is $(C-q+q',\mathcal{S}\cup\{q'\})$.
        We call \emph{extended execution} an execution in which we keep track of the seen states, 
        that is an execution $(C_0,\mathcal{S}_0)\trans{t_1}(C_1,\mathcal{S}_1)\trans{t_2}(C_2,\mathcal{S}_2)\ldots$ where
        each transition $t_i$ is enabled as described above.
        
        There exists an execution $C_0\trans{t_1}C_1\trans{t_2}\ldots C_n$ 
if{}f there exists an extended execution $(C_0, \mathcal{S}_0) \trans{t_1} (C_1, \mathcal{S}_1) \trans{t_2} \ldots (C_n,\mathcal{S}_n)$ for the sets $\mathcal{S}_i =\{ q| \exists j\leq i \ . \ C_j(q)\geq 1\}$, and these sets are minimal such that this be true.
We call them the \emph{minimal seen sets} for execution $C_0\trans{t_1}C_1\trans{t_2}\ldots C_n$.
When considering an extended execution with minimal seen sets, the final seen set is the set of all the states visited by agents during the execution.
\end{definition}

%The minimal necessary seen set for a run is described in the following lemma:
%
%\begin{lemma}
%\label{lm:extendedrun}
%\cwk{integrate this lm in definition}
%Let $\PP=(Q,\delta)$ be an MFDO protocol. 
%There exists a run $C_0\trans{t_1}C_1\trans{t_2}\ldots C_n$ in $\PP$
%if{}f there exists an extended run $(C_0, \mathcal{S}_0) \trans{t_1} (C_1, \mathcal{S}_1) \trans{t_2} \ldots (C_n,\mathcal{S}_n)$ for the sets $\mathcal{S}_i =\{ q| \exists j\leq i \ . \ C_j(q)\geq 1\}$ which are minimal such that this be true.
%\end{lemma}
%%
%\begin{proof}
%By definition of MFDO and extended runs.
% \end{proof}
%
%\begin{remark}
%When considering an extended run with minimal seen sets, the final seen set is the set of all the states visited by agents during the run.
%\end{remark}

The following lemma gives a characterization for extended executions.

\begin{lemma}
\label{lm:extendedcharact}
Let $\PP=(Q,\delta)$ be an MFDO protocol.
Sequence $(C_0, \mathcal{T}_0) \trans{t_1} (C_1, \mathcal{T}_1) \trans{t_2} \ldots (C_n,\mathcal{T}_n)$ is an extended execution in $\PP$
if{}f there exists a set $\mathcal{T} \subseteq Q$ such that $\mathcal{T}_i=\{ q| \exists j\leq i \ . \ C_j(q)\geq 1\} \cup \mathcal{T}$ for $0 \leq i \leq n$.
\end{lemma}
%
\begin{proof}
By definition of seen sets of extended configurations, the effects of transitions and the fact that extra states in the seen sets are of no consequence.
 \end{proof}

We now extend the definitions of histories to these extended executions.

\begin{definition}
An \emph{extended history} is given by a multiset of trajectories of the same length constituting a history $H$ and an initial seen set $\mathcal{S}_{H}$.
Given an extended history $(H,\mathcal{S}_{H})$ of length $n$ and index $1 \leq i \leq n$, \emph{the $i$-th extended configuration of $(H,\mathcal{S}_{H})$} is denoted $(C_{H}^i,\mathcal{S}_{H}^i)$.
Configuration $C_{H}^i$ is defined as above, and $\mathcal{S}_{H}^i$ is defined as $\mathcal{S}_{H}$ if $i=1$ and $\mathcal{S}_{H}^{i-1} \cup \{ q | \exists \tau. \tau(i)=q \}$ otherwise.

The other definitions can be extended:
\begin{itemize}
\item
An extended history $(H,\mathcal{S}_{H})$ is \emph{realizable} in an MFDO protocol $\PP$ if there exist transitions of $\PP$ $t_1, \ldots, t_{n-1}$ and numbers $k_1, \ldots, k_{n-1} \geq 0$ such that $(C_{H}^1,\mathcal{S}_{H}^1) \trans{t_1^{k_1}} (C_{H}^2,\mathcal{S}_{H}^2) \cdots  (C_{H}^{n-1},\mathcal{S}_{H}^{n-1}) \trans{t_{n-1}^{k_{n-1}}} (C_{H}^{n},\mathcal{S}_{H}^{n})$.
%this means that the seen sets are already well-defined, by definition of a run with extended configs.
\item
An extended history is \emph{well-structured} if its underlying history is well-structured.
\end{itemize}
\end{definition}

\input{figure-history-mfdo.tex}
%
\begin{example}
\label{history-ex-mfdo}
Figure \ref{figure-history-mfdo} illustrates a history $H$ of length $4$.
It consists of five trajectories: one trajectory from $a$ to $ab$, and four trajectories from $b$ to $ab$ which follow different state sequences.
$H$'s first configuration is $C_{H}^1= (1,4,0)$ and $H$'s fourth and last configuration is $C_{H}^4=(0,0,5)$.

Extended history $(H,\set{a,b})$ is realizable in the MFDO protocol of Example \ref{do-protocol-mfdo}, \ie $\PP_\textit{MFDO}=(Q,\delta)$  
which has state set $\{ a,b,ab \}$ and transitions $t_1=a \trans{b} ab$ and $t_2=b \trans{a} ab$.
Indeed $(C_{H}^1,\set{a,b}) \trans{t_2} (C_{H}^2,Q) \trans{t_1} (C_{H}^3,Q) \trans{t_2^3} (C_{H}^4,Q)$.
\end{example}


==> notation.tex <==
We are now ready to introduce the full list of models studied by Angluin \etal in \cite{AAER07}. 


The first two are restrictions of the standard population protocol of Definition \ref{def:standard-pp}, and the last two are restrictions of the queued transmission protocol of Definition \ref{def:queued-transmission}.

%rendez-vous then message
\paragraph{Standard population protocols (PP).} At each step, two agents exchange information about their current states, and update them according to a joint transition function. Communication is immediate. 

\paragraph{Immediate Transmission Protocols (IT).}
In this protocol, a first agent can transmit (or broadcast) its state. 
This transmission is immediately received by a second agent which changes its state accordingly. 
The first agent may change its state after transmission, but it knows nothing about the agent which received the transmission.
Formally, an immediate transmission protocol is like the standard population protocol except that there exists two functions $\delta_1,\delta_2$ such that the transition function $\delta$ verifies $\delta(q_1,q_2)=(\delta_1(q_1), \delta_2(q_1,q_2))$ for all $q_1,q_2\in Q$.

\paragraph{Immediate Observation Protocol (IO).}
In this protocol, the state of a first agent can be observed by a second agent.
This second agent changes its state using this information.
Unlike in the immediate transmission model, the first agent does not know it has been observed, and so it does not update its state.
Formally, an immediate transmission protocol is like the standard population protocol except that there exists a function $\delta_1,$ such that the transition function $\delta$ verifies $\delta(q_1,q_2)=(q_1, \delta_1(q_1,q_2))$ for all $q_1,q_2\in Q$.

\paragraph{Queued Transmission Protocol (QT).}
In this protocol, the agents communicate by message-passing. 
A first agent sends a message which is a function of its current state, and then updates its own state.
A second agent receives this message if it is in a state in which it can receive it.
Another way of seeing this is that an agent can "temporarily refuse" to receive a message (until it is in a "good" state).
Once the message is received, the receiving agent updates its state.
This protocol is formally defined in Definition \ref{def:queued-transmission}.
The fact that an agent can "temporarily refuse" a message is translated by the fact that the transition function for received messages is partial.

\paragraph{Delayed Transmission Protocol (DT)}
This protocol is similar to the queued transmission protocol, except that agents cannot "temporarily refuse" to receive messages. 
That is, the transition function for received messages is a total function $\delta_r:Q\times M \rightarrow Q$.
It is called delayed transmission because an agent transmits a message which will not be read immediately, unlike in the immediate transmission model where an agent directly transmits its state information to another agent.

\paragraph{Delayed Observation Protocol (DO)}
This protocol is similar to the queued transmission protocol, except that agents cannot "temporarily refuse" to receive messages \emph{and} they cannot update their states once they have sent a message.
Formally this translates as $\delta_r$ being a total function and $\delta_s$ being such that for all $q\in Q$, $\delta_s(q)=(q,m)$ for some $m\in M$.

\medbreak
In the following sections, we establish complexity bounds for the single instance correctness problem and the correctness problem for each of these five models of one-way communication. 
The order in which we will present the results is the order of increasing complexity, shown in Table \ref{tab:complexity}.
\medbreak

\cwk{the following on notation is for us, not part of the final text}
To make the transitions in the different models clearer to read, we propose the following notations:
\begin{itemize}
 \item
For general transitions, $q_1,q_2 \rightarrow q_3,q_4$. This applies to two way population protocols and IT protocols.
\item
For IO and MFDO transitions (ie that involve observation of states): $q \trans{o} q'$ for $q,q',o$ states.
\item
For models with messages, receive transitions are of the form $q \trans{m} q'$ for $q,q'$ states and $m$ a message, and send transitions are of the form $q \send{m} q'$.
For DO protocols, send transitions never modify the state of the sender, so we can write the transition $q \send{m}$.
\end{itemize}
Notice that all these shorthands allow marking the arrows with the name of the protocol, in case we are talking about more than one, e.g. $q \trans{o}_{\PP} q'$.


==> probabilistic.tex <==


Fairness conditions are often described as a deterministic
reachability-based approximation
to probabilistic properties of runs.
Message-based model permit the set of configurations
reachable from a given one to be infinite, making certain
arguments in favour of such an approximation unsuitable.
In the current section we study the
relation of fairness and probabilistic conditions
for delayed transmission
and queued transmission models.

\begin{definition}
        A run \emph{converges} to an output value $O$
        if all the configurations except a finite number
        are consensus configurations with the same output.

        A protocol \emph{converges} to and output value $O$
        from configuration $C$
        if a random run starting from $C$ converges to $O$
        almost surely.

        A protocol \emph{probabilistically implements}
        a function $O(\cdot)$ if it converges to $O(C)$
        for each input configuration $C$.

        A protocol is \emph{probabilistically well-specified}
        if it implements some function.
\end{definition}

\begin{definition}
        A configuration is \emph{recurrent}
        in a run if it occurs infinitely many times.
\end{definition}

\begin{definition}
        A probabilistic model of execution is \emph{positive}
        if every possible transition has a positive probability.

        A probabilistic model has \emph{Markov property}
        if transition probabilities conditional on the
        configuration are independent on the previous history.
\end{definition}

\begin{definition}
        A probabilistic model for a message-based protocol is \emph{message-instance-uniform}
        if for each configuration $C$ and each agent $a$ in $C$
        all message instances of message types that $a$ can receive
        are equally likely to be received by $a$ on the next step.
\end{definition}

\begin{definition}
        A probabilistic model for a message-based protocol is \emph{message-type-uniform}
        if for each configuration $C$ and each agent $a$ in $C$
        all message types that $a$ can receive
        are equally likely to be received by $a$ on the next step.
\end{definition}

\begin{theorem}
        \mr{either refer to the proof or copy}

        Consider a Markov positive probabilistic execution model
        for a message-free protocol (e.g. IO, IT or MFDO protocol).
        Then a random run i fair with probability $1$.

        Furthermore, for each fair run there is a positive probability
        for a random run to have the same set of recurrent configurations.
\end{theorem}

\begin{corollary}
        Verifying probabilistic well-specification
        of a message-free protocol
        with respect to
        a Markov positive probabilistic model has the same complexity
        as verifying well-specification.
\end{corollary}

\begin{definition}`
        \emph{Transmit-receive $p:1-p$ odds model}
        is described by the following random procedure.

        On each step, a uniformly random agent is picked.
        Afterwards, with probability $p$ it transmits a message
        of type chosen uniformly at random among all the
        message types it can send, and with probability $1-p$
        it tries to receive a message chosen uniformly at random
        from all the present ones.

        If the chosen agent cannot transmit any messages
        or cannot receive the chosen message, nothing happens.
\end{definition}

\begin{theorem}
        Consider a delayed transmission protocol
        and transmit-receive $0.1:0.9$ odds model.

        Then a random run is fair with probability $1$
        and for each fair run there is a positive probability
        for a random run to have the same set of recurrent
        configurations.
\end{theorem}

The proof is based on the following lemma.

\begin{lemma}
        Consider a delayed transmission protocol
        and transmit-receive $0.5:0.5$ odds model.

        Then a random run contains infinitely
        many configurations with no messages
        with probability $1$.
\end{lemma}

\begin{proof}
        For a configuration $C$ let $p(C)$
        denote the probability of a random run
        starting from $C$ not to each any
        state with no messages.

        Let $p(n,k)$ be the maximum $p(C)$
        among all the configurations
        with $n$ agents and $k$ messages.

        For some $n$ and $k>0$ consider the configuration
        $C_{max}$
        with $n$ agents and $k$ messages
        with $p(C_{max}=p(n,k)$.
        A step from configuration $C_{max}$
        has probability of at least $0.5$
        of consuming a message (in a delayed transmission protocol
        an agent can always receive any message),
        and probability $q$ between $0$ and $0.5$ of producing a message.
        Consumption of a message leads to a configuration
        with $k-1$ agent which has to have probability of never reaching zero messages
        at most $p(n,k-1)$; production of a message leads to a configuration with
        the corresponding probability at most $p(n,k+1)$.
        Therefore $p(n,k)=p(C_{max})\leq 0.5\,p(n,k-1) + q\,p(n,k+1) + (0.5-q)\,p(n,k)$.
        This means that either $p(n,k)>p(n,k+1)$ or $p(n,k)\leq 0.5\,p(n,k-1)+0.5\,p(n,k+1)$.
        The second case can be rewritten as $p(n,k+1)\geq p(n,k) + (p(n,k)-p(n,k-1))$.

        By definition $p(n,0)=0$. By induction it is easy to see $p(n,k)\geq k\,p(n,1)$.
        But as $p(n,k)\leq 1$ we have $p(n,1)=0$.
        If $z = max k: p(n,k)=0$ by induction we have $p(n,k)\geq (k-z)\,p(n,z)$.
        Therefor $z=\infty$ and $p(n,k)=0$, which is equivalent to the statement of the lemma.
 \end{proof}

Now we can prove the theorem.

\begin{proof}
        Consider an arbitrary configuration $C$ and initial configuration $C_0$.
        There is a finite set of configurations with zero messages reachable from $C_0$.
        For each such reachable configuration $C'$, either $C$ is unreachable from $C'$,
        or there is a shortest sequence of transitions leading from $C'$ to $C$
        (possibly not unique). Such a sequence has a positive probability of occurring
        given $C'$. Let $p_{min}$ be the minimal probability of all the
        probabilities of shortest paths, and $L$ be the maximum length
        of a shortest path.

        Now consider a random run. It starts with $C_0$.
        With probability $1$ it will reach a zero-message configuration.
        Either $C$ is unreachable by that moment, or probability of
        reaching it in at most $L$ steps is at least $p_{min}$.
        If $C$ is not reached in $L$ steps but remains reachable,
        with probability $1$ we will again reach a zero-message configuration.

        Therefore, the action of checking if $C$ is reached in $L$
        steps, then waiting for a zero-message configuration
        has a probability of complete failure $0$, and probability
        of success ($C$ is reacehd or becomes unreachable) at least $p_{min}$.
        Infinite repetition of such an action will yield an infinite number of
        successes with probability $1$. We see that a random run is fair
        with probability $1$.

        Now consider an arbitrary fair run. Every configuration can reach
        some configuration without messages and there is only a finite number
        of configurations without messages reachable from the initial configuration.
        Therefore there is a recurrent zero-message configuration $C_r$.
        The set of recurrent configurations in
        a fair run is the same as the set of all configurations reachable from $C_r$.
        There is a positive probability that a random run reaches $C_r$,
        and as the continuation is fair with probability $1$,
        the conditional probability of having the same set of recurrent states
        given that $C_r$ is reached is $1$.

        This concludes the proof.
 \end{proof}

\begin{theorem}
        For each Markov positive message-uniform model for queued transmission,
        protocol well-specification is undecidable.
\end{theorem}

\begin{proof}
        According to \cite{} binary chemical reaction networks
        with uniform rates
        can model arbitrary computable functions.
        Such a network is equivalent to having a multiset
        of molecules, and repeatedly picking two of them at random
        and letting them interact, producing an arbitrary number of product molecules.
        A binary chemical reaction network can be modelled
        by a single agent who sends the initial set of messages,
        then receives two randomly chosen messages, tries to run
        the reaction, sends the results and repeats.

        Note that such a protocol 
        will have the same distribution of the next non-silent transition
        regardless
        of details of a probabilistic model (under the chosen conditions).

        If the same agent runs the protocol on two non-interacting sets of messages
        modelling two different computations, 
        remembers the current candidate output of each computation 
        and alternates them as the output, well-specification
        is at least as hard as verifying whether two total functions
        are equal, which is undecidable.
 \end{proof}



==> pruning-setting.tex <==
This section introduces so-called pruning theorems for MFDO, DO and IO protocols. 
These results are the central tool for proving the easiness results for the well-specification problem for DO and IO protocols.
A pruning theorem for IO protocols was presented in \cite{CONCUR}.
We recall it again and adapt it to MFDO protocols.
%Put a note somewhere in the section on why it doesnt work for message-passing protocols and non-observation protocols

%the rest of the setting is currently quite similar to last paper's pruning section - might need to be changed to avoid self-plagiarism
Intuitively, the pruning theorems state that if a configuration $C$ is coverable from a configuration $C"$, then it is also coverable from a "small" configuration $D"\leq C"$, where small means $|D"| \leq |C|+|Q|$ in the case of MFDO protocols, and $|D"| \leq |C|+|Q|^3$ in the case of IO protocols.
To do this, given a covering run, we look at the trajectories of the different agents and keep only the ones that are ''necessary". 
Since the transitions of population protocols do not create or destroy agents, we can give agents identities. 
%\je{What for? Before introducing definitions or results, tell the reader why they are needed.}
Given a run, each agent of the initial configuration follows a \emph{trajectory}, or sequence of \emph{steps}, through the states of the protocol until it reaches the final configuration of the run. 

\je{This section needs pictures!!!!!}
\begin{definition}
A \emph{trajectory} is a sequence $\tau =p_1 \ldots p_n$ of states. We denote $\tau(i)$ the $i$-th state of $\tau$. The \emph{$i$-th step} of $\tau$ is the pair $\tau(i)\tau(i+1)$ of adjacent states.

A \emph{history} is a multiset of trajectories of the same length. The length of a history is the common length of its trajectories. 
Given a history $H$ of length $n$ and index $1 \leq i \leq n$, \emph{the $i$-th configuration of $H$}, denoted $C_{H}^i$, is defined as follows: for every state $p$, $C_{H}^i(p)$ is the number of trajectories $\tau \in H$ such that $\tau(i)=p$. 
The configurations $C_{H}^1$ and $C_{H}^n$ are called the \emph{initial} and \emph{final} configurations of $H$.

A history $H$ of length $n\geq 1$ is \emph{realizable} in a population protocol $\PP$ if there exist transitions of $\PP$ $t_1, \ldots, t_{n-1}$ 
and numbers $k_1, \ldots, k_{n-1} \geq 0$ such that $C_{H}^1 \trans{t_1^{k_1}}C_{H}^2 \cdots  C_{H}^{n-1} \trans{t_{n-1}^{k_{n-1}}} C_{H}^n$.
%new addition
For any transition $t$ of $\PP$, we define $t^0$ as the \emph{empty transition} which moves no agents and is always enabled, and we note it $t_{\varepsilon}$.
Notice that a history of length $1$ is always realizable.
\end{definition}

\begin{definition}
A step $\tau(i)\tau(i+1)$ of a trajectory $\tau$ is \emph{horizontal} if $\tau(i) = \tau(i+1)$, and \emph{non-horizontal} otherwise.

A history $H$ of length $n$ is \emph{well-structured} if for every $1 \leq i \leq n-1$ one of the two following conditions hold:
\begin{itemize}
\item For every trajectory $\tau \in H$, the $i$-th step of $\tau$ is horizontal.
\item For every two trajectories $\tau_1, \tau_2 \in H$, if the $i$-th steps of $\tau_1$ and $\tau_2$ are non-horizontal, then they are equal.
\end{itemize}
\end{definition}

\noindent \textbf{Extended Configurations} 
%\je{Why is this here? Where is it going to be used?} 
The results we prove over MFDO can be expressed in a clearer way by reasoning over extended configurations that include a set of states.
In a run, these extended configurations keep track of which states have been visited, or ''seen" by agents of the run.
These extended configurations allow us to express that a transition is enabled in a local way. 

\begin{definition} 
        An \emph{extended configuration} for an MFDO protocol is
        a configuration $C$ together with a set $\mathcal{S}$ of \emph{seen states}.
        The intended semantics of the seen state set, or \emph{seen set},
        is to represent the states that have occurred 
        in the configurations preceding and including $C$ in a certain run.
        We require that the set of seen states contain
        all the states of configuration $C$ in which there is at least one agent, \ie $\{ q \ | \ C(q)\geq 1\} \subseteq \seen$.

        %Extended configurations allow us to define MFDO transition enabled-ness 
        %without reference to the run. 
        Given an extended configuration $(C,\mathcal{S})$, transition $q\trans{o}q'$ is enabled
        if{}f $C(q)\geq 1$ and $o\in \mathcal{S}$. 
        The resulting extended configuration is $(C-q+q',\mathcal{S}\cup\{q'\})$.
        We call \emph{extended run} a run in which we keep track of the seen states, 
        that is a run $(C_0,\mathcal{S}_0)\trans{t_1}(C_1,\mathcal{S}_1)\trans{t_2}(C_2,\mathcal{S}_2)\ldots$ where
        each transition $t_i$ is enabled as described above.
        
        There exists a run $C_0\trans{t_1}C_1\trans{t_2}\ldots C_n$ 
if{}f there exists an extended run $(C_0, \mathcal{S}_0) \trans{t_1} (C_1, \mathcal{S}_1) \trans{t_2} \ldots (C_n,\mathcal{S}_n)$ for the sets $\mathcal{S}_i =\{ q| \exists j\leq i \ . \ C_j(q)\geq 1\}$, and these sets are minimal such that this be true.
We call them the \emph{minimal seen sets} for run $C_0\trans{t_1}C_1\trans{t_2}\ldots C_n$.
When considering an extended run with minimal seen sets, the final seen set is the set of all the states visited by agents during the run.
\end{definition}

%The minimal necessary seen set for a run is described in the following lemma:
%
%\begin{lemma}
%\label{lm:extendedrun}
%\cwk{integrate this lm in definition}
%Let $\PP=(Q,\delta)$ be an MFDO protocol. 
%There exists a run $C_0\trans{t_1}C_1\trans{t_2}\ldots C_n$ in $\PP$
%if{}f there exists an extended run $(C_0, \mathcal{S}_0) \trans{t_1} (C_1, \mathcal{S}_1) \trans{t_2} \ldots (C_n,\mathcal{S}_n)$ for the sets $\mathcal{S}_i =\{ q| \exists j\leq i \ . \ C_j(q)\geq 1\}$ which are minimal such that this be true.
%\end{lemma}
%%
%\begin{proof}
%By definition of MFDO and extended runs.
% \end{proof}
%
%\begin{remark}
%When considering an extended run with minimal seen sets, the final seen set is the set of all the states visited by agents during the run.
%\end{remark}

The following lemma gives a characterization for extended runs.

\begin{lemma}
\label{lm:extendedcharact}
Let $\PP=(Q,\delta)$ be an MFDO protocol.
Sequence $(C_0, \mathcal{T}_0) \trans{t_1} (C_1, \mathcal{T}_1) \trans{t_2} \ldots (C_n,\mathcal{T}_n)$ is an extended run in $\PP$
if{}f there exists a set $\mathcal{T} \subseteq Q$ such that $\mathcal{T}_i=\{ q| \exists j\leq i \ . \ C_j(q)\geq 1\} \cup \mathcal{T}$ for $0 \leq i \leq n$.
\end{lemma}
%
\begin{proof}
By definition of seen sets of extended configurations, the effects of transitions and the fact that extra states in the seen sets are of no consequence.
 \end{proof}

We now extend the definitions of histories to these extended runs.

\begin{definition}
An \emph{extended history} is given by a multiset of trajectories of the same length constituting a history $H$ and an initial seen set $\mathcal{S}_{H}$.
Given an extended history $(H,\mathcal{S}_{H})$ of length $n$ and index $1 \leq i \leq n$, \emph{the $i$-th extended configuration of $(H,\mathcal{S}_{H})$} is denoted $(C_{H}^i,\mathcal{S}_{H}^i)$.
Configuration $C_{H}^i$ is defined as above, and $\mathcal{S}_{H}^i$ is defined as $\mathcal{S}_{H}$ if $i=1$ and $\mathcal{S}_{H}^{i-1} \cup \{ q | \exists \tau. \tau(i)=q \}$ otherwise.

The other definitions can be extended:
\begin{itemize}
\item
An extended history $(H,\mathcal{S}_{H})$ is \emph{realizable} in an MFDO protocol $\PP$ if there exist transitions of $\PP$ $t_1, \ldots, t_{n-1}$ and numbers $k_1, \ldots, k_{n-1} \geq 0$ such that $(C_{H}^1,\mathcal{S}_{H}^1) \trans{t_1^{k_1}} (C_{H}^2,\mathcal{S}_{H}^2) \cdots  (C_{H}^{n-1},\mathcal{S}_{H}^{n-1}) \trans{t_{n-1}^{k_{n-1}}} (C_{H}^{n},\mathcal{S}_{H}^{n})$.
%this means that the seen sets are already well-defined, by definition of a run with extended configs.
\item
An extended history is \emph{well-structured} if its underlying history is well-structured.
\end{itemize}
\end{definition}




==> pruning-thm.tex <==
In this section, we present the fundamental property of immediate observation nets that entails most of the results in this paper: the Pruning Theorem. 

The Pruning Theorem intuitively states that if $M$ is coverable from a large marking $M''$, then it is also coverable from a small marking $S'' \leq M''$, where small means $|S''| \leq |M| + |P|^3$.

\begin{theorem} [Pruning Theorem]
\label{thm:pruning}
Let $N = (P,T,F)$ be an IO net, let $M$ be a marking of $N$, and let
$M'' \trans{*} M'$ be a firing sequence of $N$ such that $M' \geq M$.
There exist markings $S''$ and $S'$ such that 
\begin{center}
\(
\begin{array}[b]{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
M'' &  \trans{\hspace{1em}*\hspace{1em}} & M' & \  \geq \ &M  \\[0.1cm]
\geq &  & \geq \\[0.1cm]
S'' & \trans{\hspace{1em}*\hspace{1em}} &S'  & \geq  & M
\end{array}
\)
\end{center}
and $|S''| \leq |M| + |P|^3$.
\end{theorem}

It is easy to see that for $M' = M$ the Pruning Theorem holds, because since $N$ is conservative, $|M''|=|M|$ and we can choose $S''=M''$.
It is also not difficult to find a non-IO net for which the theorem does not hold. 

\begin{example}
Consider our IO net represented in Figure \ref{figure-running-example}.
There is an execution $(30,0,1) \trans{*} (0,0,31)$ where $(0,0,31)$ covers $(0,0,2)$. 
By application of the Pruning Theorem, we obtain an execution $(3,0,1) \trans{*} (0,0,4) \geq (0,0,2)$ where $|(3,0,1)|=4$ is smaller than $|(0,0,2)|+3^3=29$.
\end{example}
%this example is a little weird because I do not say how we obtain the result - it is almost the same execution as the one used in examples further in the section, except that for graphic reasons the execution starts in (4,0,1) instead of (30,0,1). But 4+1 is already smaller than 2+n^3 and so it doesn't make sense as an example here....

\begin{example}[A non-IO net for which the theorem does not hold.] 
To see that the IO condition cannot be replaced with conservativeness of the network, consider the net with $4$ places $q_1,q_2,q_3,q_4$ and a single transition $(q_1,q_2)\mapsto(q_3,q_4)$.
There is an execution $(1000,1000,0,0) \trans{*} (0,0,1000,1000) \geq (0,0,100,0)$.
But to cover $(0,0,100,0)$ from a marking below $(1000,1000,0,0)$ we need to fire the transition at least $100$ times.
This requires a marking with $200 > 100 + 4^3$ tokens.
\end{example}

\subsection{Trajectories and histories}

Since the transitions of IO nets do not create or destroy tokens, we can give tokens identities.
Given a firing sequence, each token of the initial marking follows a \emph{trajectory}, or sequence of \emph{steps}, through the places of the net until it reaches the final marking of the sequence. 


\begin{definition}
A \emph{trajectory} is a sequence $\tau =p_1 \ldots p_n$ of places. We denote $\tau(i)$ the $i$-th place of $\tau$. The \emph{$i$-th step} of $\tau$ is the pair $\tau(i)\tau(i+1)$ of adjacent places.

A \emph{history} is a multiset of trajectories of the same length. The length of a history is the common length of its trajectories. Given a history $H$ of length $n$ and index $1 \leq i \leq n$, \emph{the $i$-th marking of $H$}, denoted $M_{H}^i$, is defined as follows: for every place $p$, $M_{H}^i(p)$ is the number of trajectories $\tau \in H$ such that $\tau(i)=p$. The markings 
$M_{H}^1$ and $M_{H}^n$ are called the \emph{initial} and \emph{final} markings of $H$.

A history $H$ of length $n$ is \emph{realizable} if there exist transitions $t_1, \ldots, t_{n-1}$ 
and numbers $k_1, \ldots, k_{n-1} \geq 0$ such that $M_{H}^1 \trans{t_1^{k_1}}M_{H}^2 \cdots  M_{H}^{n-1} \trans{t_{n-1}^{k_{n-1}}} M_{H}^n$.
\end{definition}
\input{figure-history.tex}
%
\begin{example}
\label{history-ex}
Histories can be graphically represented. 
Consider Figure \ref{figure-history} which illustrates a history $H$ of length $7$.
It consists of five trajectories: one trajectory from $q_3$ to $q_3$ passing only through $q_3$, and four trajectories from $q_1$ to $q_3$ which follow different place sequences.
$H$'s first marking is $M_{H}^1= (4,0,1)$ and $H$'s seventh and last marking is $M_{H}^7=(0,0,5)$.
History $H$ is realizable in the IO net N of Figure \ref{figure-running-example} 
%is it necessary to recall the places and transitions here ?
which has place set $\{ q_1,q_2,q_3 \}$ and transitions $t_1 = (q_1, q_1)\mapsto(q_2,q_1), t_2 = (q_2,q_2)\mapsto(q_3,q_2),t_3 = (q_1,q_3)\mapsto(q_3,q_3)$ and $t_4 = (q_2,q_3)\mapsto(q_3,q_3)$.
Indeed $M_{H}^1 \trans{t_3 t_1^2 t_3 t_2 t_4 } M_{H}^7$.
\end{example}

We then have the following result, whose proof can be found in the appendix.

\begin{restatable}{lemma}{LemmaRealizable}
\label{lem:realizable}
$M \trans{*} M'$  if{}f $N$ has a realizable history with $M$ and $M'$ as initial and final markings.
\end{restatable}

\begin{remark}
Notice that there is more than one realizable history corresponding to a firing sequence in an IO net, because the firing sequence does not keep track of which token goes where, while the history does.
\end{remark}


\subsection{A syntactic characterization of realizable histories}

The graphical representation of histories suggests the following definition of horizontal and non-horizontal steps:

\begin{definition}
A step $\tau(i)\tau(i+1)$ of a trajectory $\tau$ is \emph{horizontal} if $\tau(i) = \tau(i+1)$, and \emph{non-horizontal} otherwise.
\end{definition}

We now proceed to give a syntactic characterization of the realizable histories. 

\begin{definition}
A history $H$ of $N$ of length $n$ is \emph{well-structured} if for every $1 \leq i \leq n-1$ one of the two following conditions hold:
\begin{itemize}
\item For every trajectory $\tau \in H$, the $i$-th step of $\tau$ is horizontal.
\item For every two trajectories $\tau_1, \tau_2 \in H$, if the $i$-th steps of $\tau_1$ and $\tau_2$ are non-horizontal, then they are equal.
\end{itemize}
$H$ is \emph{compatible with $N$}
if for every trajectory $\tau$ of $H$ and for every non-horizontal step $\tau(i)\tau(i+1)$ of $\tau$, 
the net $N$ contains a transition $(\tau(i), p_o)~\mapsto~(\tau(i+1), p_o)$ for some place $p_o$
and $H$ contains a trajectory $\tau'$ with $\tau'(i)=\tau'(i+1)=p_o$.
\end{definition}

This entails the following lemma, and the proof can be found in the appendix.

\begin{restatable}{lemma}{LemmaHistory}
A history is realizable if{}f it is well-structured and compatible with $N$.
\end{restatable}

\begin{example}
In the realizable history $H$ of Figure \ref{figure-history}, all the trajectories are such that the third step is horizontal. 
For every $i \neq 3$, there is exactly one trajectory taking a non-horizontal $i$-th step, and so $H$ is indeed well-structured.
For $N$ our IO net of Figure \ref{figure-running-example}, $H$ is compatible with $N$.
\end{example}


\subsection{Pruning histories}

We start by introducing bunches of trajectories.

\begin{definition}
 A \emph{bunch} is a multiset of trajectories with the same length and the same
        initial and final place. 
\end{definition}

\begin{example}
Figure \ref{figure-history}'s realizable history is constituted of a trajectory from $q_3$ to $q_3$ and a bunch $B$ with initial place $q_1$ and final place $q_3$ made up of four different trajectories. 
\end{example}

We show that every realizable history containing a bunch of size larger than $|P|$ can be ``pruned'', meaning that the bunch can be replaced by a smaller one, while keeping the history realizable.

\begin{lemma}
\label{lm:pruning}
Let $H$ be a realizable history of $N$ containing a bunch $B\subseteq H$ of size larger than $|P|$. There exists a nonempty bunch $B'$ of size at most $|P|$ with the same initial and final
places as $B$, such that the history $H' \defeq H - B + B'$ (where $+, -$ denote multiset addition and subtraction) is also realizable.
\end{lemma}
%
\begin{proof}
Let $P_B$ be a set of all places visited by at least one trajectory in the bunch $B$.
        For every $p\in P_B$ let $f(p)$ and $l(p)$ be the earliest and the latest
        moment in time when this place has been used by any of the trajectories
        (the first and the last occurrence can be in different trajectories).

        Let $t_p, p\in P_B$ be a trajectory that first goes to $p$ by the moment $f(p)$, then
        waits there until $l(p)$, then goes from $p$ to the final place.
        To go to and from $p$ it uses the observed segments of trajectories.

        We will take $B'=\{t_p\mid p\in P_B\}$ and prove that replacing $B$ with $B'$ in $H$
        does not violate the requirements for being a $N$-history.
        Note that we can copy the same fragment of
        a trajectory multiple times.

        First let us check well-structuring condition. Note that we build $t_p$ by taking fragments
        of existing trajectories and using them at the exact same moments in time, and by adding some
        horizontal fragments. Therefore, the set of non-horizontal steps in $B'$ is a subset (if
        we ignore multiplicity) of the set of non-horizontal steps in $B$, and the replacement
        operation cannot increase the set of non-horizontal steps occurring in $H$.

        Now let us check compatibility with $N$. We claim that the set of horizontal steps present
        in $B'$ is at least as large as in $B$
        (again, ignoring multiplicities - multiplicities are not
        relevant for compatibility with immediate-observation protocols). Indeed, any horizontal
        step with place $p$ in a trajectory in $B$ has to occur between $f(p)$ and $l(p)$, but then
        $t_p$ also has a horizontal step there.

        As the replacement operation can only decrease the set of non-horizontal steps and
        it can only increase the set of horizontal steps, it cannot create a new violation
        of compatibility condition (which has a shape of ``for each non-horizontal step there
        exists a corresponding horizontal step'').
        
 \end{proof}

\input{figure-pruned.tex}
%
\begin{remark}
Note that the bunch $B$ does not have to be maximal:
there can be some more trajectories with the same initial and final place in the history.
\end{remark}
\begin{example}
Consider the realizable history of Figure \ref{figure-history}, leading from $(4,0,1)$ to $(0,0,5)$, which covers marking $(0,0,2)$.
Bunch $B$ from $q_1$ to $q_3$ is of size four which is bigger than $|P|=3$. 
The set $P_B$ of places visited by trajectories of $B$ is equal to $P$.
Figure \ref{figure-pruned} is annotated with the first and last moments $f(p)$ and $l(p)$ for $p \in P_B$.
Lemma \ref{lm:pruning} applied to $H$ and $B$ ``prunes" bunch $B$ into $B'$ made up of trajectories $t_{q_1},t_{q_2},t_{q_3}$, drawn in blue in Figure \ref{figure-pruned}.
Notice that in this example, the non-horizontal $5$-th step in $H$ does not appear in the new realizable history $H' = H - B + B'$.
History $H'$ is such that $M_{H'}^1=(3,0,1) \trans{t_3 t_1 t_3 t_4 }(0,0,4)=M_{H'}^7$ and $M_{H'}^7 \geq (0,0,2)$.
\end{example}

\subsection{Proof of the Pruning Theorem}

Using Lemma \ref{lm:pruning} we can now finally prove the Pruning Theorem:

\begin{proof}[of Theorem \ref{thm:pruning}]
Let $M'' \trans{*}  M'  \  \geq  \ M$. 
By Lemma \ref{lem:realizable}, there is a realizable history $H$ with $M''$ and $M'$ as initial and final markings, respectively. Let $H_M \subset H$ be an arbitrary sub(multi)set of $H$ with final
marking $M$, and define $H'=H-H_M$. Further, for every $p, p' \in P$, let $H'_{p,p'}$ be the bunch of all trajectories of $H'$ with $p$ and $p'$ as initial and final places, respectively. We have

$$H' = \sum_{p,p' \in p} H'_{p,p'}$$

So $H'$ is the union of $|P|^2$ (possibly empty) bunches. Apply Lemma \ref{lm:pruning} to each bunch of $H'$ with more than $|P|$ trajectories yields a new history

$$H'' = \sum_{p,p' \in p} H''_{p,p'}$$

\noindent such that $|H''_{p,p'}| \leq |P|$ for every $p, p' \in P$, and such that the history $H'' + H_M$ is realizable. 

Let $S''$ and $S'$ be the initial and final markings of $H'' + H_M$. We show that $S''$ ans $S'$ satisfy the required properties:
\begin{itemize}
\item $S'' \trans{*} S'$, because  $H'' + H_M$ is realizable.
\item $S' \geq M$, because $H_M \subseteq H'' + H_M$. 
\item $|S''| \leq |M| + |P|^3$ because $|H'' + H_M| = \sum_{p', p} |H''_{p,p'}| + |H_M| \leq |P|^2 \cdot |P| + |M| = |M| + |P|^3$.
\end{itemize}
This concludes the proof.

 \end{proof}

\begin{remark}
A slight modification of our construction allows one to prove Theorem~\ref{thm:pruning} (but not Lemma \ref{lm:pruning}) with $2|P|^2$ overhead instead of $|P|^3$. We provide more details in the appendix.
However, since some results of Section \ref{CC} explicitly rely on Lemma~\ref{lm:pruning}, we prove Theorem~\ref{thm:pruning} as a consequence of Lemma~\ref{lm:pruning} for simplicity.
\end{remark}


==> section-decidability.tex <==

We present a generic result showing that the correctness problem is decidable for a class of protocols satisfying certain properties. All protocol models considered in the paper, with the exception of QT, satisfy the properties. The proof follows closely the one of \cite{EsparzaGLM17} for standard population protocols. 
However, the presentation emphasizes the role played by each of the properties, allowing us to pinpoint why the proof of \cite{EsparzaGLM17} can be generalized to DT protocols, but not to QT protocols. While we leave the decidabililty of correctness for QT open, we also argue that the notion of fairness chosen in \cite{AAER07}, and also used in our paper, is questionable for QT, making the correctness problem for QT less interesting than for the other five models.


\subsubsection{Reducing correctness to a reachability problem}

We introduce the class of well-behaved protocols.

\begin{definition}
\label{def:wbP}
A generalized protocol $\PP=(\Conf, \Sigma, \Step, I, O)$ is \emph{well-behaved} if every fair execution contains a \emph{bottom configuration}: a configuration $C$ such that
for every $C' \in \Conf$ if $C \trans{*} C'$ then $C' \trans{*} C$. (In other words, $C$ is a bottom configuration if it belongs to a bottom SCC of the configuration graph of the protocol.)
For $\PP$ a well-behaved protocol, let $\B$ denote the set of its bottom configurations.
\end{definition}

We show that correctness of well-behaved protocols can be reduced to a reachability question. In the next section we prove that, under certain additional conditions, this reachability question is decidable.  Before presenting the reduction, we prove a little lemma.

\begin{lemma}
\label{lem:little}
Every finite execution of a protocol leading to a bottom configuration can be extended to a fair execution.
\end{lemma}
\begin{proof}
Let $C, \ldots, C'$ with $C' \in \B$ be a finite execution.
If the SCC of $C'$ is finite, then the result is immediate: Let $C_0, \ldots, C_{n-1}$ be an enumeration of the SCC such that $C_0 = C'$. Since $C_{(i+1) \mod n}$ is reachable from $C_i$ for every $0 \leq i \leq n-1$, start with the execution $C, \ldots, C'$, and then repeat the following for $j=0,1,2, \ldots $: extend the current execution to another one leading to $C_{j \mod n}$. The infinite execution generated this way is fair. The same procedure does not work when $\B$ is infinite, but the problem can be solved by dovetailing. Since $\B$ is countable, there is an enumeration $C_0, C_1, \ldots$ of $\B$. Take any bijection $f \colon \N \rightarrow \N \times \N$, and, starting with the execution $C, \ldots, C'$, repeat for $j=0,1,2, \ldots $: if $f(j) = (k, \ell)$, then extend the current execution to another one that visits $C_k$ at least $\ell$ times. The resulting execution is fair.
 \end{proof}


Observe that every fair execution of a well-behaved protocol eventually gets trapped in a bottom SCC of the configuration graph and, by fairness, visits all its configurations infinitely often. This occurs independently of whether the SCC contains finitely or infinitely many configurations.


\begin{proposition}\label{prop:corr}
Let $\PP$ be a well-behaved protocol,
and let $\varphi$ be a predicate. For $b \in \{0,1\}$, let $\B_b$ denote the set of configurations $C \in \B$ such that every configuration $C'$ in the same SCC as $C$ satisfies $O(C')=b$. 

$\PP$ computes $\varphi$ if{}f for every $b \in \{0,1\}$ the set $\B \setminus \B_b$ is not reachable from $I(\varphi^{-1}(b))$.
\end{proposition}
\begin{proof}
Assume that $\B \setminus \B_b$ is reachable from $\varphi^{-1}(b)$ for some $b \in \{0,1\}$. Then there exists an input $a \in \pop{\Sigma}$ and an execution $C_0, C_1, \ldots, C_i$ such that $\varphi(a)=b$, $I(a) = C_0$, and $C_i \in \B \setminus \B_b$. 
Since $C_i \in \B$, by Lemma \ref{lem:little} the execution can be extended to a fair execution $C_0, C_1, \ldots$. Since $C_{i+k} \trans{*} C_i$ for every $k \geq 0$, the execution visits $C_i$ infinitely often. Since $C_i \notin \B_b$, the execution does not converge to $b$. So $\PP$ does not compute $\varphi$. 

Assume that $\PP$ does not compute $\varphi$. Then there exists an input $a \in \pop{\Sigma}$, a boolean $b \in \{0,1\}$, and a fair execution $\pi=C_0, C_1, \ldots$ such that $\varphi(a)=b$ and $I(a) = C_0$, but $\pi$ does not converge to $b$. Since $\PP$ is well-behaved, $\pi$ contains a configuration $C_i \in \B$. Since $\pi$ does not converge to $b$, there is $j > i$ such that $O(C_j)$ is undefined, or defined but different from $b$. Since $C_j$ belongs to the same SCC as $C_i$, we have $C_i \notin \B_b$.
 \end{proof}


%\paragraph{Well specification.} For the reduction of the well-specification problem we define the square of a protocol $\PP$. Intuitively, the square of $\PP$ is the protocol obtained by putting two disjoint copies of $\PP$ side by side, starting at the same initial configuration, and letting then move synchronously (i.e., a step of the square corresponds to a move in both copies of $\PP$). Since we are not interested in the predicate computed by the square, and so its output function is always undefined.
%
%\begin{definition}
%Let $\PP =(\Conf, \Sigma, \Step, I, O)$ be a protocol. The \emph{square} of $\PP$ is the protocol $\sq{\PP} = (\sq{\Conf}, \Sigma, \sq{\Step}, \sq{I}, \sq{O})$ given by 
%\begin{itemize}
%\item $\sq{\Conf} = \Conf \times \Conf$,
%\item $\big( \tup{C_1, C_2} , \tup{C_1', C_2'} \big) \in \sq{\Step}$ if{}f  $(C_1, C_1') \in \Step$ and $(C_2, C_2') \in \Step$.
%\item $\sq{I}(a) = \tup{ I(a), I(a) }$ for every $a \in \pop{\Sigma}$, and 
%\item $\sq{O}\big( \tup{C_1, C_2} \big)$ is undefined for every $\tup{C_1, C_2} \in \sq{\Conf}$.
%\end{itemize}
%\end{definition}
%
%Proposition \ref{prop:wellspec} below shows that a well-behaved protocol is well-specified if{}f its square satisfies a reachability property.
%
%
%\begin{proposition}\label{prop:wellspec}
%Let $\PP=(\Conf, \Sigma, \Step, I, O)$ be a well-behaved protocol. Let $\B$, $\B_0$, and $\B_1$ be as in Proposition \ref{prop:corr}. Further, define the set $\target$ of configurations of $\sq{\PP}$ as follows:
%$$\target = (\B \times \B) \setminus \big( (\B_0 \times \B_0) \cup (\B_1 \times \B_1) \big) \ .$$
%$\PP$ is well-specified if{}f $\target$ is not reachable from $\sq{I}$ in $\sq{\PP}$. 
%\end{proposition}
%\begin{proof}
%Assume that $\PP$ is ill specified. We prove that $\target$ is reachable from $\sq{I}$.
%Since $\PP$ is ill specified, there is a configuration $C_0$ and either a fair run $\rho = C_0, C_1, C_2 \ldots$ that does not converge, or two fair runs $\rho = C_0, C_1, C_2 \ldots$ and $\rho' = C_0, C_1', C_2' \ldots$ that converge to different values. 
%
%In the first case, since $\PP$ is well-behaved there is an index $i$ such that $C_i$ is a bottom configuration of $\PP$. Since the run does not converge, there exists $j \geq i$ such that $O(C_j)$ is undefined. Since $C_i$ is a bottom configuration of $\PP$ so is $C_j$, and therefore $\tup{C_j, C_j} \in  \target$.
%
%In the second case, since $\PP$ is well-behaved
%there exists an index $i$ such that $C_{i+k}, C_{i'+k}\in \B$ for every $k \geq 0$. Since $\rho$ and $\rho'$ converge, there is $k$ such that $O(C_{i+k})$ and $O(C_{i+k}')$ are defined, but $O(C_{i+k}) \neq O(C_{i+k}')$. If $C_{i+k}$ and $C_{i+k}'$ belong to the same SCC, then by definition of $\B_b$ we have $C_{i+k}, C_{i+k}' \in \B \setminus (\B_0 \cup \B_1)$, and so 
%$\tup{C_{i+k}, C_{i+k}'} \in \target$. 
%
%Assume now that $\target$ is reachable from $\sq{I}$, i.e., there is an initial configuration $\tup{C_0, C_0}$ of $\sq{\PP}$, and a finite execution  $\tup{C_0, C_0}, \tup{C_1, C_1'}, \ldots, \tup{C_i, C_i'} \ldots$ such that $\tup{C_i, C_i'} \in \target$. In particular we have $C_i, C_i' \in \B$. There are three possible cases:
%\begin{itemize}
%\item $C_i \notin (\B_0 \cup \B_1)$. Then the SCC of $C_i$ contains either a configuration $C$ such that $O(C)$ is undefined, or two configurations $C, C'$ such that $O(C)$ and $O(C')$ are defined but$O(C) \neq O(C')$. Since $C_i \in \B$, the execution $C_0, C_1, \ldots, C_i$ can be extended to an infinite fair run that visits all configurations of $\B$ infinitely often. (When $\B$ is infinite this can be easily proved with the help of an enumeration of $\N \times \N$.).This run does not converge, and so $\PP$ is ill specified.
%\item $C_i' \notin (\B_0 \cup \B_1)$. Symmetric. 
%\item $C_i, C_i' \in (\B_0 \cup \B_1)$. Then we can assume without loss of generality that $C_i \in \B_0$ and $C_i' \in \B_1$. Then $C_0, C_1, \ldots, C_i$ and $C_0', C_1', \ldots, C_i'$ are executions of $\PP$ that can be extended to fair runs converging to $0$ and $1$ respectively. So $\PP$ is ill specified.
%\end{itemize}
% \end{proof}

\subsubsection{Correctness is decidable for WFP-protocols}

We introduce some further properties of protocols:

\begin{definition} \label{def:wbP}
	A protocol $\PP=(\Conf, \Sigma, \Step, I, O)$ is 
	\begin{itemize}
		\item \emph{finitely generated} if  $\Conf \subseteq \N^k$ for some $k \geq 0$, and
			there is a finite set $\Delta \subseteq \Z^k$ such that 
			$(C, C') \in \Step$ if{}f $C' - C \in \Delta$; we say that $\Step$ is \emph{generated} by $\Delta$.
		\item \emph{input-Presburger} if for every effectively Presburger set $L \subseteq \pop{\sigma}$ of inputs the set $I(L) \subseteq \pop{Q}$ is an effectively computable Presburger set of configurations.
		\item \emph{output-Presburger} if $O^{-1}(0)$ and $O^{-1}(1)$ are effectively Presburger sets of configurations.
	\end{itemize}

We call a protocol that is well-behaved, finitely generated, and input/output-Presburger a \emph{WFP-protocol}.	
\end{definition}

We show that the condition of Proposition \ref{prop:corr} is decidable for WFP-protocols. A finitely generated protocol $\PP=(\Conf, \Sigma, \Step, I, O)$ can be easily represented as a VAS. Indeed, if $\Conf \subseteq \N^k$ and $\Step$ is generated by $\Delta$, then the VAS has dimension $k$ and has $\Delta$ as set of transitions. Using this fact, and the powerful result stating the decidability of the reachability problem in a VAS between effectively Presburger sets of configurations, we obtain:

\begin{proposition}{\cite{EsparzaGLM17}}\label{prop:effectPres}
Let $\Conf, \Conf'$ be two effectively Presburger sets of configurations of a finitely generated protocol. It is decidable if $\Conf'$ is reachable from $\Conf$. 
\end{proposition}

By Proposition \ref{prop:effectPres}, in order to prove the decidability of correctness it suffices to show that the sets $I(\varphi^{-1}(b))$ and $\B \setminus \B_b$ of a WFP-protocol are effectively Presburger. $I(\varphi^{-1}(b))$ holds by the definition of WFP-protocols (recall that $\varphi^{-1}(b)$ is always a Presburger set). It remains to show that $\B \setminus \B_b$ is effectively Presburger. Since effectively Presburger sets are closed under boolean operations, it suffices to show that $\B$ and $\B_b$ are effectively Presburger. This is a nontrivial result, but already proved in  \cite{EsparzaGLM17}:

\begin{proposition}{(\cite{EsparzaGLM17}, Proposition ??)}
\label{prop:homesemi} 
There is an algorithm that takes as input a finitely generated, output-Presburger protocol, and returns Presburger 
predicates denoting the sets \(\B\), \(\B_0\), and \(\B_1\). 
\end{proposition} 

So we finally obtain:

\begin{theorem}\label{prop:maincorr}
The correctness problem is decidable for WFP-protocols.
\end{theorem}

%\paragraph{Well specification.}  By Proposition \ref{prop:wellspec} and Proposition \ref{prop:effectPres}, in order to prove the decidability of the well-specification problem for FWO-protocols it suffices to show that the 
%sets $\sq{I}(\Sigma^*)$ and $\target$ are effectively Presburger. But this is now an easy task: 
%\begin{itemize}
%	\item $\sq{I}(\Sigma^*)$ is effectively Presburger. Since $\varphi$ is input-Presburger, and Presburger sets are closed under union, the set $I(\Sigma^*)=\varphi^{-1}(0) \cup \varphi^{-1}(1)$ is effectively Presburger. Now we observe that effectively Presburger sets are also closed under \emph{duplication}: for every effectively Presburger set $\C \subseteq \N^k$, the set $\C'=\{ \tup{C, C} \mid C \in \C \} \subseteq \N^{2k}$ is also effectively Presburger. Indeed, if $\varphi(x)$ captures $\C$ then $\varphi( x) \wedge \varphi(y) \wedge x=y$ captures $\C'$. Since $\sq{I}(\Sigma^*)$ is the duplication of $I(\Sigma^*)$, we are done.
%	\item $\target$ is effectively semilinear. Follows easily from the fact that Presburger sets are effectively closed under boolean operations and cartesian product.
%\end{itemize}
%
%\begin{theorem}\label{prop:mainwellspec}
%	The well-specification problem is decidable for FWP-protocols. 
%\end{theorem}


\subsection{Correctness is decidable for PP and DT}

Applying Theorem \ref{prop:maincorr} we can easily prove that the correctness problems is decidable for PP and DT. 
Since IT and IO are subclasses of PP and DO is a subclass of DT, the proof is valid for them as well.

\begin{lemma}
Standard population and delayed-transmission protocols are WFP. 
\end{lemma}
\begin{proof}
The protocols are finitely generated and input/output Presburger by hypothesis. We show that they are also well-behaved.

	In standard population protocols, if $C \trans{*} C'$ then $|C|=|C'|$. It follows that for every configuration $C\in \Conf$ the set of configurations reachable from $C$ is finite. So every fair execution eventually visits a bottom configuration.
	
	In delayed-transmision protocols the size of a configuration is equal to the number of agents plus the number of messages in transit. So there is no bound on the size of the configurations reachable from a given configuration $C$, and in particular the set of configurations reachable from $C$ can be infinite. However, since agents can always receive any message, for every configuration $C$ there is at least one reachable configuration $C'$ without any message in transit. Since the number of such configurations is finite, for every fair execution $\pi = C_0, C_1, \ldots$ there is a configuration $C$ without messages in transit such that $C_i=C$ for infinitely many $i$. By fairness, every configuration $C'$ reachable from $C$ appears infinitely often in $\pi$, and so every configuration $C'$ reachable from $C' \trans{*} C$. So $C$ is a bottom configuration. 
 \end{proof}

\begin{corollary}\label{cor:main}
The correctness problem is decidable for PP, DT, and their subclasses.
\end{corollary}

However, queued-transmission protocols are not necessarily well-behaved, and so not necessarily WFP:

\begin{example}
	\label{ex:fair}
Consider a queued-transmission protocol in which an agent in state $q$ can send a message $m$, staying in $q$. Assume further that no agent can ever receive a message $m$ (because, for example, there are no receiving transitions for it, or because no reachable configuration contains agents in states from which they can receive the message). Then the execution in which the agent in state $q$ sends infinitely often the message $q$ is fair: Indeed, after $k$ steps the system can only reach configurations with at least $k$ messages, and so no configuration is reachable from infinitely many configurations in the execution. Since this fair execution does not visit any bottom configuration, the protocol is not well-behaved.	
\end{example}

Currently, to the best of our knowledge the decidability of the well-specification and correctess problems for queued-transmission protocols is open. At the same time, Example \ref{ex:fair} shows that our fairness condition is questionable for queued-transmission models: An execution $C_0, C_1, \ldots$ in which only one agent acts, even though other agents have enabled actions in $C_i$ for every $i \geq 0$ (because the send function is complete), can still be fair. 
Is the fairness notion of \cite{AAER07} adequate for queued-transmission protocols?

%In the next section we define what it means for a protocol to compute a predicate in a probabilistic setting, and compare it with the definition based on fairness.

%\section{Population Protocols as Petri Nets}
%\label{sec:petrinets}
%The computation of a population protocol can be simulated by an associated Petri net.
%This allows us to apply results on Petri nets to population
%protocols.
%
%%A Petri net $N = (P, T, F)$ consists of a finite set $P$ of \emph{places}, a
%%finite set $T$ of \emph{transitions}, and a {\em flow function} $F \colon (P
%%\times T) \cup (T\times P) \rightarrow \N$. The {\em preset} of a transition
%%\(t\) is the multiset \(\prebullet{t}\) of places given by \(\prebullet{t}(p) =
%%F(p,t)\) and its {\em postset} the multiset \(\prebullet{t}\) given by
%%\(\postbullet{t}(p) = F(t,p)\).  A \emph{marking} \(M \in \setN^{P}\) is a
%%multiset on the set \(P\) of places and we say that $M$ puts \(M(p)\)
%%\emph{tokens} in place \(p\).  A transition $t\in T$ is \emph{enabled at}
%%marking $M$, written $M\fire{t}$, if $\prebullet{t} \leq M$.  A transition $t$
%%that is enabled at $M$ can \emph{fire}, yielding the marking $M' = M -
%%\prebullet{t} + \postbullet{t}$.  We denote this fact as $M\fire{t}M'$.  We
%%extend enabledness and firing inductively to words of transitions as follows.
%%Let $w=t_1\ldots t_k$ be a finite word of transitions $t_j\in T$. We write
%%$M\fire{w}M'$ if there exists a sequence $M_0,\ldots,M_k$ of markings such that
%%$M=M_0\fire{t_1}M_1\cdots\fire{t_k}M_k=M'$, and say that $M'$ is
%%\emph{reachable from $M$}.
%
%
%
%\begin{theorem}\label{thm:reachPres}
%Let $N$ be a Petri net, and let $\phi, \phi'$ be two Presburger predicates denoting 
%sets ${\cal M}, {\cal M'}$ of markings of $N$. The problem whether ${\cal M}'$ is reachable from 
%${\cal M}$ can be reduced to the reachability problem for Petri nets, and is thus decidable.
%\end{theorem}
%
%\begin{theorem}
%\label{thm:mutual}
%The mutual reachability relation of a Petri net $N$ is effectively Presburger-definable.
%\end{theorem}
%
%Using this theorem, we can easily derive an algorithm to construct Presburger predicates for $\mathcal{B}$, $\mathcal{B}_0$, and $\mathcal{B}_1$.
%
%\begin{proposition}
%\label{prop:homesemi} 
%There is an algorithm that takes as input a Petri net $N$ and returns Presburger 
%predicates denoting the sets \(\mathcal{B}\), \(\mathcal{B}_0\), and \(\mathcal{B}_1\). 
%\end{proposition}
%\begin{proof} 
%We show that the predicate $\mathtt{B}(C)$ associated to the set
%of bottom configurations is definable in Presburger arithmetic. Let us
%introduce the predicate $\mathtt{MR}(C,C')$ associated to the mutual
%reachability relation. Theorem~\ref{thm:mutual} shows that
%$\mathtt{MR}(C,C')$ is effectively Presburger.
%Now, we just
%observe that $C$ is a bottom configuration if{}f for every configuration
%$C'$ such that $C$ and $C'$ are mutually reachable and for every 
%$C''$ such that $C' \rightarrow C''$, we have $C$ and $C''$ are also mutually reachable:
%\[\mathtt{B}(C)= \forall C'\,\forall C'' \colon (\mathtt{MR}(C, C') \wedge C' \rightarrow C'') \Rightarrow \mathtt{MR}(C, C'')\enspace .\]
%%
%We claim that ${\cal B}_b$ is a Presburger set of configurations. 
%To prove this, we just notice that  ${\cal B}_b$ is denoted by the
%following predicate:
%%
%\[\mathtt{B}_b(C) = \mathtt{B}(C) \wedge \forall C' \colon \mathtt{MR}(C,C') \Rightarrow \mathtt{O}(C',b)\enspace .\]
%%
%  
% \end{proof}

%\begin{lemma}\label{lem:charwellspec}
%A protocol $(\Conf, \Sigma, \Step, I, O)$ is ill specified if{}f 
%\begin{compactenum}[(1)]
%\item\label{item:unstable} \(\mathcal{B} \setminus (\mathcal{B}_0 \cup \mathcal{B}_1 )\) 
%is reachable from ${\cal I}$, or
%\item\label{item:hesitant} ${\cal I}$ contains a configuration $C \in {\cal I}$ such that 
%both $\mathcal{B}_0$ and $\mathcal{B}_1$ are reachable from $C$.
%\end{compactenum}
%\end{lemma}
%\begin{proof}
%By definition, a protocol is ill specified if{}f
%\begin{compactenum}[(a)]
%\item some fair execution starting at a configuration of ${\cal I}$ does not stabilize to either $0$ or $1$; or
%\item two fair executions starting at the same configuration of ${\cal I}$ stabilize to $0$ and $1$, respectively.
%\end{compactenum}
%We prove that (a) holds if{}f (1) holds, and (b) holds if{}f (2) holds. 
%
%(a) $\Leftrightarrow$ (1). By Lemma~\ref{lem:fair}, a fair execution eventually gets trapped in a bottom SCC $\mathcal{S}$ of the configuration graph, and visits infinitely often every configuration of $\mathcal{S}$. Therefore, the execution
%does not stabilize to either $0$ or $1$ if{}f either $O(C) = \bot$ for some $C \in \mathcal{S}$,
%or $\mathcal{S}$ contains two configurations 
%$C_1$, $C_2$ such that $O(C_1) \neq O(C_2)$. In both cases we have $\mathcal{S} \cap (\mathcal{B}_0 \cup \mathcal{B}_1)= \emptyset$,
%and so $\mathcal{S} \subseteq \mathcal{B} \setminus (\mathcal{B}_0 \cup \mathcal{B}_1 )$.
%
%(b) $\Leftrightarrow$ (2). By Lemma~\ref{lem:fair}, two executions that stabilize to $0$ and $1$ 
%get trapped in two bottom SCCs $\mathcal{S}_0$ and $\mathcal{S}_1$, and visit all configurations of these SCCs infinitely often. So, we have $O(C_0)=0$ for every $C_0 \in \mathcal{S}_0$, and $O(C_1)=1$ for every $C_1 \in \mathcal{S}_1$. It follows $\mathcal{S}_0 \subseteq {\cal B}_0$ and $\mathcal{S}_1 \subseteq {\cal B}_1$, and so both $\mathcal{B}_0$ and $\mathcal{B}_1$ are reachable from some $C \in {I}$. 
% \end{proof}
%
%This lemma reduces the ill specification problem to reachability questions
%for the sets ${\cal I}$, $\mathcal{B}$, $\mathcal{B}_0$, and
%$\mathcal{B}_1$. We use some results of Petri net theory to prove that all these sets
%are effectively Presburger, which allows us to apply Theorem~\ref{thm:reachPres}.


==> small-instance-section-with-mfdo.tex <==
To prove our complexity results for the correctness problem of IO and DO protocols, we are going to show that it is sufficient to only examine ``small" configurations of some ``big" (possibly infinite) sets of configurations.
To describe sets of configurations, we use the formalism of counting sets. 
These were introduced in \cite{EsparzaGMW18} in the context of IO protocols - we recall them here and also adapt them to the new context of MFDO. 
We prove that they are closed under reachability, and describe their size.

%almost directly from old article
\paragraph{Counting constraints and counting sets. }  A \emph{cube} of a protocol $\PP$ is defined as a set of configurations given by a lower bound $L \colon P \rightarrow \N$ and an upper bound $U \colon Q \rightarrow \N \cup \{\infty\}$, written $(L,U)$, and such that configuration $C \in (L,U)$ if{}f $L \leq C \leq U$. 
In the rest of the paper, the term cube will refer both to the set of configurations and to the description by upper and lower bound $(L,U)$.
A \emph{counting constraint} is a formal finite union of cubes, i.e. a formal finite union of upper and lower bound pairs of the form $(L,U)$.
The semantics of a counting constraint is called a \emph{counting set} and it is the union of the cubes defining the counting constraint.
The counting set for a counting constraint $\Gamma$ is denoted $\sem{\Gamma}$.
Notice that one counting set can be the semantics of different counting constraints.
For example, consider a protocol with just one state $q_1$. Let $(L,U)=(1,3)$, $(L',U')=(2,4)$, $(L'',U'')=(1,4)$. 
The counting constraints $(L,U)\cup(L',U')$ and $(L'',U'')$ define the same counting set.
It is easy to show (see also \cite{EsparzaGMW18}) that counting sets are closed under Boolean operations.

%\cwk{new}
An \emph{extended cube} is defined as a cube $\mathcal{C}$ and a seen set $\mathcal{S}$.
An \emph{extended counting constraint} is a formal finite union of extended cubes, and its semantics is called an \emph{extended counting set}.

\paragraph{Measures of counting constraints.} Let $\mathcal{C}=(L,U)$ be a cube, and let $\Gamma = \bigcup_{i=1}^m \mathcal{C}_i$
be a counting constraint. We use the following notations:
$$\begin{array}{lcl}
\lnorm{\mathcal{C}} \defeq \displaystyle \sum_{p \in Q} L(p) & \quad & \unorm{\mathcal{C}} \defeq \displaystyle \sum_{\substack{p\in Q\\ U(p)<\infty}} \!\!\!\!U(p) \mbox{ (and \( 0\) if \(U(p)=\infty\) for all \(p\))}. \\[0.2cm]
\lnorm{\Gamma} \defeq \displaystyle \max_{i\in [1,m]} \{ \lnorm{\mathcal{C}_i} \} &  & \unorm{\Gamma} \defeq \displaystyle \max_{i\in[1,m]} \{ \unorm{\mathcal{C}_i} \}
\end{array}$$
\noindent We call $\lnorm{\mathcal{C}}$ the $l$-norm  and $\unorm{\mathcal{C}}$ the $u$-norm of $\mathcal{C}$. Similarly for $\Gamma$.
We do not take the seen sets into account when defining the norm 
of an extended counting constraint. 
Indeed, a seen set is always of size smaller or equal to the number of states, and so is negligible in the context of our complexity problems.
We recall Proposition 5 of~\cite{EsparzaGMW18} for the norms of the union, intersection and complement.

\begin{proposition}
\label{prop:oponconf}
Let $\Gamma_1, \Gamma_2$ be counting constraints.
\begin{itemize}
\item There exists a counting constraint $\Gamma$ with $\sem{\Gamma} = \sem{\Gamma_1} \cup \sem{\Gamma_2}$ such that
$\unorm{\Gamma} \leq \max \{\unorm{\Gamma_1}, \unorm{\Gamma_2} \}$ and $\lnorm{\Gamma} \leq \max \{\lnorm{\Gamma_1}, \lnorm{\Gamma_2} \}$.
%
\item  There exists a counting constraint $\Gamma$ with $\sem{\Gamma} = \sem{\Gamma_1} \cap \sem{\Gamma_2}$ such that
$\unorm{\Gamma} \leq \unorm{\Gamma_1} + \unorm{\Gamma_2}$ and $\lnorm{\Gamma} \leq \lnorm{\Gamma_1} + \lnorm{\Gamma_2}$.
%
\item There exists a counting constraint $\Gamma$ with $\sem{\Gamma} = \N^n \setminus \sem{\Gamma_1}$ such that
$\unorm{\Gamma} \leq n\lnorm{\Gamma_1}$ and $\lnorm{\Gamma} \leq n\unorm{\Gamma_1} + n$.
%
\end{itemize}
 \end{proposition}

\paragraph{Predecessors and successors of counting sets.}
Fix an IO, DO or MFDO protocol $\PP$. The sets of predecessors and successors of a set $\mathcal{M}$ of configurations of $\PP$ are defined as follows:
$\prestar(\mathcal{M}) \defeq \{ C' | \exists C \in \mathcal{M} \, . \, C' \xrightarrow{*} C \}$, and 
$\poststar(\mathcal{M}) \defeq \{ C | \exists C' \in \mathcal{M} \, . \, C' \xrightarrow{*} C \}$.\\
For $\PP$ an MFDO protocol, the sets of predecessors and successors for a set of extended counting sets $\mathcal{M}_{ext}$ are:
$\prestar(\mathcal{M}_{ext}) \defeq \{ (C',\mathcal{S}') | \exists (C,\seen) \in \mathcal{M}_{ext} \, . \, (C',\mathcal{S}') \xrightarrow{*} (C,\mathcal{S}) \}$, and
$\poststar(\mathcal{M}_{ext}) \defeq \{ (C,\mathcal{S}) | (\exists C',\seen') \in \mathcal{M}_{ext} \, . \, (C',\mathcal{S}') \xrightarrow{*} (C,\mathcal{S}) \}$
%For $\PP$ an MFDO protocol, the predecessor set and successor set for an extended counting set $(\mathcal{M},\mathcal{S})$ are:
%$\prestar(\mathcal{M},\mathcal{S}) \defeq \{ (C',\mathcal{S}') | \exists C \in \mathcal{M} \, . \, (C',\mathcal{S}') \xrightarrow{*} (C,\mathcal{S}) \}$, and
%$\poststar(\mathcal{M},\mathcal{S}) \defeq \{ (C,\mathcal{S}') | \exists C' \in \mathcal{M} \, . \, (C',\mathcal{S}) \xrightarrow{*} (C,\mathcal{S}') \}$.

\begin{lemma}
\label{lm:smallminterm}
Let $(L,U)$ be a cube of an IO protocol $\PP$ of state set $Q$.
For all $C' \in \prestar(L,U)$, there exists a cube $(L',U')$ such that 
\begin{enumerate}
\item $C' \in (L',U') \subseteq  \prestar(L,U)$, and
\item $\lnorm{(L',U')} \leq \lnorm{(L,U)}  + |Q|^3$ and $\unorm{(L',U')} \leq \unorm{(L,U)}$.
\end{enumerate}
\end{lemma}
%
\begin{proof}
Let $C'$ be a configuration of $\prestar(L,U)$.
There exists a configuration $C \in (L,U)$ such that $C' \longrightarrow C$, and $C \geq L$.
The construction from the Pruning Theorem 
applied to this execution
yields configurations $D',D$ such that 
\begin{center}
\(
\begin{array}[b]{@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
C' &  \trans{\hspace{1em}*\hspace{1em}} & C & \  \geq \ &L  \\[0.1cm]
\geq &  & \geq \\[0.1cm]
D' & \trans{\hspace{1em}*\hspace{1em}} &D  & \geq & L
\end{array}
\)
\end{center}
and $|D'| \leq |L| + |Q|^3$.
Since $C$ is in $(L,U)$, we have $U\geq C \geq D \geq L$ and so configuration $D$ is in $(L,U)$ and $D'$ is in $\prestar(L,U)$.

We want to find $L',U'$ satisfying the conditions of the Lemma, i.e. such that $C' \in (L', U')$ and $(L',U') \subseteq  \prestar(L,U)$.
We define $L'$ as equal to configuration $D'$ over each state of $Q$.
The following part of the proof plays out in the setting of the Pruning Theorem section, in which the tokens are de-anonymized. 
Let $H_C$ be a well-structured realizable history from $C'$ to $C$. 
Let $q$ be a state of $Q$.
We want to define $U'(q)$.
Consider $\mathcal{B}^C_q$ the set of bunches in history $H_C$ that have $q$ as an initial state.
For every bunch $B$, let $f_B$ be the final state of the bunch.
We define $U'(q)$ depending on the final states of bunches in $\mathcal{B}^C_q$.

\noindent
\emph{Case 1.} 
There exists a bunch $B$ in $\mathcal{B}^C_q$ whose final state $f_B$ is such that $U(f_B) = \infty$.
In this case we define $U'(q)$ to be $\infty$.

\noindent
\emph{Case 2.}
For all bunches $B$ in $\mathcal{B}^C_q$, the final state $f_B$ of $B$ is such that $U(f_B) < \infty$.
In this case we define $U'(q)$ to be $\sum_{B \in \mathcal{B}^C_q} size(B)$, where $size(B)$ is the number of trajectories with multiplicity in $B$, and $0$ if $\mathcal{B}^C_q$ is empty.

Let us show that $(L',U')$ has the properties we want.
The number of tokens in configuration $C'$ at state $q \in Q$ is the sum of the sizes of the bunches that start from $q$ in history $H_C$.
That is, $C'(q)=\sum_{B \in \mathcal{B}^C_q} size(B)$ which is exactly $U'(q)$ when $U'(q)$ is finite.
Thus for all $q \in Q$, $C'(q) \leq U'(q)$ and $C'(q) \geq D'(q)=L'(q)$, so $C'$ is in $(L', U')$.

The construction from the Pruning Theorem ``prunes" history $H_C$ from $C'$ to $C$ into a well-structured realizable history $H_D$ from $D'$ to $D$ with the same set of non-empty bunches.
We are going to show that $(L',U') \subseteq \prestar(L,U)$ by ``boosting" the bunches of history $H_D$ to create histories $H_R$ which will start in any configuration $R'$ of $(L',U')$ and end at some configuration $R$ in $(L,U)$.
For any constant $k \in \N$, a bunch $B$ of history $H_D$ is \emph{boosted by k} into a bunch $B'$ by selecting any trajectory $\tau$ in $B$ and augmenting its multiplicity by $k$ to create a new bunch $B'$ of size $size(B) + k$.

\input{figure-boost.tex}

Let $R'$ be a configuration in $(L',U')$.
We construct a new history $H_R$ starting in $R'$, and we prove that its final state is in $(L,U)$.
What we aim to build is illustrated in Figure \ref{figure-boost}.
We initialize $H_R$ as the bunches of history $H_D$.
We call $\mathcal{B}^D_q$ the set of the bunches of $H_D$ starting in $q$.

For $q$ such that there is a bunch $B_D \in \mathcal{B}^D_q$ with infinite $U(f_{B_D})$, i.e. such that $\mathcal{B}^D_q$ is in \emph{Case 1} defined above, we take this bunch $B_D$ and boost it by $R'(q) - D'(q)$ into a new bunch $B_R$. 
Informally, we need not worry about exceeding the bound $U$ on the final state of the trajectories of $B_R$, because this state is $f_{B_D}$ and its upper bound is infinite.
The number of trajectories starting in $q$ in history $H_R$ is now $R'(q)$.

Otherwise, $q$ is such that $\mathcal{B}^D_q$ is in \emph{Case 2}, so we know that $R'(q)\leq C'(q)$ because $U'(q)$ was defined to be $C'(q)$. 
Each bunch in $\mathcal{B}^D_q$ in history $H_D$ has a corresponding bunch in history $H_C$ because the pruning operation never erases a bunch completely, it only diminishes its size.
We can boost all bunches in $\mathcal{B}^D_q$ to the size of the corresponding bunches in $H_C$ and not exceed the finite bounds of $U$ on the final states of these bunches.
We arbitrarily select bunches in $\mathcal{B}^D_q$ which we boost so that the sum of the size of bunches in $\mathcal{B}^D_q$ is equal to $R'(q)$.

Now by construction, history $H_R$ starts in configuration $R'$, and it ends in a configuration $R$ such that $D\leq R\leq U$, as every bunch is either boosted to a size no greater than it had in $H_C$, or leads to a state $q$ with $U(q)=\infty$.
Since $D \geq L$, this implies that $R \geq L$ and so $R \in (L,U)$ and $R' \in \prestar(L,U)$.

Finally, we show that the norms of $(L',U')$ are bounded.
For the $l$-norm, we simply add up the tokens in $D=L'$. 
Thus by the Pruning Theorem
\begin{align*}
\lnorm{(L',U')} \leq |L| + |Q|^3 \leq \lnorm{(L,U)} + |Q|^3.
\end{align*}
%
By definition of the $u$-norm, 
$\unorm{(L',U')} = \sum_{\substack{q\in Q | U'(q)<\infty}} U'(q).$
If $U'(q)<\infty$ then $\mathcal{B}^C_q$ of history $H_C$ is in Case $2$ and there is no bunch $B\in \mathcal{B}^C_q$ going from $q$ to a final state $f_B$ such that $U(f_B)=\infty$.
So the set of bunches $B$ starting in a state $q$ such that $U'(q)<\infty$ is included in the set of bunches $B'$ such that $U(f_{B'})<\infty$, and thus
\begin{align*}
\sum_{\substack{q\in Q | U'(q)<\infty}} U'(q) = \sum_{\substack{q\in Q | U'(q)<\infty}} \left( \sum_{B \in \mathcal{B}^C_q} size(B) \right)
\leq \sum_{B | U(f_B)<\infty} size(B).
\end{align*}
Now $\sum_{B | U(f_B)<\infty} size(B)$ in history $H_C$ is exactly $\sum_{\substack{q\in Q | U(q)<\infty}} C(q)$.
Since $C \in (L,U)$, for all states we have $C(q)\leq U(q)$ and so 
\begin{align*}
\sum_{\substack{q\in Q | U'(q)<\infty}} U'(q) \leq \sum_{\substack{q\in Q | U(q)<\infty}} C(q)
\leq \sum_{\substack{q\in Q | U(q)<\infty}} U(q).
\end{align*}
So by definition of the norm, $\unorm{(L',U')} \leq \unorm{(L,U)}$.
 \end{proof}

\begin{restatable}{lemma}{LemmaSmallCubeMFDO}
\label{lm:smallminterm-mfdo}
%\cwk{we could change the notation of cube to $\mathcal{K}$ to not have notation problems}
Let $(\mathcal{C},\mathcal{S})$ be an extended cube of an MFDO protocol $\PP$ of state set $Q$.
For all $(C',\mathcal{S}') \in \prestar(\mathcal{C},\mathcal{S})$, there exists an extended cube $(\mathcal{C}',\mathcal{S}')$ such that 
\begin{enumerate}
\item $(C',\mathcal{S}') \in (\mathcal{C}',\mathcal{S}') \subseteq  \prestar(\mathcal{C},\mathcal{S})$, and
\item $\lnorm{\mathcal{C}'} \leq \lnorm{\mathcal{C}}  + |Q|$ and $\unorm{\mathcal{C}'} \leq \unorm{\mathcal{C}}$.
\end{enumerate}
\end{restatable}
%
\cwk{add proof sketch, whole proof is in appendix}

This results in the following theorems:

\begin{restatable}{theorem}{ThmCCReachabilityIO}
\label{thm:ccreach-io} 
Let $\PP$ be an IO protocol with a set $Q$ of states, and let $S$ be a counting set defined by a counting constraint $\Gamma$.
Then $pre^*(S)$ is a counting set and there exists a counting constraint $\Gamma'$ satisfying $\sem{\Gamma'} = \prestar(S)$, and we can bound the norm of $\Gamma'$ by
 \begin{align*}
\unorm{\Gamma'} \leq \unorm{\Gamma} \text{ and }
\lnorm{\Gamma'} \leq  \lnorm{\Gamma} + |Q|^3
 \end{align*}
The same holds for $\poststar$ by using the protocol with reversed transitions.
\end{restatable}
%
\begin{proof}[Sketch]
Lemma \ref{lm:smallminterm} gives ``small" cubes such that $\prestar(\mathcal{S})$ is the union of these cubes.
Since there are only a finite number of such ``small" cubes, this union is finite and $\prestar(\mathcal{S})$ is a counting set. 
The bounds on the norms of $\prestar(\mathcal{S})$ are derived from the bounds on the norms of these cubes.
 \end{proof}

\begin{restatable}{theorem}{ThmCCReachability}
\label{thm:reachofcc}
Let $\PP$ be an MFDO protocol with a set $Q$ of states, and let $\mathcal{D}$ be an extended counting set defined by an extended counting constraint $\Gamma$. \cwk{what is a good notation for extended counting cstrs/sets?}
Then $pre^*(\mathcal{D})$ is an extended counting set and there exists  an extended counting constraint $\Gamma'$ satisfying $\sem{\Gamma'} = \prestar(\mathcal{D})$, and we can bound the norm of $\Gamma'$ by
 \begin{align*}
\unorm{\Gamma'} \leq \unorm{\Gamma} \text{ and }
\lnorm{\Gamma'} \leq  \lnorm{\Gamma} + |Q|
 \end{align*}
The same holds for $\poststar$ by using the protocol with reversed transitions.
%TRUE FOR ANY GAMMA REPRESENTING D - CHANGE ?
\end{restatable}
%
\begin{proof}[Sketch]
Lemma \ref{lm:smallminterm-mfdo} gives ``small" extended cubes such that $\prestar(\mathcal{D})$ is the union of these extended cubes.
Since there are only a finite number of such ``small" extended cubes, this union is finite and $\prestar(\mathcal{D})$ is an extended counting set. 
The bounds on the norms of $\prestar(\mathcal{D})$ are derived from the bounds on the norms of these extended cubes.
 \end{proof}

